Efficient distributed matrix-free multigrid methods on locally refined meshes for FEM computations

This work studies three multigrid variants for matrix-free finite-element computations on locally refined meshes: geometric local smoothing, geometric global coarsening, and polynomial global coarsening. We have integrated the algorithms into the same framework-the open-source finite-element library deal.II-, which allows us to make fair comparisons regarding their implementation complexity, computational efficiency, and parallel scalability as well as to compare the measurements with theoretically derived performance models. Serial simulations and parallel weak and strong scaling on up to 147,456 CPU cores on 3,072 compute nodes are presented. The results obtained indicate that global coarsening algorithms show a better parallel behavior for comparable smoothers due to the better load balance particularly on the expensive fine levels. In the serial case, the costs of applying hanging-node constraints might be significant, leading to advantages of local smoothing, even though the number of solver iterations needed is slightly higher.

==> chapters/includes.tex <==
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{bm}
\usepackage{pgfplots}
\usepackage{multirow}
\usepackage{subfig}
\usepackage{tikz-uml}
\usepackage{pgf-pie}

\usepackage{setspace}
%\setstretch{2.0}
\usepackage[normalem]{ulem}


\newcommand{\myred}{black}
\newcommand{\myblue}{blue}
\newcommand{\rsout}[1]{{\color{\myred}\sout{#1}}}
\newcommand{\rtext}[1]{{\color{\myred}#1}}

\usepackage{listings}
\usepackage{textcomp}
\definecolor{lbcolor}{rgb}{0.93,0.93,0.93}
\lstset{
	backgroundcolor=\color{lbcolor},
	tabsize=8,
	rulecolor=,
	language=C++,
        basicstyle=\small,
        upquote=true,
        aboveskip={1.5\baselineskip},
        columns=fixed,
        showstringspaces=false,
        extendedchars=true,
        breaklines=true,
        prebreak = \raisebox{0ex}[0ex][0ex]{\ensuremath{\hookleftarrow}},
        frame=single,
        showtabs=false,
        showspaces=false,
        showstringspaces=false,
        identifierstyle=\ttfamily,
        keywordstyle=\color[rgb]{0.7,0.126,0.85},
        commentstyle=\color[rgb]{0.133,0.545,0.133},
        stringstyle=\color[rgb]{0.627,0.126,0.941},
}

\makeatletter
%primitive input in tabular
\AddToHook{env/tabular/begin}{\let\input\@@input}
\makeatother

\usepackage{lineno}
\linenumbers

\usepackage{lineno}
\usetikzlibrary{patterns}
\linenumbers

\definecolor{gnuplot@orange}{RGB}{229,158,0}
\definecolor{gnuplot@purple}{RGB}{148,0,212}
\definecolor{gnuplot@red}{RGB}{200,0,0}
\definecolor{gnuplot@lightblue}{RGB}{87,181,232}
\definecolor{gnuplot@green}{RGB}{0,158,65}
\definecolor{gnuplot@darkblue}{RGB}{0,115,179}
\definecolor{gnuplot@yellow}{RGB}{240,227,66}
\pgfplotscreateplotcyclelist{colorGPL}{%
gnuplot@darkblue,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=o\\%
gnuplot@red,every mark/.append style={fill=gnuplot@red!50!black},mark=square\\%
gnuplot@green,every mark/.append style={fill=gnuplot@green!50!black},mark=triangle*\\%
gnuplot@orange,every mark/.append style={fill=gnuplot@orange!80!black,mark size=2.5pt},mark=x\\%
gnuplot@purple,mark=diamond\\%
black,densely dashed,every mark/.append style={solid,fill=gnuplot@darkblue!80!black},mark=square*\\%
gnuplot@lightblue,densely dashed,every mark/.append style={solid,fill=gnuplot@lightblue!30!black},mark=otimes*\\%
red!80!white,densely dashed,every mark/.append style={solid,fill=red!40!white},mark=oplus*\\%
}

\graphicspath{{svg_with_latex/}}

==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0003_gc_1.tex <==
1 1.000000e-04 2.083300e-02 1.000000e+02 5.625000e-01 1.000000e+02
2 1.000000e-04 1.041700e-02 1.000000e+02 2.812500e-01 1.000000e+02
4 1.000000e-04 5.208300e-03 1.000000e+02 1.406250e-01 1.000000e+02
8 1.000000e-04 2.604200e-03 1.000000e+02 7.031250e-02 1.000000e+02
16 1.000000e-04 1.302100e-03 1.000000e+02 3.515625e-02 1.000000e+02
32 1.000000e-04 6.510400e-04 2.000000e+02 1.757812e-02 1.000000e+02
64 1.000000e-04 3.255200e-04 1.000000e+02 8.789062e-03 1.000000e+02
128 2.000000e-04 1.627600e-04 1.000000e+02 4.394531e-03 1.000000e+02
256 2.000000e-04 8.138000e-05 1.000000e+02 2.197266e-03 1.000000e+02
512 3.000000e-04 1.831100e-04 1.000000e+02 1.098633e-03 4.500123e+02
1024 3.000000e-04 9.155300e-05 1.333333e+02 5.493164e-04 4.500025e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0003_gc_4.tex <==
1 1.750000e-04 2.083300e-02 8.571429e+01 1.518750e+01
2 1.750000e-04 1.041700e-02 8.571429e+01 7.593750e+00
4 1.750000e-04 5.208300e-03 8.571429e+01 3.796875e+00
8 2.000000e-04 2.604200e-03 8.750000e+01 1.898438e+00
16 2.000000e-04 1.302100e-03 8.750000e+01 9.492188e-01
32 2.500000e-04 6.510400e-04 8.000000e+01 4.746094e-01
64 2.250000e-04 3.255200e-04 8.888889e+01 2.373047e-01
128 2.500000e-04 1.627600e-04 9.000000e+01 1.186523e-01
256 2.500000e-04 8.138000e-05 9.000000e+01 5.932617e-02
512 3.250000e-04 4.069000e-05 1.000000e+02 2.966309e-02
1024 3.250000e-04 2.034500e-05 1.000000e+02 1.483154e-02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0003_ls_1.tex <==
1 1.000000e-04 2.083300e-02
2 1.000000e-04 1.041700e-02
4 1.000000e-04 5.208300e-03
8 1.000000e-04 2.604200e-03
16 1.000000e-04 1.302100e-03
32 2.000000e-04 6.510400e-04
64 1.000000e-04 3.255200e-04
128 2.000000e-04 1.627600e-04
256 2.000000e-04 8.138000e-05
512 3.000000e-04 4.069000e-05
1024 4.000000e-04 2.034500e-05


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0003_ls_4.tex <==
1 1.500000e-04
2 1.500000e-04
4 1.500000e-04
8 1.750000e-04
16 1.750000e-04
32 2.000000e-04
64 2.000000e-04
128 2.250000e-04
256 2.250000e-04
512 3.250000e-04
1024 3.250000e-04


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0004_gc_1.tex <==
1 1.000000e-04 2.083300e-02 1.000000e+02 5.625000e-01 1.000000e+02
2 1.000000e-04 1.041700e-02 1.000000e+02 2.812500e-01 1.000000e+02
4 1.000000e-04 5.208300e-03 1.000000e+02 1.406250e-01 1.000000e+02
8 1.000000e-04 2.604200e-03 1.000000e+02 7.031250e-02 1.000000e+02
16 1.000000e-04 1.302100e-03 1.000000e+02 3.515625e-02 1.000000e+02
32 1.000000e-04 6.510400e-04 1.000000e+02 1.757812e-02 1.000000e+02
64 1.000000e-04 3.255200e-04 2.000000e+02 8.789062e-03 1.000000e+02
128 2.000000e-04 1.627600e-04 1.000000e+02 4.394531e-03 1.000000e+02
256 2.000000e-04 8.138000e-05 1.000000e+02 2.197266e-03 1.000000e+02
512 3.000000e-04 4.069000e-05 1.333333e+02 1.098633e-03 1.000000e+02
1024 3.000000e-04 9.155300e-05 1.000000e+02 5.493164e-04 4.500025e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0004_gc_4.tex <==
1 1.750000e-04 2.083300e-02 8.571429e+01 1.518750e+01
2 1.750000e-04 1.041700e-02 8.571429e+01 7.593750e+00
4 1.750000e-04 5.208300e-03 8.571429e+01 3.796875e+00
8 2.000000e-04 2.604200e-03 8.750000e+01 1.898438e+00
16 2.000000e-04 1.302100e-03 8.750000e+01 9.492188e-01
32 2.750000e-04 2.929700e-03 7.272727e+01 4.746094e-01
64 2.250000e-04 3.255200e-04 8.888889e+01 2.373047e-01
128 2.500000e-04 1.627600e-04 1.000000e+02 1.186523e-01
256 2.500000e-04 8.138000e-05 1.000000e+02 5.932617e-02
512 3.000000e-04 4.069000e-05 9.166667e+01 2.966309e-02
1024 3.000000e-04 2.034500e-05 1.000000e+02 1.483154e-02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0004_ls_1.tex <==
1 1.000000e-04 2.083300e-02
2 1.000000e-04 1.041700e-02
4 1.000000e-04 5.208300e-03
8 1.000000e-04 2.604200e-03
16 1.000000e-04 1.302100e-03
32 1.000000e-04 6.510400e-04
64 2.000000e-04 3.255200e-04
128 2.000000e-04 1.627600e-04
256 2.000000e-04 8.138000e-05
512 4.000000e-04 4.069000e-05
1024 3.000000e-04 2.034500e-05


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0004_ls_4.tex <==
1 1.500000e-04
2 1.500000e-04
4 1.500000e-04
8 1.750000e-04
16 1.750000e-04
32 2.000000e-04
64 2.000000e-04
128 2.500000e-04
256 2.500000e-04
512 2.750000e-04
1024 3.000000e-04


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0005_gc_1.tex <==
1 6.250000e-04 5.699600e-01 1.120000e+02 4.093750e+01 1.597422e+02
2 7.750000e-04 3.535900e-01 1.083871e+02 2.046875e+01 1.329686e+02
4 8.000000e-04 2.169700e-01 1.100000e+02 1.023438e+01 9.852868e+01
8 8.250000e-04 1.136500e-01 1.090909e+02 5.117188e+00 9.031310e+01
16 8.750000e-04 5.821300e-02 1.028571e+02 2.558594e+00 9.252054e+01
32 1.075000e-03 2.910600e-02 1.283721e+02 1.279297e+00 8.921653e+01
64 9.250000e-04 1.455300e-02 1.145946e+02 6.396484e-01 8.921653e+01
128 1.025000e-03 7.276600e-03 1.073171e+02 3.198242e-01 8.921666e+01
256 8.500000e-04 3.638300e-03 1.223529e+02 1.599121e-01 8.921557e+01
512 1.075000e-03 1.819100e-03 1.134884e+02 7.995605e-02 8.921530e+01
1024 9.750000e-04 9.095700e-04 1.230769e+02 3.997803e-02 8.921726e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0005_gc_4.tex <==
1 1.625000e-03 5.699600e-01 7.846154e+01 1.928688e+03
2 1.650000e-03 3.535900e-01 8.333333e+01 9.643438e+02
4 1.725000e-03 2.169700e-01 8.115942e+01 4.821719e+02
8 1.700000e-03 1.136500e-01 8.382353e+01 2.410859e+02
16 1.725000e-03 5.821300e-02 8.550725e+01 1.205430e+02
32 2.025000e-03 2.910600e-02 9.753086e+01 6.027148e+01
64 1.800000e-03 1.455300e-02 8.750000e+01 3.013574e+01
128 1.950000e-03 7.276600e-03 9.615385e+01 1.506787e+01
256 1.775000e-03 3.638300e-03 8.873239e+01 7.533936e+00
512 1.800000e-03 1.819100e-03 9.722222e+01 3.766968e+00
1024 1.850000e-03 9.095700e-04 9.054054e+01 1.883484e+00


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0005_ls_1.tex <==
1 7.000000e-04 3.568000e-01
2 8.400000e-04 2.659200e-01
4 8.800000e-04 2.202100e-01
8 9.000000e-04 1.258400e-01
16 9.000000e-04 6.291900e-02
32 1.380000e-03 3.262400e-02
64 1.060000e-03 1.631200e-02
128 1.100000e-03 8.156100e-03
256 1.040000e-03 4.078100e-03
512 1.220000e-03 2.039000e-03
1024 1.200000e-03 1.019500e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0005_ls_4.tex <==
1 1.275000e-03
2 1.375000e-03
4 1.400000e-03
8 1.425000e-03
16 1.475000e-03
32 1.975000e-03
64 1.575000e-03
128 1.875000e-03
256 1.575000e-03
512 1.750000e-03
1024 1.675000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0006_gc_1.tex <==
1 9.000000e-04 8.327000e-01 1.044444e+02 2.033958e+02 1.896984e+02
2 1.000000e-03 7.020200e-01 1.080000e+02 1.016979e+02 2.043310e+02
4 1.100000e-03 5.227000e-01 1.145455e+02 5.084896e+01 1.848760e+02
8 1.175000e-03 3.588700e-01 1.140426e+02 2.542448e+01 1.586586e+02
16 1.175000e-03 2.072800e-01 1.140426e+02 1.271224e+01 1.181150e+02
32 1.425000e-03 1.178600e-01 1.150877e+02 6.356120e+00 8.568521e+01
64 1.350000e-03 6.011100e-02 1.037037e+02 3.178060e+00 8.976748e+01
128 1.350000e-03 3.005500e-02 1.140741e+02 1.589030e+00 8.504046e+01
256 1.350000e-03 1.533400e-02 1.051852e+02 7.945150e-01 8.436400e+01
512 1.600000e-03 7.667200e-03 1.125000e+02 3.972575e-01 8.436805e+01
1024 1.325000e-03 3.833600e-03 1.162264e+02 1.986287e-01 8.436805e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0006_gc_4.tex <==
1 3.675000e-03 8.327000e-01 8.503401e+01 1.062652e+04
2 3.000000e-03 7.020200e-01 8.583333e+01 5.313260e+03
4 2.575000e-03 5.227000e-01 8.737864e+01 2.656630e+03
8 2.525000e-03 3.588700e-01 8.712871e+01 1.328315e+03
16 2.425000e-03 2.072800e-01 8.453608e+01 6.641576e+02
32 2.600000e-03 1.178600e-01 8.076923e+01 3.320788e+02
64 2.450000e-03 6.011100e-02 8.571429e+01 1.660394e+02
128 2.425000e-03 3.005500e-02 9.175258e+01 8.301969e+01
256 2.350000e-03 1.533400e-02 8.936170e+01 4.150985e+01
512 2.625000e-03 7.667200e-03 9.333333e+01 2.075492e+01
1024 2.400000e-03 3.833600e-03 9.062500e+01 1.037746e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0006_ls_1.tex <==
1 9.400000e-04 4.389600e-01
2 1.080000e-03 3.435700e-01
4 1.260000e-03 2.827300e-01
8 1.340000e-03 2.261900e-01
16 1.340000e-03 1.754900e-01
32 1.640000e-03 1.375500e-01
64 1.400000e-03 6.696300e-02
128 1.540000e-03 3.534200e-02
256 1.420000e-03 1.817600e-02
512 1.800000e-03 9.087800e-03
1024 1.540000e-03 4.543900e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0006_ls_4.tex <==
1 3.125000e-03
2 2.575000e-03
4 2.250000e-03
8 2.200000e-03
16 2.050000e-03
32 2.100000e-03
64 2.100000e-03
128 2.225000e-03
256 2.100000e-03
512 2.450000e-03
1024 2.175000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0007_gc_1.tex <==
1 1.550000e-03 9.568600e-01 9.935484e+01 1.000854e+03 1.785586e+02
2 1.550000e-03 9.105600e-01 1.019355e+02 5.004271e+02 2.373723e+02
4 1.575000e-03 8.356800e-01 1.092063e+02 2.502135e+02 2.438233e+02
8 1.575000e-03 7.217200e-01 1.130159e+02 1.251068e+02 2.305520e+02
16 1.800000e-03 5.475100e-01 1.022222e+02 6.255339e+01 2.106780e+02
32 2.100000e-03 3.826000e-01 9.809524e+01 3.127669e+01 1.638895e+02
64 1.825000e-03 2.335000e-01 1.128767e+02 1.563835e+01 1.169722e+02
128 1.825000e-03 1.323200e-01 1.194521e+02 7.819173e+00 8.261738e+01
256 1.750000e-03 6.843900e-02 1.085714e+02 3.909587e+00 7.353813e+01
512 2.050000e-03 3.482000e-02 1.209756e+02 1.954793e+00 7.280559e+01
1024 1.800000e-03 1.741000e-02 1.111111e+02 9.773966e-01 7.280559e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0007_gc_4.tex <==
1 1.232500e-02 9.073100e-01 9.148073e+01 5.512835e+04
2 7.600000e-03 9.105600e-01 1.072368e+02 2.756418e+04
4 5.300000e-03 8.356800e-01 1.014151e+02 1.378209e+04
8 4.450000e-03 7.217200e-01 8.651685e+01 6.891044e+03
16 3.850000e-03 5.475100e-01 8.311688e+01 3.445522e+03
32 3.725000e-03 3.826000e-01 8.456376e+01 1.722761e+03
64 3.525000e-03 2.335000e-01 9.007092e+01 8.613805e+02
128 3.450000e-03 1.323200e-01 8.550725e+01 4.306903e+02
256 3.050000e-03 6.843900e-02 8.688525e+01 2.153451e+02
512 3.600000e-03 3.482000e-02 9.930556e+01 1.076726e+02
1024 3.150000e-03 1.741000e-02 8.809524e+01 5.383628e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0007_ls_1.tex <==
1 1.540000e-03 5.358800e-01
2 1.580000e-03 3.836000e-01
4 1.720000e-03 3.427400e-01
8 1.780000e-03 3.130400e-01
16 1.840000e-03 2.598800e-01
32 2.060000e-03 2.334500e-01
64 2.060000e-03 1.996200e-01
128 2.180000e-03 1.601600e-01
256 1.900000e-03 9.306600e-02
512 2.480000e-03 4.782600e-02
1024 2.000000e-03 2.391300e-02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0007_ls_4.tex <==
1 1.127500e-02
2 8.150000e-03
4 5.375000e-03
8 3.850000e-03
16 3.200000e-03
32 3.150000e-03
64 3.175000e-03
128 2.950000e-03
256 2.650000e-03
512 3.575000e-03
1024 2.775000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0008_gc_1.tex <==
1 5.125000e-03 9.935300e-01 9.717073e+01 6.605479e+03 1.788275e+02
2 3.375000e-03 9.845800e-01 1.131852e+02 3.302740e+03 2.276591e+02
4 2.675000e-03 9.695500e-01 1.121495e+02 1.651370e+03 2.406010e+02
8 2.350000e-03 9.383100e-01 1.157447e+02 8.256849e+02 2.583239e+02
16 2.525000e-03 8.806100e-01 1.053465e+02 4.128424e+02 2.678091e+02
32 2.900000e-03 7.912700e-01 9.517241e+01 2.064212e+02 2.716154e+02
64 3.025000e-03 6.461300e-01 8.595041e+01 1.032106e+02 2.405726e+02
128 3.750000e-03 4.831700e-01 8.000000e+01 5.160531e+01 1.922682e+02
256 2.700000e-03 3.102100e-01 1.185185e+02 2.580265e+01 1.344414e+02
512 2.925000e-03 1.796000e-01 1.169231e+02 1.290133e+01 9.906779e+01
1024 2.275000e-03 1.018600e-01 1.178022e+02 6.450663e+00 7.063310e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0008_gc_4.tex <==
1 8.500000e-02 9.992200e-01 1.054706e+02 3.870539e+05
2 4.247500e-02 9.845800e-01 1.174809e+02 1.935269e+05
4 2.167500e-02 9.695500e-01 1.197232e+02 9.676346e+04
8 1.230000e-02 9.383100e-01 1.241870e+02 4.838173e+04
16 8.200000e-03 8.806100e-01 1.210366e+02 2.419087e+04
32 6.400000e-03 7.912700e-01 1.058594e+02 1.209543e+04
64 5.525000e-03 6.461300e-01 9.276018e+01 6.047716e+03
128 4.850000e-03 4.831700e-01 9.690722e+01 3.023858e+03
256 4.350000e-03 3.102100e-01 1.063218e+02 1.511929e+03
512 4.950000e-03 1.796000e-01 1.055556e+02 7.559646e+02
1024 4.250000e-03 1.018600e-01 8.764706e+01 3.779823e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0008_ls_1.tex <==
1 4.980000e-03 5.555800e-01
2 3.820000e-03 4.324800e-01
4 3.000000e-03 4.029700e-01
8 2.720000e-03 3.632300e-01
16 2.660000e-03 3.288200e-01
32 2.760000e-03 2.913200e-01
64 2.600000e-03 2.685800e-01
128 3.000000e-03 2.513000e-01
256 3.200000e-03 2.307400e-01
512 3.420000e-03 1.812900e-01
1024 2.680000e-03 1.442100e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0008_ls_4.tex <==
1 8.965000e-02
2 4.990000e-02
4 2.595000e-02
8 1.527500e-02
16 9.925000e-03
32 6.775000e-03
64 5.125000e-03
128 4.700000e-03
256 4.625000e-03
512 5.225000e-03
1024 3.725000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0009_gc_1.tex <==
1 2.582500e-02 9.313600e-01 1.206583e+02 4.869377e+04 1.681641e+02
2 1.505000e-02 9.977100e-01 1.330233e+02 2.434689e+04 2.300143e+02
4 9.175000e-03 9.953500e-01 1.270845e+02 1.217344e+04 2.448766e+02
8 6.025000e-03 9.902200e-01 1.221577e+02 6.086721e+03 2.693890e+02
16 4.350000e-03 9.799700e-01 1.177011e+02 3.043361e+03 2.895721e+02
32 3.975000e-03 9.615000e-01 1.076730e+02 1.521680e+03 3.212067e+02
64 3.875000e-03 9.239800e-01 1.063226e+02 7.608402e+02 3.207930e+02
128 5.225000e-03 8.271600e-01 8.191388e+01 3.804201e+02 2.974647e+02
256 5.425000e-03 7.562200e-01 7.926267e+01 1.902100e+02 2.760935e+02
512 5.625000e-03 5.988500e-01 7.466667e+01 9.510502e+01 2.257852e+02
1024 4.875000e-03 4.316700e-01 9.558974e+01 4.755251e+01 1.743487e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0009_gc_4.tex <==
1 6.017000e-01 9.989300e-01 1.202260e+02 2.974569e+06
2 3.058500e-01 9.977100e-01 1.363413e+02 1.487285e+06
4 1.566750e-01 9.995500e-01 1.371629e+02 7.436423e+05
8 7.990000e-02 9.902200e-01 1.465269e+02 3.718211e+05
16 4.105000e-02 9.799700e-01 1.493910e+02 1.859106e+05
32 2.225000e-02 9.013700e-01 1.596629e+02 9.295528e+04
64 1.320000e-02 9.239800e-01 1.518939e+02 4.647764e+04
128 9.100000e-03 8.579800e-01 1.324176e+02 2.323882e+04
256 7.050000e-03 7.562200e-01 1.163121e+02 1.161941e+04
512 6.375000e-03 5.988500e-01 1.105882e+02 5.809705e+03
1024 5.475000e-03 4.316700e-01 1.210046e+02 2.904853e+03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0009_ls_1.tex <==
1 3.116000e-02 5.538400e-01
2 2.002000e-02 4.337600e-01
4 1.166000e-02 4.064700e-01
8 7.360000e-03 3.675800e-01
16 5.120000e-03 3.384200e-01
32 4.280000e-03 2.993400e-01
64 4.120000e-03 2.880300e-01
128 4.280000e-03 2.780700e-01
256 4.300000e-03 2.739000e-01
512 4.200000e-03 2.652300e-01
1024 4.660000e-03 2.475900e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0009_ls_4.tex <==
1 7.234000e-01
2 4.170000e-01
4 2.149000e-01
8 1.170750e-01
16 6.132500e-02
32 3.552500e-02
64 2.005000e-02
128 1.205000e-02
256 8.200000e-03
512 7.050000e-03
1024 6.625000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0010_gc_1.tex <==
1 1.763750e-01 9.617200e-01 1.279887e+02 3.747775e+05 1.737368e+02
2 8.867500e-02 9.996700e-01 1.546772e+02 1.873888e+05 2.306576e+02
4 4.637500e-02 8.682400e-01 1.615526e+02 9.369438e+04 2.144173e+02
8 2.547500e-02 9.074600e-01 1.718548e+02 4.684719e+04 2.480348e+02
16 1.572500e-02 9.972000e-01 1.597456e+02 2.342360e+04 2.977783e+02
32 1.050000e-02 9.944200e-01 1.485714e+02 1.171180e+04 3.316060e+02
64 7.825000e-03 9.987600e-01 1.216613e+02 5.855899e+03 3.487169e+02
128 7.050000e-03 9.770800e-01 9.957447e+01 2.927949e+03 3.507107e+02
256 6.325000e-03 9.564600e-01 8.442688e+01 1.463975e+03 3.467696e+02
512 6.525000e-03 9.136200e-01 9.134100e+01 7.319873e+02 3.322013e+02
1024 7.375000e-03 8.445800e-01 7.810169e+01 3.659937e+02 3.090869e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0010_gc_4.tex <==
8 5.725500e-01 9.986700e-01 1.644660e+02 2.927377e+06
16 2.911250e-01 9.744200e-01 1.750537e+02 1.463688e+06
32 1.509000e-01 9.661600e-01 2.003148e+02 7.318442e+05
64 7.737500e-02 9.532500e-01 2.094023e+02 3.659221e+05
128 4.102500e-02 9.388500e-01 2.009750e+02 1.829610e+05
256 2.245000e-02 9.105600e-01 1.828508e+02 9.148052e+04
512 1.412500e-02 8.858500e-01 1.695575e+02 4.574026e+04
1024 1.010000e-02 8.445800e-01 1.381188e+02 2.287013e+04


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0010_ls_1.tex <==
1 2.257400e-01 5.535500e-01
2 1.371600e-01 4.334000e-01
4 7.492000e-02 4.049300e-01
8 4.378000e-02 3.658600e-01
16 2.512000e-02 3.348800e-01
32 1.560000e-02 2.998800e-01
64 9.520000e-03 2.864100e-01
128 7.020000e-03 2.786000e-01
256 5.340000e-03 2.758200e-01
512 5.960000e-03 2.750200e-01
1024 5.760000e-03 2.732500e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0010_ls_4.tex <==
8 9.416500e-01
16 5.096250e-01
32 3.022750e-01
64 1.620250e-01
128 8.245000e-02
256 4.105000e-02
512 2.395000e-02
1024 1.395000e-02


==> global-coarsening-paper-data/gmg-scaling/hmg-annulus/data_0011_ls_1.tex <==
8 3.135400e-01 3.660900e-01
16 1.705400e-01 3.354100e-01
32 9.988000e-02 3.000900e-01
64 5.526000e-02 2.869100e-01
128 3.124000e-02 2.788300e-01
256 1.802000e-02 2.764000e-01
512 1.356000e-02 2.756900e-01
1024 8.340000e-03 2.755400e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0003_gc_1.tex <==
1 2.750000e-04 1.200000e-01 1.181818e+02 4.645833e+00 7.568113e+01
2 2.750000e-04 6.000000e-02 1.272727e+02 2.322917e+00 7.567922e+01
4 2.750000e-04 3.000000e-02 1.272727e+02 1.161458e+00 7.567922e+01
8 3.000000e-04 1.500000e-02 1.416667e+02 5.807292e-01 7.567731e+01
16 3.000000e-04 7.500000e-03 1.333333e+02 2.903646e-01 7.567884e+01
32 3.000000e-04 3.750000e-03 1.333333e+02 1.451823e-01 7.567808e+01
64 3.250000e-04 1.875000e-03 1.461538e+02 7.259115e-02 7.567808e+01
128 3.500000e-04 9.375000e-04 1.357143e+02 3.629557e-02 7.567808e+01
256 3.500000e-04 4.687500e-04 1.857143e+02 1.814779e-02 7.567930e+01
512 3.750000e-04 2.343700e-04 1.666667e+02 9.073893e-03 7.567646e+01
1024 4.250000e-04 1.171900e-04 1.470588e+02 4.536947e-03 7.567969e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0003_gc_4.tex <==
1 6.250000e-04 1.200000e-01 9.600000e+01 1.936458e+02
2 6.250000e-04 6.000000e-02 1.040000e+02 9.682292e+01
4 6.250000e-04 3.000000e-02 1.000000e+02 4.841146e+01
8 6.500000e-04 1.500000e-02 1.000000e+02 2.420573e+01
16 6.500000e-04 7.500000e-03 9.615385e+01 1.210286e+01
32 6.500000e-04 3.750000e-03 1.000000e+02 6.051432e+00
64 6.500000e-04 1.875000e-03 1.076923e+02 3.025716e+00
128 7.250000e-04 9.375000e-04 9.655172e+01 1.512858e+00
256 7.250000e-04 4.687500e-04 1.103448e+02 7.564290e-01
512 7.500000e-04 2.343700e-04 1.300000e+02 3.782145e-01
1024 7.500000e-04 1.171900e-04 1.133333e+02 1.891073e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0003_ls_1.tex <==
1 3.250000e-04 1.585600e-01
2 3.500000e-04 7.928200e-02
4 3.500000e-04 3.964100e-02
8 4.250000e-04 1.982100e-02
16 4.000000e-04 9.910300e-03
32 4.000000e-04 4.955200e-03
64 4.750000e-04 2.477600e-03
128 4.750000e-04 1.238800e-03
256 6.500000e-04 6.193900e-04
512 6.250000e-04 3.097000e-04
1024 6.250000e-04 1.548500e-04


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0003_ls_4.tex <==
1 6.000000e-04
2 6.500000e-04
4 6.250000e-04
8 6.500000e-04
16 6.250000e-04
32 6.500000e-04
64 7.000000e-04
128 7.000000e-04
256 8.000000e-04
512 9.750000e-04
1024 8.500000e-04


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0004_gc_1.tex <==
1 4.250000e-04 4.000900e-01 1.411765e+02 2.100000e+01 1.006972e+02
2 4.500000e-04 2.445000e-01 1.333333e+02 1.050000e+01 7.325843e+01
4 4.500000e-04 1.294400e-01 1.388889e+02 5.250000e+00 6.825924e+01
8 4.500000e-04 6.668200e-02 1.444444e+02 2.625000e+00 6.393289e+01
16 4.750000e-04 3.334100e-02 1.421053e+02 1.312500e+00 6.073816e+01
32 4.750000e-04 1.667100e-02 1.578947e+02 6.562500e-01 6.073888e+01
64 5.250000e-04 8.335300e-03 1.666667e+02 3.281250e-01 6.073963e+01
128 5.000000e-04 4.167700e-03 1.500000e+02 1.640625e-01 6.073948e+01
256 5.500000e-04 2.083800e-03 1.545455e+02 8.203125e-02 6.073802e+01
512 6.000000e-04 1.041900e-03 1.875000e+02 4.101562e-02 6.073802e+01
1024 5.750000e-04 5.209600e-04 1.608696e+02 2.050781e-02 6.073919e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0004_gc_4.tex <==
1 1.100000e-03 4.000900e-01 8.409091e+01 1.053188e+03
2 1.075000e-03 2.445000e-01 8.372093e+01 5.265938e+02
4 1.075000e-03 1.294400e-01 8.837209e+01 2.632969e+02
8 1.125000e-03 6.668200e-02 9.111111e+01 1.316484e+02
16 1.100000e-03 3.334100e-02 1.000000e+02 6.582422e+01
32 1.125000e-03 1.667100e-02 1.000000e+02 3.291211e+01
64 1.075000e-03 8.335300e-03 1.116279e+02 1.645605e+01
128 1.175000e-03 4.167700e-03 1.021277e+02 8.228027e+00
256 1.225000e-03 2.083800e-03 1.020408e+02 4.114014e+00
512 1.200000e-03 1.041900e-03 1.083333e+02 2.057007e+00
1024 1.150000e-03 5.209600e-04 1.152174e+02 1.028503e+00


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0004_ls_1.tex <==
1 6.000000e-04 3.973200e-01
2 6.000000e-04 3.337500e-01
4 6.250000e-04 1.896300e-01
8 6.500000e-04 1.043000e-01
16 6.750000e-04 5.489300e-02
32 7.500000e-04 2.744700e-02
64 8.750000e-04 1.372300e-02
128 7.500000e-04 6.861600e-03
256 8.500000e-04 3.430800e-03
512 1.125000e-03 1.715400e-03
1024 9.250000e-04 8.577000e-04


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0004_ls_4.tex <==
1 9.250000e-04
2 9.000000e-04
4 9.500000e-04
8 1.025000e-03
16 1.100000e-03
32 1.125000e-03
64 1.200000e-03
128 1.200000e-03
256 1.250000e-03
512 1.300000e-03
1024 1.325000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0005_gc_1.tex <==
1 6.750000e-04 7.822400e-01 1.296296e+02 1.188125e+02 1.736189e+02
2 7.000000e-04 6.291900e-01 1.321429e+02 5.940625e+01 1.536709e+02
4 7.750000e-04 4.385300e-01 1.225806e+02 2.970312e+01 1.203926e+02
8 7.250000e-04 2.894300e-01 1.379310e+02 1.485156e+01 9.906897e+01
16 7.250000e-04 1.682700e-01 1.310345e+02 7.425781e+00 7.439650e+01
32 7.250000e-04 8.824000e-02 1.413793e+02 3.712891e+00 6.292519e+01
64 7.750000e-04 4.412000e-02 1.419355e+02 1.856445e+00 5.537218e+01
128 8.000000e-04 2.206000e-02 1.406250e+02 9.282227e-01 5.033886e+01
256 9.000000e-04 1.103000e-02 1.722222e+02 4.641113e-01 5.033771e+01
512 8.750000e-04 5.515000e-03 1.400000e+02 2.320557e-01 5.033771e+01
1024 8.500000e-04 2.757500e-03 1.529412e+02 1.160278e-01 5.033863e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0005_gc_4.tex <==
1 2.366667e-03 7.822400e-01 9.823944e+01 6.692562e+03
2 1.966667e-03 6.291900e-01 9.025424e+01 3.346281e+03
4 1.833333e-03 6.891100e-01 9.272727e+01 1.673141e+03
8 1.733333e-03 2.894300e-01 9.375000e+01 8.365703e+02
16 1.700000e-03 1.682700e-01 9.117647e+01 4.182852e+02
32 1.666667e-03 8.824000e-02 9.450000e+01 2.091426e+02
64 1.666667e-03 4.412000e-02 1.470000e+02 1.045713e+02
128 1.733333e-03 2.206000e-02 9.663462e+01 5.228564e+01
256 1.766667e-03 1.103000e-02 1.004717e+02 2.614282e+01
512 1.900000e-03 5.515000e-03 9.736842e+01 1.307141e+01
1024 1.700000e-03 2.757500e-03 1.029412e+02 6.535706e+00


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0005_ls_1.tex <==
1 8.750000e-04 4.505500e-01
2 9.250000e-04 4.094400e-01
4 9.500000e-04 3.642500e-01
8 1.000000e-03 2.921500e-01
16 9.500000e-04 2.261800e-01
32 1.025000e-03 1.402300e-01
64 1.100000e-03 7.967900e-02
128 1.125000e-03 4.382300e-02
256 1.550000e-03 2.191200e-02
512 1.225000e-03 1.095600e-02
1024 1.300000e-03 5.477900e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0005_ls_4.tex <==
1 2.325000e-03
2 1.775000e-03
4 1.700000e-03
8 1.625000e-03
16 1.550000e-03
32 1.575000e-03
64 2.450000e-03
128 1.675000e-03
256 1.775000e-03
512 1.850000e-03
1024 1.750000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0006_gc_1.tex <==
1 1.400000e-03 9.611400e-01 1.178571e+02 8.000417e+02 1.859791e+02
2 1.200000e-03 9.162100e-01 1.291667e+02 4.000208e+02 1.911758e+02
4 1.150000e-03 8.395600e-01 1.260870e+02 2.000104e+02 1.834663e+02
8 1.125000e-03 7.216800e-01 1.288889e+02 1.000052e+02 1.709049e+02
16 1.125000e-03 5.545500e-01 1.377778e+02 5.000260e+01 1.516117e+02
32 1.175000e-03 3.817600e-01 1.361702e+02 2.500130e+01 1.073113e+02
64 1.275000e-03 2.195100e-01 1.627451e+02 1.250065e+01 9.297725e+01
128 1.275000e-03 1.291200e-01 1.196078e+02 6.250326e+00 6.960647e+01
256 1.500000e-03 6.719700e-02 1.050000e+02 3.125163e+00 5.589038e+01
512 1.375000e-03 3.359800e-02 1.236364e+02 1.562581e+00 4.967987e+01
1024 1.225000e-03 1.679900e-02 1.387755e+02 7.812907e-01 4.347005e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0006_gc_4.tex <==
1 9.233333e-03 9.182100e-01 1.215704e+02 4.802960e+04
2 5.466667e-03 9.142300e-01 1.193598e+02 2.401480e+04
4 3.766667e-03 8.395600e-01 1.134956e+02 1.200740e+04
8 3.200000e-03 8.231600e-01 9.921875e+01 6.003701e+03
16 2.733333e-03 5.545500e-01 9.420732e+01 3.001850e+03
32 2.600000e-03 3.817600e-01 1.028846e+02 1.500925e+03
64 2.700000e-03 2.195100e-01 1.120370e+02 7.504626e+02
128 2.500000e-03 1.291200e-01 9.100000e+01 3.752313e+02
256 2.533333e-03 6.719700e-02 8.881579e+01 1.876156e+02
512 2.366667e-03 3.359800e-02 1.077465e+02 9.380782e+01
1024 2.333333e-03 1.679900e-02 9.857143e+01 4.690391e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0006_ls_1.tex <==
1 1.650000e-03 5.168000e-01
2 1.550000e-03 4.792500e-01
4 1.450000e-03 4.576100e-01
8 1.450000e-03 4.222700e-01
16 1.550000e-03 3.657700e-01
32 1.600000e-03 3.557500e-01
64 2.075000e-03 2.360900e-01
128 1.525000e-03 1.855000e-01
256 1.575000e-03 1.202300e-01
512 1.700000e-03 6.762900e-02
1024 1.700000e-03 3.864500e-02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0006_ls_4.tex <==
1 1.122500e-02
2 6.525000e-03
4 4.275000e-03
8 3.175000e-03
16 2.575000e-03
32 2.675000e-03
64 3.025000e-03
128 2.275000e-03
256 2.250000e-03
512 2.550000e-03
1024 2.300000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0007_gc_1.tex <==
1 3.800000e-03 9.204300e-01 1.453947e+02 5.898104e+03 1.727015e+02
2 2.733333e-03 8.848000e-01 1.371951e+02 2.949052e+03 1.682193e+02
4 2.200000e-03 8.510400e-01 1.375000e+02 1.474526e+03 1.678646e+02
8 1.966667e-03 9.467000e-01 1.296610e+02 7.372630e+02 1.954498e+02
16 1.966667e-03 8.963200e-01 1.144068e+02 3.686315e+02 1.952001e+02
32 2.133333e-03 8.117300e-01 1.019531e+02 1.843158e+02 1.854662e+02
64 2.433333e-03 4.210900e-01 9.143836e+01 9.215788e+01 1.014528e+02
128 2.566667e-03 4.953900e-01 1.071429e+02 4.607894e+01 1.351346e+02
256 2.100000e-03 3.281200e-01 1.333333e+02 2.303947e+01 1.032246e+02
512 2.033333e-03 1.885500e-01 1.487705e+02 1.151973e+01 9.310651e+01
1024 1.733333e-03 1.070600e-01 1.254808e+02 5.759867e+00 6.991902e+01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0007_gc_4.tex <==
1 7.316667e-02 9.582000e-01 1.330182e+02 3.656660e+05
2 3.696667e-02 9.576400e-01 1.297791e+02 1.828330e+05
4 1.806667e-02 9.182100e-01 1.306273e+02 9.141649e+04
8 1.020000e-02 9.156100e-01 1.262255e+02 4.570825e+04
16 6.766667e-03 9.084100e-01 1.174877e+02 2.285412e+04
32 5.333333e-03 8.352100e-01 1.035938e+02 1.142706e+04
64 4.333333e-03 6.605300e-01 1.182692e+02 5.713531e+03
128 3.700000e-03 4.953900e-01 1.114865e+02 2.856765e+03
256 3.666667e-03 3.281200e-01 1.152273e+02 1.428383e+03
512 3.633333e-03 1.885500e-01 1.245413e+02 7.141914e+02
1024 3.466667e-03 1.070600e-01 9.807692e+01 3.570957e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0007_ls_1.tex <==
1 5.525000e-03 5.329600e-01
2 3.750000e-03 5.259800e-01
4 3.025000e-03 5.069800e-01
8 2.550000e-03 4.843700e-01
16 2.250000e-03 4.591800e-01
32 2.175000e-03 4.376700e-01
64 2.225000e-03 4.150600e-01
128 2.750000e-03 3.665900e-01
256 2.800000e-03 3.178700e-01
512 3.025000e-03 2.025100e-01
1024 2.175000e-03 1.531200e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0007_ls_4.tex <==
1 9.732500e-02
2 4.797500e-02
4 2.360000e-02
8 1.287500e-02
16 7.950000e-03
32 5.525000e-03
64 5.125000e-03
128 4.125000e-03
256 4.225000e-03
512 4.525000e-03
1024 3.400000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0008_gc_1.tex <==
1 2.023333e-02 9.390900e-01 1.569193e+02 4.537383e+04 1.496057e+02
2 1.130000e-02 9.584500e-01 1.750000e+02 2.268692e+04 1.797240e+02
4 7.100000e-03 9.201400e-01 1.595070e+02 1.134346e+04 1.754988e+02
8 4.666667e-03 9.197400e-01 1.601786e+02 5.671729e+03 1.766998e+02
16 3.533333e-03 9.189400e-01 1.386792e+02 2.835865e+03 1.810042e+02
32 3.466667e-03 9.671000e-01 1.110577e+02 1.417932e+03 1.997480e+02
64 3.600000e-03 5.576300e-01 9.375000e+01 7.089661e+02 1.202126e+02
128 3.533333e-03 8.719800e-01 1.125000e+02 3.544831e+02 1.943694e+02
256 4.700000e-03 7.718900e-01 9.468085e+01 1.772415e+02 1.845435e+02
512 5.233333e-03 6.199300e-01 8.359873e+01 8.862077e+01 1.610584e+02
1024 4.400000e-03 4.549900e-01 1.068182e+02 4.431038e+01 1.278672e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0008_gc_4.tex <==
1 5.549000e-01 9.585400e-01 1.291404e+02 2.858333e+06
2 2.927667e-01 9.584500e-01 1.398725e+02 1.429167e+06
4 1.484000e-01 9.581900e-01 1.395047e+02 7.145833e+05
8 7.493333e-02 9.577600e-01 1.390569e+02 3.572916e+05
16 3.776667e-02 9.772200e-01 1.388129e+02 1.786458e+05
32 2.043333e-02 9.548800e-01 1.340946e+02 8.932291e+04
64 1.286667e-02 9.324400e-01 1.152202e+02 4.466145e+04
128 8.366667e-03 9.424000e-01 1.117530e+02 2.233073e+04
256 6.600000e-03 9.269900e-01 1.064394e+02 1.116536e+04
512 5.733333e-03 6.199300e-01 1.085756e+02 5.582682e+03
1024 4.766667e-03 4.549900e-01 1.384615e+02 2.791341e+03


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0008_ls_1.tex <==
1 3.175000e-02 6.277100e-01
2 1.977500e-02 5.332900e-01
4 1.132500e-02 5.243000e-01
8 7.475000e-03 5.205100e-01
16 4.900000e-03 5.076900e-01
32 3.850000e-03 4.841600e-01
64 3.375000e-03 4.638700e-01
128 3.975000e-03 4.486200e-01
256 4.450000e-03 4.182700e-01
512 4.375000e-03 3.849100e-01
1024 4.700000e-03 3.558300e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0008_ls_4.tex <==
1 7.166000e-01
2 4.095000e-01
4 2.070250e-01
8 1.042000e-01
16 5.242500e-02
32 2.740000e-02
64 1.482500e-02
128 9.350000e-03
256 7.025000e-03
512 6.225000e-03
1024 6.600000e-03


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0009_gc_1.tex <==
1 1.504667e-01 9.585300e-01 1.271876e+02 3.561329e+05 1.238299e+02
2 7.573333e-02 9.788100e-01 1.518816e+02 1.780664e+05 1.550197e+02
4 3.866667e-02 9.685200e-01 1.797414e+02 8.903322e+04 1.815986e+02
8 2.073333e-02 9.684600e-01 1.870177e+02 4.451661e+04 1.831153e+02
16 1.210000e-02 9.785500e-01 1.849174e+02 2.225831e+04 1.855951e+02
32 8.466667e-03 9.580700e-01 1.567913e+02 1.112915e+04 1.838095e+02
64 7.100000e-03 9.675700e-01 1.207746e+02 5.564576e+03 1.899841e+02
128 5.866667e-03 9.799200e-01 1.052557e+02 2.782288e+03 2.012776e+02
256 5.666667e-03 9.598900e-01 9.397059e+01 1.391144e+03 2.053812e+02
512 5.200000e-03 9.211100e-01 9.951923e+01 6.955721e+02 2.010674e+02
1024 5.233333e-03 8.569000e-01 9.984076e+01 3.477860e+02 1.934879e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0009_gc_4.tex <==
8 5.782000e-01 9.787000e-01 1.445953e+02 2.826665e+06
16 2.927000e-01 9.785500e-01 1.458234e+02 1.413332e+06
32 1.509333e-01 9.783200e-01 1.484927e+02 7.066662e+05
64 8.063333e-02 9.880800e-01 1.544337e+02 3.533331e+05
128 4.290000e-02 9.869900e-01 1.451632e+02 1.766665e+05
256 2.300000e-02 9.741600e-01 1.346739e+02 8.833327e+04
512 1.410000e-02 9.699500e-01 1.202128e+02 4.416664e+04
1024 1.013333e-02 9.500400e-01 1.085526e+02 2.208332e+04


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0009_ls_1.tex <==
1 1.913750e-01 7.740700e-01
2 1.150250e-01 6.314100e-01
4 6.950000e-02 5.333300e-01
8 3.877500e-02 5.288800e-01
16 2.237500e-02 5.272500e-01
32 1.327500e-02 5.212300e-01
64 8.575000e-03 5.092900e-01
128 6.175000e-03 4.868500e-01
256 5.325000e-03 4.673700e-01
512 5.175000e-03 4.581100e-01
1024 5.225000e-03 4.428700e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0009_ls_4.tex <==
8 8.360500e-01
16 4.268250e-01
32 2.241250e-01
64 1.245250e-01
128 6.227500e-02
256 3.097500e-02
512 1.695000e-02
1024 1.100000e-02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0010_gc_1.tex <==
8 2.204000e-01 9.998500e-01 1.226520e+02 3.527983e+05 1.874695e+02
16 7.755000e-02 9.839900e-01 1.801741e+02 1.763992e+05 1.852705e+02
32 4.055000e-02 9.787600e-01 1.854501e+02 8.819958e+04 1.845603e+02
64 2.260000e-02 9.786800e-01 1.899336e+02 4.409979e+04 1.856056e+02
128 1.455000e-02 9.889700e-01 1.671821e+02 2.204990e+04 1.896540e+02
256 1.050000e-02 9.834200e-01 1.414286e+02 1.102495e+04 1.928501e+02
512 1.005000e-02 9.881500e-01 1.072139e+02 5.512474e+03 2.023902e+02
1024 7.450000e-03 9.776700e-01 1.110738e+02 2.756237e+03 2.089262e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0010_gc_4.tex <==
128 3.163667e-01 9.889700e-01 1.631809e+02 1.405642e+06
256 1.690000e-01 9.886200e-01 1.592308e+02 7.028210e+05
512 8.680000e-02 9.879900e-01 1.581509e+02 3.514105e+05
1024 4.546667e-02 9.922200e-01 1.486254e+02 1.757053e+05


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0010_ls_1.tex <==
8 2.703250e-01 5.333400e-01
16 1.397250e-01 5.311100e-01
32 7.520000e-02 5.303200e-01
64 4.292500e-02 5.272900e-01
128 2.432500e-02 5.214600e-01
256 1.485000e-02 5.099400e-01
512 1.077500e-02 4.882400e-01
1024 8.275000e-03 4.679500e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0010_ls_4.tex <==
64 8.900000e-01
128 5.162500e-01
256 2.691000e-01
512 1.372750e-01
1024 6.757500e-02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0011_gc_1.tex <==
256 4.355000e-02 9.892200e-01 1.921929e+02 8.778855e+04 1.875583e+02
512 2.560000e-02 9.944500e-01 1.820312e+02 4.389428e+04 1.906391e+02
1024 1.655000e-02 9.915700e-01 1.690332e+02 2.194714e+04 1.943150e+02


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0011_ls_1.tex <==
256 8.370000e-02 5.274200e-01
512 4.660000e-02 5.216400e-01
1024 2.797500e-02 5.102900e-01


==> global-coarsening-paper-data/gmg-scaling/hmg-quadrant/data_0011_ls_4.tex <==
1024 6.071750e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0003_amg_4.tex <==
1 5.250000e-04 3.125000e-01
2 5.750000e-04 1.562500e-01
4 6.000000e-04 7.812500e-02
8 6.250000e-04 3.906200e-02
16 6.500000e-04 1.953100e-02
32 6.000000e-04 9.765600e-03
64 6.000000e-04 4.882800e-03
128 7.500000e-04 2.441400e-03
256 7.250000e-04 1.220700e-03
512 6.750000e-04 6.103500e-04


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0004_amg_4.tex <==
1 1.250000e-03 7.686400e-01
2 1.350000e-03 6.638300e-01
4 1.375000e-03 4.056700e-01
8 1.400000e-03 2.281900e-01
16 1.400000e-03 1.141000e-01
32 1.450000e-03 5.704800e-02
64 1.425000e-03 2.852400e-02
128 1.500000e-03 1.426200e-02
256 1.425000e-03 7.130900e-03
512 1.400000e-03 3.565500e-03


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0005_amg_4.tex <==
1 2.950000e-03 9.439100e-01
2 2.950000e-03 8.764900e-01
4 3.100000e-03 7.669300e-01
8 2.925000e-03 7.218100e-01
16 2.850000e-03 6.135400e-01
32 2.650000e-03 3.834600e-01
64 2.725000e-03 1.917300e-01
128 2.800000e-03 9.586600e-02
256 2.775000e-03 4.793300e-02
512 2.775000e-03 2.396600e-02


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0006_amg_4.tex <==
1 1.208000e-02 9.974600e-01
2 8.780000e-03 9.879700e-01
4 7.220000e-03 9.826300e-01
8 7.160000e-03 9.468000e-01
16 6.180000e-03 8.739700e-01
32 7.000000e-03 8.115500e-01
64 7.140000e-03 5.979800e-01
128 7.540000e-03 5.680800e-01
256 6.700000e-03 3.550500e-01
512 7.300000e-03 1.775300e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0007_amg_4.tex <==
1 8.738333e-02 9.987500e-01
2 4.565000e-02 9.987500e-01
4 2.638333e-02 9.959200e-01
8 2.073333e-02 9.931100e-01
16 1.835000e-02 9.875300e-01
32 1.590000e-02 9.765600e-01
64 1.556667e-02 9.450500e-01
128 1.596667e-02 8.616700e-01
256 1.748333e-02 7.847300e-01
512 1.898333e-02 6.103500e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0008_amg_4.tex <==
1 6.596857e-01 9.999200e-01
2 3.625143e-01 9.998300e-01
4 1.891429e-01 9.997400e-01
8 1.058571e-01 9.986600e-01
16 6.191429e-02 9.977600e-01
32 4.590000e-02 9.948900e-01
64 3.830000e-02 9.906200e-01
128 4.341667e-02 9.808000e-01
256 4.021429e-02 9.617300e-01
512 3.884286e-02 9.307000e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0009_amg_4.tex <==
8 7.791000e-01 9.999200e-01
16 4.164286e-01 9.999200e-01
32 2.422143e-01 9.996500e-01
64 1.585000e-01 9.988300e-01
128 4.273714e-01 9.977400e-01
256 1.261200e+00 9.948500e-01
512 1.042200e+00 9.905500e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant-amg/data_0010_amg_4.tex <==
128 1.743875e+00 9.996800e-01
256 2.684862e+00 9.993100e-01
512 4.596100e+00 9.985800e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0003_gc_4.tex <==
1 7.250000e-04 2.727300e-01 0.000000e+00 1.936458e+02
2 8.000000e-04 1.363600e-01 0.000000e+00 9.682292e+01
4 8.500000e-04 6.818200e-02 0.000000e+00 4.841146e+01
8 9.000000e-04 3.409100e-02 0.000000e+00 2.420573e+01
16 8.750000e-04 1.704500e-02 0.000000e+00 1.210286e+01
32 8.500000e-04 8.522700e-03 0.000000e+00 6.051432e+00
64 8.750000e-04 4.261400e-03 0.000000e+00 3.025716e+00
128 9.750000e-04 2.130700e-03 0.000000e+00 1.512858e+00
256 9.750000e-04 1.065300e-03 0.000000e+00 7.564290e-01
512 9.000000e-04 5.326700e-04 0.000000e+00 3.782145e-01
1024 9.750000e-04 2.663400e-04 0.000000e+00 1.891073e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0003_ls_4.tex <==
1 7.250000e-04 1.585600e-01 0.000000e+00 1.936458e+02
2 8.250000e-04 7.928200e-02 0.000000e+00 9.682292e+01
4 8.000000e-04 3.964100e-02 0.000000e+00 4.841146e+01
8 9.000000e-04 1.982100e-02 0.000000e+00 2.420573e+01
16 8.750000e-04 9.910300e-03 0.000000e+00 1.210286e+01
32 8.750000e-04 4.955200e-03 0.000000e+00 6.051432e+00
64 8.750000e-04 2.477600e-03 0.000000e+00 3.025716e+00
128 1.000000e-03 1.238800e-03 0.000000e+00 1.512858e+00
256 1.050000e-03 6.193900e-04 0.000000e+00 7.564290e-01
512 1.000000e-03 3.097000e-04 0.000000e+00 3.782145e-01
1024 1.225000e-03 1.548500e-04 0.000000e+00 1.891073e-01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0004_gc_4.tex <==
1 1.300000e-03 8.382900e-01 0.000000e+00 1.053188e+03
2 1.250000e-03 4.191500e-01 0.000000e+00 5.265938e+02
4 1.300000e-03 2.750700e-01 0.000000e+00 2.632969e+02
8 1.325000e-03 1.692700e-01 0.000000e+00 1.316484e+02
16 1.350000e-03 9.168800e-02 0.000000e+00 6.582422e+01
32 1.450000e-03 4.584400e-02 0.000000e+00 3.291211e+01
64 1.450000e-03 2.292200e-02 0.000000e+00 1.645605e+01
128 1.525000e-03 1.146100e-02 0.000000e+00 8.228027e+00
256 1.550000e-03 5.730500e-03 0.000000e+00 4.114014e+00
512 1.550000e-03 2.865300e-03 0.000000e+00 2.057007e+00
1024 1.750000e-03 3.438300e-03 0.000000e+00 1.028503e+00


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0004_ls_4.tex <==
1 1.300000e-03 4.070100e-01 0.000000e+00 1.053188e+03
2 1.250000e-03 3.337500e-01 0.000000e+00 5.265938e+02
4 1.300000e-03 1.896300e-01 0.000000e+00 2.632969e+02
8 1.350000e-03 1.043000e-01 0.000000e+00 1.316484e+02
16 1.350000e-03 5.489300e-02 0.000000e+00 6.582422e+01
32 1.475000e-03 2.744700e-02 0.000000e+00 3.291211e+01
64 1.525000e-03 1.372300e-02 0.000000e+00 1.645605e+01
128 1.625000e-03 6.861600e-03 0.000000e+00 8.228027e+00
256 1.800000e-03 3.430800e-03 0.000000e+00 4.114014e+00
512 1.625000e-03 1.715400e-03 0.000000e+00 2.057007e+00
1024 1.800000e-03 8.577000e-04 0.000000e+00 1.028503e+00


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0005_gc_4.tex <==
1 2.275000e-03 6.692000e-01 0.000000e+00 6.692562e+03
2 2.050000e-03 7.327300e-01 0.000000e+00 3.346281e+03
4 1.925000e-03 6.891100e-01 0.000000e+00 1.673141e+03
8 1.900000e-03 3.617800e-01 0.000000e+00 8.365703e+02
16 1.800000e-03 2.679900e-01 0.000000e+00 4.182852e+02
32 1.800000e-03 1.904100e-01 0.000000e+00 2.091426e+02
64 1.925000e-03 1.205900e-01 0.000000e+00 1.045713e+02
128 2.050000e-03 6.957400e-02 0.000000e+00 5.228564e+01
256 2.100000e-03 3.478700e-02 0.000000e+00 2.614282e+01
512 2.000000e-03 1.739300e-02 0.000000e+00 1.307141e+01
1024 2.075000e-03 8.696700e-03 0.000000e+00 6.535706e+00


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0005_ls_4.tex <==
1 2.325000e-03 4.856600e-01 0.000000e+00 6.692562e+03
2 2.050000e-03 4.487500e-01 0.000000e+00 3.346281e+03
4 1.900000e-03 4.249500e-01 0.000000e+00 1.673141e+03
8 1.875000e-03 2.921500e-01 0.000000e+00 8.365703e+02
16 1.750000e-03 2.261800e-01 0.000000e+00 4.182852e+02
32 1.850000e-03 1.402300e-01 0.000000e+00 2.091426e+02
64 1.925000e-03 7.967900e-02 0.000000e+00 1.045713e+02
128 2.125000e-03 4.382300e-02 0.000000e+00 5.228564e+01
256 2.200000e-03 2.191200e-02 0.000000e+00 2.614282e+01
512 2.100000e-03 1.095600e-02 0.000000e+00 1.307141e+01
1024 2.275000e-03 5.477900e-03 0.000000e+00 6.535706e+00


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0006_gc_4.tex <==
1 8.775000e-03 8.531500e-01 0.000000e+00 4.802960e+04
2 5.425000e-03 7.922100e-01 0.000000e+00 2.401480e+04
4 3.775000e-03 8.395600e-01 0.000000e+00 1.200740e+04
8 3.075000e-03 7.216800e-01 0.000000e+00 6.003701e+03
16 2.925000e-03 3.902400e-01 0.000000e+00 3.001850e+03
32 3.300000e-03 3.608400e-01 0.000000e+00 1.500925e+03
64 3.225000e-03 2.485000e-01 0.000000e+00 7.504626e+02
128 2.875000e-03 2.124300e-01 0.000000e+00 3.752313e+02
256 2.675000e-03 1.646300e-01 0.000000e+00 1.876156e+02
512 2.525000e-03 9.684200e-02 0.000000e+00 9.380782e+01
1024 2.825000e-03 5.879700e-02 0.000000e+00 4.690391e+01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0006_ls_4.tex <==
1 8.900000e-03 5.599900e-01 0.000000e+00 4.802960e+04
2 5.425000e-03 5.320200e-01 0.000000e+00 2.401480e+04
4 3.850000e-03 5.054900e-01 0.000000e+00 1.200740e+04
8 3.100000e-03 4.787000e-01 0.000000e+00 6.003701e+03
16 2.825000e-03 4.364600e-01 0.000000e+00 3.001850e+03
32 2.775000e-03 3.934800e-01 0.000000e+00 1.500925e+03
64 2.900000e-03 2.360900e-01 0.000000e+00 7.504626e+02
128 2.775000e-03 1.855000e-01 0.000000e+00 3.752313e+02
256 2.775000e-03 1.202300e-01 0.000000e+00 1.876156e+02
512 2.600000e-03 6.762900e-02 0.000000e+00 9.380782e+01
1024 3.025000e-03 3.864500e-02 0.000000e+00 4.690391e+01


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0007_gc_4.tex <==
1 7.010000e-02 9.582000e-01 0.000000e+00 3.656660e+05
2 3.460000e-02 9.197800e-01 0.000000e+00 1.828330e+05
4 1.670000e-02 9.182100e-01 0.000000e+00 9.141649e+04
8 9.400000e-03 8.807000e-01 0.000000e+00 4.570825e+04
16 6.425000e-03 9.084100e-01 0.000000e+00 2.285412e+04
32 5.400000e-03 8.352100e-01 0.000000e+00 1.142706e+04
64 5.150000e-03 4.210900e-01 0.000000e+00 5.713531e+03
128 5.475000e-03 3.198100e-01 0.000000e+00 2.856765e+03
256 5.725000e-03 2.659500e-01 0.000000e+00 1.428383e+03
512 5.500000e-03 2.070900e-01 0.000000e+00 7.141914e+02
1024 4.175000e-03 1.707100e-01 0.000000e+00 3.570957e+02


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0007_ls_4.tex <==
1 7.122500e-02 5.882600e-01 0.000000e+00 3.656660e+05
2 3.537500e-02 6.098000e-01 0.000000e+00 1.828330e+05
4 1.720000e-02 5.923800e-01 0.000000e+00 9.141649e+04
8 9.475000e-03 5.814500e-01 0.000000e+00 4.570825e+04
16 6.200000e-03 5.444200e-01 0.000000e+00 2.285412e+04
32 4.900000e-03 5.342900e-01 0.000000e+00 1.142706e+04
64 4.250000e-03 4.760500e-01 0.000000e+00 5.713531e+03
128 4.925000e-03 3.665900e-01 0.000000e+00 2.856765e+03
256 5.425000e-03 3.804800e-01 0.000000e+00 1.428383e+03
512 4.550000e-03 2.025100e-01 0.000000e+00 7.141914e+02
1024 4.500000e-03 1.531200e-01 0.000000e+00 3.570957e+02


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0008_gc_4.tex <==
1 5.443000e-01 9.585400e-01 0.000000e+00 2.858333e+06
2 2.771500e-01 9.584500e-01 0.000000e+00 1.429167e+06
4 1.396750e-01 9.581900e-01 0.000000e+00 7.145833e+05
8 6.922500e-02 9.577600e-01 0.000000e+00 3.572916e+05
16 3.442500e-02 9.566100e-01 0.000000e+00 1.786458e+05
32 1.750000e-02 9.357400e-01 0.000000e+00 8.932291e+04
64 1.027500e-02 9.324400e-01 0.000000e+00 4.466145e+04
128 8.975000e-03 9.248300e-01 0.000000e+00 2.233073e+04
256 8.650000e-03 4.321900e-01 0.000000e+00 1.116536e+04
512 7.225000e-03 3.317300e-01 0.000000e+00 5.582682e+03
1024 7.975000e-03 8.550700e-01 0.000000e+00 2.791341e+03


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0008_ls_4.tex <==
1 5.524250e-01 7.303200e-01 0.000000e+00 2.858333e+06
2 2.823250e-01 6.442900e-01 0.000000e+00 1.429167e+06
4 1.423000e-01 6.354400e-01 0.000000e+00 7.145833e+05
8 7.105000e-02 6.296300e-01 0.000000e+00 3.572916e+05
16 3.530000e-02 6.115600e-01 0.000000e+00 1.786458e+05
32 1.790000e-02 5.774300e-01 0.000000e+00 8.932291e+04
64 1.050000e-02 5.640500e-01 0.000000e+00 4.466145e+04
128 8.400000e-03 5.480400e-01 0.000000e+00 2.233073e+04
256 7.150000e-03 5.021400e-01 0.000000e+00 1.116536e+04
512 6.575000e-03 4.282300e-01 0.000000e+00 5.582682e+03
1024 7.450000e-03 3.558300e-01 0.000000e+00 2.791341e+03


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0009_gc_4.tex <==
8 5.416250e-01 9.787000e-01 0.000000e+00 2.826665e+06
16 2.754250e-01 9.785500e-01 0.000000e+00 1.413332e+06
32 1.378500e-01 9.783200e-01 0.000000e+00 7.066662e+05
64 6.937500e-02 9.776400e-01 0.000000e+00 3.533331e+05
128 3.535000e-02 9.765800e-01 0.000000e+00 1.766665e+05
256 1.887500e-02 9.546500e-01 0.000000e+00 8.833327e+04
512 1.182500e-02 9.511900e-01 0.000000e+00 4.416664e+04
1024 1.132500e-02 9.409500e-01 0.000000e+00 2.208332e+04


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0009_ls_4.tex <==
8 5.536250e-01 6.529200e-01 0.000000e+00 2.826665e+06
16 2.816500e-01 6.498500e-01 0.000000e+00 1.413332e+06
32 1.411000e-01 6.869100e-01 0.000000e+00 7.066662e+05
64 7.112500e-02 6.226700e-01 0.000000e+00 3.533331e+05
128 3.625000e-02 5.870700e-01 0.000000e+00 1.766665e+05
256 1.950000e-02 5.949600e-01 0.000000e+00 8.833327e+04
512 1.282500e-02 5.635900e-01 0.000000e+00 4.416664e+04
1024 1.202500e-02 4.928800e-01 0.000000e+00 2.208332e+04


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0010_gc_4.tex <==
256 1.388500e-01 9.886200e-01 0.000000e+00 7.028210e+05
512 7.012500e-02 9.827300e-01 0.000000e+00 3.514105e+05
1024 3.650000e-02 9.764500e-01 0.000000e+00 1.757053e+05


==> global-coarsening-paper-data/gmg-scaling/hpmg-quadrant/data_0010_ls_4.tex <==
128 2.789750e-01 6.467800e-01 0.000000e+00 1.405642e+06
256 1.414000e-01 6.285700e-01 0.000000e+00 7.028210e+05
512 7.217500e-02 6.332800e-01 0.000000e+00 3.514105e+05
1024 3.842500e-02 5.656700e-01 0.000000e+00 1.757053e+05


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0003_0.tex <==
1 1.000000e-04 5.625000e-01 1.000000e+00
2 1.000000e-04 2.812500e-01 1.000000e+00
4 1.000000e-04 1.406250e-01 1.000000e+00
8 1.000000e-04 7.031250e-02 1.000000e+00
16 1.000000e-04 3.515625e-02 1.000000e+00
32 1.000000e-04 1.757812e-02 1.000000e+00
64 3.000000e-04 8.789062e-03 1.000000e+00
128 2.000000e-04 4.394531e-03 1.000000e+00
256 2.000000e-04 2.197266e-03 1.000000e+00
512 3.000000e-04 1.098633e-03 1.000000e+00
1024 3.000000e-04 5.493164e-04 1.000000e+00
2048 4.000000e-04 2.746582e-04 1.000000e+00
3072 4.000000e-04 1.831055e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0003_1.tex <==
1 1.000000e-04 5.625000e-01 1.000000e+00
2 1.000000e-04 2.812500e-01 1.000000e+00
4 1.000000e-04 1.406250e-01 1.000000e+00
8 1.000000e-04 7.031250e-02 1.000000e+00
16 1.000000e-04 3.515625e-02 1.000000e+00
32 2.000000e-04 1.757812e-02 1.000000e+00
64 3.000000e-04 8.789062e-03 1.000000e+00
128 2.000000e-04 4.394531e-03 1.000000e+00
256 2.000000e-04 2.197266e-03 1.000000e+00
512 4.000000e-04 1.098633e-03 1.000000e+00
1024 3.000000e-04 5.493164e-04 1.000000e+00
2048 3.000000e-04 2.746582e-04 1.000000e+00
3072 6.000000e-04 1.831055e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0004_0.tex <==
1 1.000000e-04 5.625000e-01 1.000000e+00
2 1.000000e-04 2.812500e-01 1.000000e+00
4 1.000000e-04 1.406250e-01 1.000000e+00
8 1.000000e-04 7.031250e-02 1.000000e+00
16 1.000000e-04 3.515625e-02 1.000000e+00
32 1.000000e-04 1.757812e-02 1.000000e+00
64 1.000000e-04 8.789062e-03 1.000000e+00
128 2.000000e-04 4.394531e-03 1.000000e+00
256 2.000000e-04 2.197266e-03 1.000000e+00
512 3.000000e-04 1.098633e-03 1.000000e+00
1024 3.000000e-04 5.493164e-04 1.000000e+00
2048 4.000000e-04 2.746582e-04 1.000000e+00
3072 4.000000e-04 1.831055e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0004_1.tex <==
1 1.000000e-04 5.625000e-01 1.000000e+00
2 1.000000e-04 2.812500e-01 1.000000e+00
4 1.000000e-04 1.406250e-01 1.000000e+00
8 1.000000e-04 7.031250e-02 1.000000e+00
16 1.000000e-04 3.515625e-02 1.000000e+00
32 1.000000e-04 1.757812e-02 1.000000e+00
64 3.000000e-04 8.789062e-03 1.000000e+00
128 2.000000e-04 4.394531e-03 1.000000e+00
256 3.000000e-04 2.197266e-03 1.000000e+00
512 3.000000e-04 1.098633e-03 1.000000e+00
1024 3.000000e-04 5.493164e-04 1.000000e+00
2048 3.000000e-04 2.746582e-04 1.000000e+00
3072 4.000000e-04 1.831055e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0005_0.tex <==
1 7.200000e-04 4.093750e+01 5.000000e+00
2 8.200000e-04 2.046875e+01 5.000000e+00
4 9.000000e-04 1.023438e+01 5.000000e+00
8 8.800000e-04 5.117188e+00 5.000000e+00
16 9.200000e-04 2.558594e+00 5.000000e+00
32 9.400000e-04 1.279297e+00 5.000000e+00
64 1.280000e-03 6.396484e-01 5.000000e+00
128 9.600000e-04 3.198242e-01 5.000000e+00
256 1.060000e-03 1.599121e-01 5.000000e+00
512 1.200000e-03 7.995605e-02 5.000000e+00
1024 1.100000e-03 3.997803e-02 5.000000e+00
2048 1.160000e-03 1.998901e-02 5.000000e+00
3072 1.300000e-03 1.332601e-02 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0005_1.tex <==
1 5.750000e-04 4.093750e+01 4.000000e+00
2 6.750000e-04 2.046875e+01 4.000000e+00
4 7.250000e-04 1.023438e+01 4.000000e+00
8 7.250000e-04 5.117188e+00 4.000000e+00
16 7.250000e-04 2.558594e+00 4.000000e+00
32 7.500000e-04 1.279297e+00 4.000000e+00
64 8.750000e-04 6.396484e-01 4.000000e+00
128 8.250000e-04 3.198242e-01 4.000000e+00
256 8.000000e-04 1.599121e-01 4.000000e+00
512 8.500000e-04 7.995605e-02 4.000000e+00
1024 8.250000e-04 3.997803e-02 4.000000e+00
2048 8.250000e-04 1.998901e-02 4.000000e+00
3072 8.750000e-04 1.332601e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0006_0.tex <==
1 1.000000e-03 2.033958e+02 5.000000e+00
2 1.100000e-03 1.016979e+02 5.000000e+00
4 1.300000e-03 5.084896e+01 5.000000e+00
8 1.300000e-03 2.542448e+01 5.000000e+00
16 1.340000e-03 1.271224e+01 5.000000e+00
32 1.300000e-03 6.356120e+00 5.000000e+00
64 1.500000e-03 3.178060e+00 5.000000e+00
128 1.380000e-03 1.589030e+00 5.000000e+00
256 1.360000e-03 7.945150e-01 5.000000e+00
512 1.540000e-03 3.972575e-01 5.000000e+00
1024 1.480000e-03 1.986287e-01 5.000000e+00
2048 1.460000e-03 9.931437e-02 5.000000e+00
3072 1.500000e-03 6.620958e-02 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0006_1.tex <==
1 8.750000e-04 2.033958e+02 4.000000e+00
2 9.250000e-04 1.016979e+02 4.000000e+00
4 1.000000e-03 5.084896e+01 4.000000e+00
8 1.025000e-03 2.542448e+01 4.000000e+00
16 1.050000e-03 1.271224e+01 4.000000e+00
32 1.050000e-03 6.356120e+00 4.000000e+00
64 1.000000e-03 3.178060e+00 4.000000e+00
128 1.050000e-03 1.589030e+00 4.000000e+00
256 1.025000e-03 7.945150e-01 4.000000e+00
512 1.100000e-03 3.972575e-01 4.000000e+00
1024 1.050000e-03 1.986287e-01 4.000000e+00
2048 1.075000e-03 9.931437e-02 4.000000e+00
3072 1.075000e-03 6.620958e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0007_0.tex <==
1 1.580000e-03 1.000854e+03 5.000000e+00
2 1.720000e-03 5.004271e+02 5.000000e+00
4 1.800000e-03 2.502135e+02 5.000000e+00
8 1.840000e-03 1.251068e+02 5.000000e+00
16 1.860000e-03 6.255339e+01 5.000000e+00
32 1.900000e-03 3.127669e+01 5.000000e+00
64 1.860000e-03 1.563835e+01 5.000000e+00
128 1.880000e-03 7.819173e+00 5.000000e+00
256 1.820000e-03 3.909587e+00 5.000000e+00
512 1.980000e-03 1.954793e+00 5.000000e+00
1024 1.820000e-03 9.773966e-01 5.000000e+00
2048 1.820000e-03 4.886983e-01 5.000000e+00
3072 1.920000e-03 3.257989e-01 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0007_1.tex <==
1 1.625000e-03 1.000854e+03 4.000000e+00
2 1.475000e-03 5.004271e+02 4.000000e+00
4 1.400000e-03 2.502135e+02 4.000000e+00
8 1.375000e-03 1.251068e+02 4.000000e+00
16 1.500000e-03 6.255339e+01 4.000000e+00
32 1.500000e-03 3.127669e+01 4.000000e+00
64 1.600000e-03 1.563835e+01 4.000000e+00
128 1.450000e-03 7.819173e+00 4.000000e+00
256 1.375000e-03 3.909587e+00 4.000000e+00
512 1.500000e-03 1.954793e+00 4.000000e+00
1024 1.425000e-03 9.773966e-01 4.000000e+00
2048 1.475000e-03 4.886983e-01 4.000000e+00
3072 1.500000e-03 3.257989e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0008_0.tex <==
1 5.060000e-03 6.605479e+03 5.000000e+00
2 4.120000e-03 3.302740e+03 5.000000e+00
4 3.200000e-03 1.651370e+03 5.000000e+00
8 2.800000e-03 8.256849e+02 5.000000e+00
16 2.640000e-03 4.128424e+02 5.000000e+00
32 2.580000e-03 2.064212e+02 5.000000e+00
64 2.480000e-03 1.032106e+02 5.000000e+00
128 2.700000e-03 5.160531e+01 5.000000e+00
256 3.040000e-03 2.580265e+01 5.000000e+00
512 3.040000e-03 1.290133e+01 5.000000e+00
1024 2.620000e-03 6.450663e+00 5.000000e+00
2048 2.460000e-03 3.225332e+00 5.000000e+00
3072 2.560000e-03 2.150221e+00 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0008_1.tex <==
1 5.250000e-03 6.605479e+03 4.000000e+00
2 3.375000e-03 3.302740e+03 4.000000e+00
4 2.575000e-03 1.651370e+03 4.000000e+00
8 2.200000e-03 8.256849e+02 4.000000e+00
16 2.125000e-03 4.128424e+02 4.000000e+00
32 1.950000e-03 2.064212e+02 4.000000e+00
64 1.950000e-03 1.032106e+02 4.000000e+00
128 2.075000e-03 5.160531e+01 4.000000e+00
256 2.175000e-03 2.580265e+01 4.000000e+00
512 2.100000e-03 1.290133e+01 4.000000e+00
1024 1.975000e-03 6.450663e+00 4.000000e+00
2048 2.025000e-03 3.225332e+00 4.000000e+00
3072 2.100000e-03 2.150221e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0009_0.tex <==
1 2.990000e-02 4.869377e+04 5.000000e+00
2 2.124000e-02 2.434689e+04 5.000000e+00
4 1.242000e-02 1.217344e+04 5.000000e+00
8 7.560000e-03 6.086721e+03 5.000000e+00
16 5.240000e-03 3.043361e+03 5.000000e+00
32 4.160000e-03 1.521680e+03 5.000000e+00
64 7.460000e-03 7.608402e+02 5.000000e+00
128 3.660000e-03 3.804201e+02 5.000000e+00
256 3.800000e-03 1.902100e+02 5.000000e+00
512 4.440000e-03 9.510502e+01 5.000000e+00
1024 4.300000e-03 4.755251e+01 5.000000e+00
2048 3.940000e-03 2.377626e+01 5.000000e+00
3072 3.520000e-03 1.585084e+01 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0009_1.tex <==
1 2.687500e-02 4.869377e+04 4.000000e+00
2 1.512500e-02 2.434689e+04 4.000000e+00
4 8.725000e-03 1.217344e+04 4.000000e+00
8 5.400000e-03 6.086721e+03 4.000000e+00
16 3.825000e-03 3.043361e+03 4.000000e+00
32 3.050000e-03 1.521680e+03 4.000000e+00
64 3.850000e-03 7.608402e+02 4.000000e+00
128 2.500000e-03 3.804201e+02 4.000000e+00
256 2.625000e-03 1.902100e+02 4.000000e+00
512 2.925000e-03 9.510502e+01 4.000000e+00
1024 3.525000e-03 4.755251e+01 4.000000e+00
2048 3.800000e-03 2.377626e+01 4.000000e+00
3072 3.450000e-03 1.585084e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0010_0.tex <==
1 2.198200e-01 3.747775e+05 5.000000e+00
2 1.374400e-01 1.873888e+05 5.000000e+00
4 7.746000e-02 9.369438e+04 5.000000e+00
8 4.326000e-02 4.684719e+04 5.000000e+00
16 2.494000e-02 2.342360e+04 5.000000e+00
32 1.520000e-02 1.171180e+04 5.000000e+00
64 9.460000e-03 5.855899e+03 5.000000e+00
128 6.540000e-03 2.927949e+03 5.000000e+00
256 5.360000e-03 1.463975e+03 5.000000e+00
512 5.160000e-03 7.319873e+02 5.000000e+00
1024 5.940000e-03 3.659937e+02 5.000000e+00
2048 5.600000e-03 1.829968e+02 5.000000e+00
3072 5.440000e-03 1.219979e+02 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0010_1.tex <==
1 1.739250e-01 3.747775e+05 4.000000e+00
2 8.907500e-02 1.873888e+05 4.000000e+00
4 4.660000e-02 9.369438e+04 4.000000e+00
8 2.640000e-02 4.684719e+04 4.000000e+00
16 1.480000e-02 2.342360e+04 4.000000e+00
32 8.675000e-03 1.171180e+04 4.000000e+00
64 5.900000e-03 5.855899e+03 4.000000e+00
128 4.225000e-03 2.927949e+03 4.000000e+00
256 4.100000e-03 1.463975e+03 4.000000e+00
512 3.450000e-03 7.319873e+02 4.000000e+00
1024 4.350000e-03 3.659937e+02 4.000000e+00
2048 4.500000e-03 1.829968e+02 4.000000e+00
3072 4.475000e-03 1.219979e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0011_0.tex <==
8 3.260800e-01 3.674826e+05 5.000000e+00
16 1.663200e-01 1.837413e+05 5.000000e+00
32 1.008400e-01 9.187066e+04 5.000000e+00
64 5.444000e-02 4.593533e+04 5.000000e+00
128 3.034000e-02 2.296766e+04 5.000000e+00
256 1.946000e-02 1.148383e+04 5.000000e+00
512 1.226000e-02 5.741916e+03 5.000000e+00
1024 8.060000e-03 2.870958e+03 5.000000e+00
2048 6.560000e-03 1.435479e+03 5.000000e+00
3072 7.280000e-03 9.569860e+02 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0011_1.tex <==
8 1.996250e-01 3.674826e+05 4.000000e+00
16 8.517500e-02 1.837413e+05 4.000000e+00
32 4.872500e-02 9.187066e+04 4.000000e+00
64 2.605000e-02 4.593533e+04 4.000000e+00
128 1.525000e-02 2.296766e+04 4.000000e+00
256 1.235000e-02 1.148383e+04 4.000000e+00
512 7.075000e-03 5.741916e+03 4.000000e+00
1024 5.800000e-03 2.870958e+03 4.000000e+00
2048 5.425000e-03 1.435479e+03 4.000000e+00
3072 5.525000e-03 9.569860e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0012_0.tex <==
64 4.128500e-01 3.638852e+05 4.000000e+00
128 2.279000e-01 1.819426e+05 4.000000e+00
256 1.134250e-01 9.097131e+04 4.000000e+00
512 6.892500e-02 4.548565e+04 4.000000e+00
1024 3.335000e-02 2.274283e+04 4.000000e+00
2048 2.220000e-02 1.137141e+04 4.000000e+00
3072 1.485000e-02 7.580942e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0012_1.tex <==
64 1.914000e-01 3.638852e+05 4.000000e+00
128 9.862500e-02 1.819426e+05 4.000000e+00
256 4.985000e-02 9.097131e+04 4.000000e+00
512 2.870000e-02 4.548565e+04 4.000000e+00
1024 1.897500e-02 2.274283e+04 4.000000e+00
2048 1.377500e-02 1.137141e+04 4.000000e+00
3072 1.127500e-02 7.580942e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-1/data_0013_0.tex <==
512 5.404750e-01 3.620633e+05 4.000000e+00
1024 2.515000e-01 1.810317e+05 4.000000e+00
2048 1.304750e-01 9.051584e+04 4.000000e+00
3072 8.295000e-02 6.034389e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0003_0.tex <==
1 1.500000e-04 1.518750e+01 4.000000e+00
2 1.750000e-04 7.593750e+00 4.000000e+00
4 1.750000e-04 3.796875e+00 4.000000e+00
8 2.000000e-04 1.898438e+00 4.000000e+00
16 2.000000e-04 9.492188e-01 4.000000e+00
32 2.250000e-04 4.746094e-01 4.000000e+00
64 2.250000e-04 2.373047e-01 4.000000e+00
128 2.500000e-04 1.186523e-01 4.000000e+00
256 3.000000e-04 5.932617e-02 4.000000e+00
512 2.750000e-04 2.966309e-02 4.000000e+00
1024 3.000000e-04 1.483154e-02 4.000000e+00
2048 3.250000e-04 7.415771e-03 4.000000e+00
3072 3.500000e-04 4.943848e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0003_1.tex <==
1 1.750000e-04 1.518750e+01 4.000000e+00
2 1.750000e-04 7.593750e+00 4.000000e+00
4 1.750000e-04 3.796875e+00 4.000000e+00
8 2.000000e-04 1.898438e+00 4.000000e+00
16 2.000000e-04 9.492188e-01 4.000000e+00
32 2.250000e-04 4.746094e-01 4.000000e+00
64 2.750000e-04 2.373047e-01 4.000000e+00
128 2.750000e-04 1.186523e-01 4.000000e+00
256 2.750000e-04 5.932617e-02 4.000000e+00
512 2.750000e-04 2.966309e-02 4.000000e+00
1024 3.000000e-04 1.483154e-02 4.000000e+00
2048 3.250000e-04 7.415771e-03 4.000000e+00
3072 3.500000e-04 4.943848e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0003_2.tex <==
1 1.500000e-04 1.518750e+01 4.000000e+00
2 1.750000e-04 7.593750e+00 4.000000e+00
4 1.750000e-04 3.796875e+00 4.000000e+00
8 1.750000e-04 1.898438e+00 4.000000e+00
16 2.000000e-04 9.492188e-01 4.000000e+00
32 2.000000e-04 4.746094e-01 4.000000e+00
64 2.000000e-04 2.373047e-01 4.000000e+00
128 2.000000e-04 1.186523e-01 4.000000e+00
256 2.000000e-04 5.932617e-02 4.000000e+00
512 2.500000e-04 2.966309e-02 4.000000e+00
1024 3.250000e-04 1.483154e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0004_0.tex <==
1 1.500000e-04 1.518750e+01 4.000000e+00
2 1.750000e-04 7.593750e+00 4.000000e+00
4 1.750000e-04 3.796875e+00 4.000000e+00
8 2.000000e-04 1.898438e+00 4.000000e+00
16 2.000000e-04 9.492188e-01 4.000000e+00
32 2.750000e-04 4.746094e-01 4.000000e+00
64 2.750000e-04 2.373047e-01 4.000000e+00
128 2.250000e-04 1.186523e-01 4.000000e+00
256 6.000000e-04 5.932617e-02 4.000000e+00
512 3.000000e-04 2.966309e-02 4.000000e+00
1024 3.250000e-04 1.483154e-02 4.000000e+00
2048 3.500000e-04 7.415771e-03 4.000000e+00
3072 3.750000e-04 4.943848e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0004_1.tex <==
1 1.750000e-04 1.518750e+01 4.000000e+00
2 2.000000e-04 7.593750e+00 4.000000e+00
4 2.000000e-04 3.796875e+00 4.000000e+00
8 2.000000e-04 1.898438e+00 4.000000e+00
16 2.250000e-04 9.492188e-01 4.000000e+00
32 2.500000e-04 4.746094e-01 4.000000e+00
64 4.250000e-04 2.373047e-01 4.000000e+00
128 2.500000e-04 1.186523e-01 4.000000e+00
256 4.000000e-04 5.932617e-02 4.000000e+00
512 3.000000e-04 2.966309e-02 4.000000e+00
1024 3.000000e-04 1.483154e-02 4.000000e+00
2048 3.500000e-04 7.415771e-03 4.000000e+00
3072 3.750000e-04 4.943848e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0004_2.tex <==
1 1.575000e-03 1.928688e+03 4.000000e+00
2 1.675000e-03 9.643438e+02 4.000000e+00
4 1.700000e-03 4.821719e+02 4.000000e+00
8 1.750000e-03 2.410859e+02 4.000000e+00
16 1.775000e-03 1.205430e+02 4.000000e+00
32 1.750000e-03 6.027148e+01 4.000000e+00
64 1.775000e-03 3.013574e+01 4.000000e+00
128 1.750000e-03 1.506787e+01 4.000000e+00
256 1.775000e-03 7.533936e+00 4.000000e+00
512 1.825000e-03 3.766968e+00 4.000000e+00
1024 1.850000e-03 1.883484e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0005_0.tex <==
1 1.375000e-03 1.928688e+03 4.000000e+00
2 1.400000e-03 9.643438e+02 4.000000e+00
4 1.525000e-03 4.821719e+02 4.000000e+00
8 1.475000e-03 2.410859e+02 4.000000e+00
16 1.550000e-03 1.205430e+02 4.000000e+00
32 1.625000e-03 6.027148e+01 4.000000e+00
64 1.550000e-03 3.013574e+01 4.000000e+00
128 2.075000e-03 1.506787e+01 4.000000e+00
256 1.600000e-03 7.533936e+00 4.000000e+00
512 1.600000e-03 3.766968e+00 4.000000e+00
1024 1.700000e-03 1.883484e+00 4.000000e+00
2048 1.700000e-03 9.417419e-01 4.000000e+00
3072 1.725000e-03 6.278280e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0005_1.tex <==
1 1.450000e-03 1.928688e+03 4.000000e+00
2 1.525000e-03 9.643438e+02 4.000000e+00
4 1.575000e-03 4.821719e+02 4.000000e+00
8 1.575000e-03 2.410859e+02 4.000000e+00
16 1.600000e-03 1.205430e+02 4.000000e+00
32 1.575000e-03 6.027148e+01 4.000000e+00
64 1.750000e-03 3.013574e+01 4.000000e+00
128 1.675000e-03 1.506787e+01 4.000000e+00
256 1.750000e-03 7.533936e+00 4.000000e+00
512 1.550000e-03 3.766968e+00 4.000000e+00
1024 1.575000e-03 1.883484e+00 4.000000e+00
2048 1.625000e-03 9.417419e-01 4.000000e+00
3072 1.575000e-03 6.278280e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0005_2.tex <==
1 1.197500e-02 5.512835e+04 4.000000e+00
2 8.450000e-03 2.756418e+04 4.000000e+00
4 6.000000e-03 1.378209e+04 4.000000e+00
8 4.100000e-03 6.891044e+03 4.000000e+00
16 3.400000e-03 3.445522e+03 4.000000e+00
32 3.250000e-03 1.722761e+03 4.000000e+00
64 3.200000e-03 8.613805e+02 4.000000e+00
128 3.150000e-03 4.306903e+02 4.000000e+00
256 3.000000e-03 2.153451e+02 4.000000e+00
512 3.300000e-03 1.076726e+02 4.000000e+00
1024 3.325000e-03 5.383628e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0006_0.tex <==
1 3.000000e-03 1.062652e+04 4.000000e+00
2 2.525000e-03 5.313260e+03 4.000000e+00
4 2.275000e-03 2.656630e+03 4.000000e+00
8 2.150000e-03 1.328315e+03 4.000000e+00
16 2.175000e-03 6.641576e+02 4.000000e+00
32 2.550000e-03 3.320788e+02 4.000000e+00
64 2.950000e-03 1.660394e+02 4.000000e+00
128 2.675000e-03 8.301969e+01 4.000000e+00
256 2.150000e-03 4.150985e+01 4.000000e+00
512 2.150000e-03 2.075492e+01 4.000000e+00
1024 2.200000e-03 1.037746e+01 4.000000e+00
2048 2.200000e-03 5.188731e+00 4.000000e+00
3072 2.325000e-03 3.459154e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0006_1.tex <==
1 2.950000e-03 1.062652e+04 4.000000e+00
2 2.425000e-03 5.313260e+03 4.000000e+00
4 2.225000e-03 2.656630e+03 4.000000e+00
8 2.200000e-03 1.328315e+03 4.000000e+00
16 2.125000e-03 6.641576e+02 4.000000e+00
32 2.275000e-03 3.320788e+02 4.000000e+00
64 2.075000e-03 1.660394e+02 4.000000e+00
128 2.750000e-03 8.301969e+01 4.000000e+00
256 2.725000e-03 4.150985e+01 4.000000e+00
512 2.100000e-03 2.075492e+01 4.000000e+00
1024 2.025000e-03 1.037746e+01 4.000000e+00
2048 2.150000e-03 5.188731e+00 4.000000e+00
3072 2.100000e-03 3.459154e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0006_2.tex <==
1 8.470000e-02 3.870539e+05 4.000000e+00
2 4.112500e-02 1.935269e+05 4.000000e+00
4 2.357500e-02 9.676346e+04 4.000000e+00
8 1.282500e-02 4.838173e+04 4.000000e+00
16 8.275000e-03 2.419087e+04 4.000000e+00
32 5.650000e-03 1.209543e+04 4.000000e+00
64 5.175000e-03 6.047716e+03 4.000000e+00
128 4.650000e-03 3.023858e+03 4.000000e+00
256 4.475000e-03 1.511929e+03 4.000000e+00
512 4.900000e-03 7.559646e+02 4.000000e+00
1024 4.825000e-03 3.779823e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0007_0.tex <==
1 1.080000e-02 5.512835e+04 4.000000e+00
2 8.150000e-03 2.756418e+04 4.000000e+00
4 5.775000e-03 1.378209e+04 4.000000e+00
8 4.050000e-03 6.891044e+03 4.000000e+00
16 3.300000e-03 3.445522e+03 4.000000e+00
32 3.475000e-03 1.722761e+03 4.000000e+00
64 3.175000e-03 8.613805e+02 4.000000e+00
128 3.100000e-03 4.306903e+02 4.000000e+00
256 3.100000e-03 2.153451e+02 4.000000e+00
512 3.050000e-03 1.076726e+02 4.000000e+00
1024 3.625000e-03 5.383628e+01 4.000000e+00
2048 3.125000e-03 2.691814e+01 4.000000e+00
3072 3.200000e-03 1.794543e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0007_1.tex <==
1 9.700000e-03 5.512835e+04 4.000000e+00
2 6.100000e-03 2.756418e+04 4.000000e+00
4 4.600000e-03 1.378209e+04 4.000000e+00
8 3.725000e-03 6.891044e+03 4.000000e+00
16 3.300000e-03 3.445522e+03 4.000000e+00
32 3.300000e-03 1.722761e+03 4.000000e+00
64 3.075000e-03 8.613805e+02 4.000000e+00
128 4.000000e-03 4.306903e+02 4.000000e+00
256 4.950000e-03 2.153451e+02 4.000000e+00
512 2.875000e-03 1.076726e+02 4.000000e+00
1024 2.975000e-03 5.383628e+01 4.000000e+00
2048 3.125000e-03 2.691814e+01 4.000000e+00
3072 3.000000e-03 1.794543e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0007_2.tex <==
8 1.128200e+00 2.927377e+06 4.000000e+00
16 6.092000e-01 1.463688e+06 4.000000e+00
32 3.073750e-01 7.318442e+05 4.000000e+00
64 1.910250e-01 3.659221e+05 4.000000e+00
128 8.340000e-02 1.829610e+05 4.000000e+00
256 4.170000e-02 9.148052e+04 4.000000e+00
512 2.560000e-02 4.574026e+04 4.000000e+00
1024 1.532500e-02 2.287013e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0008_0.tex <==
1 8.207500e-02 3.870539e+05 4.000000e+00
2 5.065000e-02 1.935269e+05 4.000000e+00
4 2.677500e-02 9.676346e+04 4.000000e+00
8 1.720000e-02 4.838173e+04 4.000000e+00
16 9.900000e-03 2.419087e+04 4.000000e+00
32 7.400000e-03 1.209543e+04 4.000000e+00
64 5.250000e-03 6.047716e+03 4.000000e+00
128 4.800000e-03 3.023858e+03 4.000000e+00
256 8.275000e-03 1.511929e+03 4.000000e+00
512 4.850000e-03 7.559646e+02 4.000000e+00
1024 4.625000e-03 3.779823e+02 4.000000e+00
2048 4.500000e-03 1.889911e+02 4.000000e+00
3072 4.575000e-03 1.259941e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0008_1.tex <==
1 6.807500e-02 3.870539e+05 4.000000e+00
2 3.445000e-02 1.935269e+05 4.000000e+00
4 1.717500e-02 9.676346e+04 4.000000e+00
8 1.170000e-02 4.838173e+04 4.000000e+00
16 6.825000e-03 2.419087e+04 4.000000e+00
32 5.450000e-03 1.209543e+04 4.000000e+00
64 4.350000e-03 6.047716e+03 4.000000e+00
128 6.025000e-03 3.023858e+03 4.000000e+00
256 3.825000e-03 1.511929e+03 4.000000e+00
512 4.100000e-03 7.559646e+02 4.000000e+00
1024 3.900000e-03 3.779823e+02 4.000000e+00
2048 3.875000e-03 1.889911e+02 4.000000e+00
3072 3.850000e-03 1.259941e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0008_2.tex <==
64 6.676500e-01 2.904492e+06 4.000000e+00
128 2.624250e-01 1.452246e+06 4.000000e+00
256 1.368250e-01 7.261231e+05 4.000000e+00
512 1.138250e-01 3.630615e+05 4.000000e+00
1024 5.587500e-02 1.815308e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0009_0.tex <==
1 6.500750e-01 2.974569e+06 4.000000e+00
2 3.938500e-01 1.487285e+06 4.000000e+00
4 2.110750e-01 7.436423e+05 4.000000e+00
8 1.436250e-01 3.718211e+05 4.000000e+00
16 6.147500e-02 1.859106e+05 4.000000e+00
32 3.765000e-02 9.295528e+04 4.000000e+00
64 2.082500e-02 4.647764e+04 4.000000e+00
128 1.165000e-02 2.323882e+04 4.000000e+00
256 8.575000e-03 1.161941e+04 4.000000e+00
512 6.575000e-03 5.809705e+03 4.000000e+00
1024 6.400000e-03 2.904853e+03 4.000000e+00
2048 6.775000e-03 1.452426e+03 4.000000e+00
3072 6.850000e-03 9.682842e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0009_1.tex <==
1 4.996000e-01 2.974569e+06 4.000000e+00
2 2.554500e-01 1.487285e+06 4.000000e+00
4 1.299250e-01 7.436423e+05 4.000000e+00
8 1.014250e-01 3.718211e+05 4.000000e+00
16 3.417500e-02 1.859106e+05 4.000000e+00
32 2.172500e-02 9.295528e+04 4.000000e+00
64 1.187500e-02 4.647764e+04 4.000000e+00
128 7.375000e-03 2.323882e+04 4.000000e+00
256 5.875000e-03 1.161941e+04 4.000000e+00
512 5.500000e-03 5.809705e+03 4.000000e+00
1024 4.525000e-03 2.904853e+03 4.000000e+00
2048 4.700000e-03 1.452426e+03 4.000000e+00
3072 5.200000e-03 9.682842e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0010_0.tex <==
8 1.169925e+00 2.927377e+06 4.000000e+00
16 4.858500e-01 1.463688e+06 4.000000e+00
32 3.443500e-01 7.318442e+05 4.000000e+00
64 1.691750e-01 3.659221e+05 4.000000e+00
128 9.732500e-02 1.829610e+05 4.000000e+00
256 4.642500e-02 9.148052e+04 4.000000e+00
512 2.297500e-02 4.574026e+04 4.000000e+00
1024 1.337500e-02 2.287013e+04 4.000000e+00
2048 9.750000e-03 1.143507e+04 4.000000e+00
3072 9.725000e-03 7.623377e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0010_1.tex <==
8 8.134750e-01 2.927377e+06 4.000000e+00
16 2.666500e-01 1.463688e+06 4.000000e+00
32 2.031250e-01 7.318442e+05 4.000000e+00
64 8.225000e-02 3.659221e+05 4.000000e+00
128 5.072500e-02 1.829610e+05 4.000000e+00
256 2.507500e-02 9.148052e+04 4.000000e+00
512 1.310000e-02 4.574026e+04 4.000000e+00
1024 8.250000e-03 2.287013e+04 4.000000e+00
2048 6.625000e-03 1.143507e+04 4.000000e+00
3072 6.425000e-03 7.623377e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0011_0.tex <==
64 1.289925e+00 2.904492e+06 4.000000e+00
128 8.208500e-01 1.452246e+06 4.000000e+00
256 4.774750e-01 7.261231e+05 4.000000e+00
512 2.266000e-01 3.630615e+05 4.000000e+00
1024 1.132250e-01 1.815308e+05 4.000000e+00
2048 5.225000e-02 9.076538e+04 4.000000e+00
3072 3.477500e-02 6.051025e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0011_1.tex <==
64 6.316250e-01 2.904492e+06 4.000000e+00
128 4.051750e-01 1.452246e+06 4.000000e+00
256 2.479750e-01 7.261231e+05 4.000000e+00
512 1.045750e-01 3.630615e+05 4.000000e+00
1024 5.205000e-02 1.815308e+05 4.000000e+00
2048 2.537500e-02 9.076538e+04 4.000000e+00
3072 1.865000e-02 6.051025e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0012_0.tex <==
512 1.852740e+00 2.893403e+06 5.000000e+00
1024 9.919800e-01 1.446702e+06 5.000000e+00
2048 5.289000e-01 7.233509e+05 5.000000e+00
3072 3.463000e-01 4.822339e+05 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0012_1.tex <==
512 8.062600e-01 2.893403e+06 5.000000e+00
1024 4.138800e-01 1.446702e+06 5.000000e+00
2048 2.508800e-01 7.233509e+05 5.000000e+00
3072 1.459400e-01 4.822339e+05 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-annulus-4/data_0013_0.tex <==
3072 2.769500e+00 3.850226e+06 5.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0003_0.tex <==
1 2.750000e-04 4.645833e+00 4.000000e+00
2 3.000000e-04 2.322917e+00 4.000000e+00
4 3.000000e-04 1.161458e+00 4.000000e+00
8 3.250000e-04 5.807292e-01 4.000000e+00
16 3.500000e-04 2.903646e-01 4.000000e+00
32 4.500000e-04 1.451823e-01 4.000000e+00
64 3.750000e-04 7.259115e-02 4.000000e+00
128 5.500000e-04 3.629557e-02 4.000000e+00
256 8.000000e-04 1.814779e-02 4.000000e+00
512 7.000000e-04 9.073893e-03 4.000000e+00
1024 5.250000e-04 4.536947e-03 4.000000e+00
2048 5.750000e-04 2.268473e-03 4.000000e+00
3072 5.750000e-04 1.512316e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0003_1.tex <==
1 2.250000e-04 4.645833e+00 4.000000e+00
2 2.250000e-04 2.322917e+00 4.000000e+00
4 2.250000e-04 1.161458e+00 4.000000e+00
8 3.000000e-04 5.807292e-01 4.000000e+00
16 2.500000e-04 2.903646e-01 4.000000e+00
32 3.000000e-04 1.451823e-01 4.000000e+00
64 2.750000e-04 7.259115e-02 4.000000e+00
128 3.000000e-04 3.629557e-02 4.000000e+00
256 3.250000e-04 1.814779e-02 4.000000e+00
512 3.500000e-04 9.073893e-03 4.000000e+00
1024 3.750000e-04 4.536947e-03 4.000000e+00
2048 3.750000e-04 2.268473e-03 4.000000e+00
3072 4.250000e-04 1.512316e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0004_0.tex <==
1 6.500000e-04 2.100000e+01 4.000000e+00
2 6.500000e-04 1.050000e+01 4.000000e+00
4 6.500000e-04 5.250000e+00 4.000000e+00
8 8.000000e-04 2.625000e+00 4.000000e+00
16 7.000000e-04 1.312500e+00 4.000000e+00
32 8.000000e-04 6.562500e-01 4.000000e+00
64 8.250000e-04 3.281250e-01 4.000000e+00
128 9.500000e-04 1.640625e-01 4.000000e+00
256 7.750000e-04 8.203125e-02 4.000000e+00
512 8.000000e-04 4.101562e-02 4.000000e+00
1024 8.750000e-04 2.050781e-02 4.000000e+00
2048 9.500000e-04 1.025391e-02 4.000000e+00
3072 9.500000e-04 6.835938e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0004_1.tex <==
1 4.000000e-04 2.100000e+01 4.000000e+00
2 4.000000e-04 1.050000e+01 4.000000e+00
4 4.000000e-04 5.250000e+00 4.000000e+00
8 5.500000e-04 2.625000e+00 4.000000e+00
16 4.250000e-04 1.312500e+00 4.000000e+00
32 5.250000e-04 6.562500e-01 4.000000e+00
64 4.500000e-04 3.281250e-01 4.000000e+00
128 5.750000e-04 1.640625e-01 4.000000e+00
256 5.000000e-04 8.203125e-02 4.000000e+00
512 5.000000e-04 4.101562e-02 4.000000e+00
1024 5.250000e-04 2.050781e-02 4.000000e+00
2048 5.750000e-04 1.025391e-02 4.000000e+00
3072 5.500000e-04 6.835938e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0005_0.tex <==
1 8.750000e-04 1.188125e+02 4.000000e+00
2 1.025000e-03 5.940625e+01 4.000000e+00
4 1.025000e-03 2.970312e+01 4.000000e+00
8 1.850000e-03 1.485156e+01 4.000000e+00
16 1.175000e-03 7.425781e+00 4.000000e+00
32 1.100000e-03 3.712891e+00 4.000000e+00
64 1.225000e-03 1.856445e+00 4.000000e+00
128 1.550000e-03 9.282227e-01 4.000000e+00
256 1.125000e-03 4.641113e-01 4.000000e+00
512 1.200000e-03 2.320557e-01 4.000000e+00
1024 1.225000e-03 1.160278e-01 4.000000e+00
2048 1.200000e-03 5.801392e-02 4.000000e+00
3072 1.225000e-03 3.867594e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0005_1.tex <==
1 6.250000e-04 1.188125e+02 4.000000e+00
2 6.250000e-04 5.940625e+01 4.000000e+00
4 6.250000e-04 2.970312e+01 4.000000e+00
8 7.000000e-04 1.485156e+01 4.000000e+00
16 6.500000e-04 7.425781e+00 4.000000e+00
32 6.250000e-04 3.712891e+00 4.000000e+00
64 7.500000e-04 1.856445e+00 4.000000e+00
128 9.250000e-04 9.282227e-01 4.000000e+00
256 7.000000e-04 4.641113e-01 4.000000e+00
512 7.250000e-04 2.320557e-01 4.000000e+00
1024 7.500000e-04 1.160278e-01 4.000000e+00
2048 7.750000e-04 5.801392e-02 4.000000e+00
3072 8.250000e-04 3.867594e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0006_0.tex <==
1 1.525000e-03 8.000417e+02 4.000000e+00
2 1.375000e-03 4.000208e+02 4.000000e+00
4 1.325000e-03 2.000104e+02 4.000000e+00
8 1.600000e-03 1.000052e+02 4.000000e+00
16 1.425000e-03 5.000260e+01 4.000000e+00
32 2.925000e-03 2.500130e+01 4.000000e+00
64 1.600000e-03 1.250065e+01 4.000000e+00
128 1.500000e-03 6.250326e+00 4.000000e+00
256 1.600000e-03 3.125163e+00 4.000000e+00
512 1.575000e-03 1.562581e+00 4.000000e+00
1024 1.500000e-03 7.812907e-01 4.000000e+00
2048 1.625000e-03 3.906453e-01 4.000000e+00
3072 1.700000e-03 2.604302e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0006_1.tex <==
1 1.125000e-03 8.000417e+02 4.000000e+00
2 1.000000e-03 4.000208e+02 4.000000e+00
4 9.500000e-04 2.000104e+02 4.000000e+00
8 1.050000e-03 1.000052e+02 4.000000e+00
16 1.175000e-03 5.000260e+01 4.000000e+00
32 1.225000e-03 2.500130e+01 4.000000e+00
64 1.375000e-03 1.250065e+01 4.000000e+00
128 1.825000e-03 6.250326e+00 4.000000e+00
256 1.050000e-03 3.125163e+00 4.000000e+00
512 1.050000e-03 1.562581e+00 4.000000e+00
1024 1.075000e-03 7.812907e-01 4.000000e+00
2048 1.050000e-03 3.906453e-01 4.000000e+00
3072 1.100000e-03 2.604302e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0007_0.tex <==
1 5.025000e-03 5.898104e+03 4.000000e+00
2 4.800000e-03 2.949052e+03 4.000000e+00
4 2.550000e-03 1.474526e+03 4.000000e+00
8 2.275000e-03 7.372630e+02 4.000000e+00
16 1.975000e-03 3.686315e+02 4.000000e+00
32 2.150000e-03 1.843158e+02 4.000000e+00
64 3.550000e-03 9.215788e+01 4.000000e+00
128 3.575000e-03 4.607894e+01 4.000000e+00
256 5.525000e-03 2.303947e+01 4.000000e+00
512 2.475000e-03 1.151973e+01 4.000000e+00
1024 2.150000e-03 5.759867e+00 4.000000e+00
2048 2.000000e-03 2.879934e+00 4.000000e+00
3072 1.950000e-03 1.919956e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0007_1.tex <==
1 3.633333e-03 5.898104e+03 3.000000e+00
2 2.433333e-03 2.949052e+03 3.000000e+00
4 1.833333e-03 1.474526e+03 3.000000e+00
8 1.800000e-03 7.372630e+02 3.000000e+00
16 2.000000e-03 3.686315e+02 3.000000e+00
32 1.733333e-03 1.843158e+02 3.000000e+00
64 1.833333e-03 9.215788e+01 3.000000e+00
128 2.033333e-03 4.607894e+01 3.000000e+00
256 2.466667e-03 2.303947e+01 3.000000e+00
512 1.700000e-03 1.151973e+01 3.000000e+00
1024 1.900000e-03 5.759867e+00 3.000000e+00
2048 2.166667e-03 2.879934e+00 3.000000e+00
3072 1.566667e-03 1.919956e+00 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0008_0.tex <==
1 2.790000e-02 4.537383e+04 4.000000e+00
2 1.632500e-02 2.268692e+04 4.000000e+00
4 9.575000e-03 1.134346e+04 4.000000e+00
8 6.125000e-03 5.671729e+03 4.000000e+00
16 4.300000e-03 2.835865e+03 4.000000e+00
32 3.650000e-03 1.417932e+03 4.000000e+00
64 5.825000e-03 7.089661e+02 4.000000e+00
128 3.825000e-03 3.544831e+02 4.000000e+00
256 4.850000e-03 1.772415e+02 4.000000e+00
512 3.100000e-03 8.862077e+01 4.000000e+00
1024 4.075000e-03 4.431038e+01 4.000000e+00
2048 3.450000e-03 2.215519e+01 4.000000e+00
3072 3.300000e-03 1.477013e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0008_1.tex <==
1 2.090000e-02 4.537383e+04 3.000000e+00
2 1.183333e-02 2.268692e+04 3.000000e+00
4 6.700000e-03 1.134346e+04 3.000000e+00
8 4.466667e-03 5.671729e+03 3.000000e+00
16 3.000000e-03 2.835865e+03 3.000000e+00
32 2.700000e-03 1.417932e+03 3.000000e+00
64 3.166667e-03 7.089661e+02 3.000000e+00
128 2.366667e-03 3.544831e+02 3.000000e+00
256 4.333333e-03 1.772415e+02 3.000000e+00
512 3.200000e-03 8.862077e+01 3.000000e+00
1024 3.600000e-03 4.431038e+01 3.000000e+00
2048 4.200000e-03 2.215519e+01 3.000000e+00
3072 3.700000e-03 1.477013e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0009_0.tex <==
1 1.690250e-01 3.561329e+05 4.000000e+00
2 1.045000e-01 1.780664e+05 4.000000e+00
4 5.560000e-02 8.903322e+04 4.000000e+00
8 3.080000e-02 4.451661e+04 4.000000e+00
16 1.712500e-02 2.225831e+04 4.000000e+00
32 1.142500e-02 1.112915e+04 4.000000e+00
64 7.175000e-03 5.564576e+03 4.000000e+00
128 5.450000e-03 2.782288e+03 4.000000e+00
256 7.100000e-03 1.391144e+03 4.000000e+00
512 4.225000e-03 6.955721e+02 4.000000e+00
1024 5.075000e-03 3.477860e+02 4.000000e+00
2048 4.675000e-03 1.738930e+02 4.000000e+00
3072 4.375000e-03 1.159287e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0009_1.tex <==
1 1.467333e-01 3.561329e+05 3.000000e+00
2 7.853333e-02 1.780664e+05 3.000000e+00
4 4.206667e-02 8.903322e+04 3.000000e+00
8 2.153333e-02 4.451661e+04 3.000000e+00
16 1.296667e-02 2.225831e+04 3.000000e+00
32 7.733333e-03 1.112915e+04 3.000000e+00
64 5.633333e-03 5.564576e+03 3.000000e+00
128 4.233333e-03 2.782288e+03 3.000000e+00
256 3.600000e-03 1.391144e+03 3.000000e+00
512 3.800000e-03 6.955721e+02 3.000000e+00
1024 4.233333e-03 3.477860e+02 3.000000e+00
2048 4.900000e-03 1.738930e+02 3.000000e+00
3072 5.366667e-03 1.159287e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0010_0.tex <==
8 2.160500e-01 3.527983e+05 4.000000e+00
16 1.113500e-01 1.763992e+05 4.000000e+00
32 6.117500e-02 8.819958e+04 4.000000e+00
64 3.322500e-02 4.409979e+04 4.000000e+00
128 1.937500e-02 2.204990e+04 4.000000e+00
256 1.672500e-02 1.102495e+04 4.000000e+00
512 8.650000e-03 5.512474e+03 4.000000e+00
1024 6.575000e-03 2.756237e+03 4.000000e+00
2048 6.450000e-03 1.378118e+03 4.000000e+00
3072 6.625000e-03 9.187456e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0010_1.tex <==
8 1.644500e-01 3.527983e+05 2.000000e+00
16 8.020000e-02 1.763992e+05 2.000000e+00
32 4.520000e-02 8.819958e+04 2.000000e+00
64 2.265000e-02 4.409979e+04 2.000000e+00
128 1.370000e-02 2.204990e+04 2.000000e+00
256 9.900000e-03 1.102495e+04 2.000000e+00
512 6.750000e-03 5.512474e+03 2.000000e+00
1024 5.650000e-03 2.756237e+03 2.000000e+00
2048 6.350000e-03 1.378118e+03 2.000000e+00
3072 6.100000e-03 9.187456e+02 2.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0011_0.tex <==
64 2.426750e-01 3.511542e+05 4.000000e+00
128 1.335000e-01 1.755771e+05 4.000000e+00
256 8.167500e-02 8.778855e+04 4.000000e+00
512 3.780000e-02 4.389428e+04 4.000000e+00
1024 2.562500e-02 2.194714e+04 4.000000e+00
2048 1.842500e-02 1.097357e+04 4.000000e+00
3072 1.440000e-02 7.315713e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0011_1.tex <==
128 9.255000e-02 1.755771e+05 2.000000e+00
256 5.180000e-02 8.778855e+04 2.000000e+00
512 2.715000e-02 4.389428e+04 2.000000e+00
1024 1.745000e-02 2.194714e+04 2.000000e+00
2048 1.225000e-02 1.097357e+04 2.000000e+00
3072 1.105000e-02 7.315713e+03 2.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0012_0.tex <==
2048 7.765000e-02 8.758447e+04 4.000000e+00
3072 5.767500e-02 5.838965e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-1/data_0012_1.tex <==
2048 5.630000e-02 8.758447e+04 3.000000e+00
3072 3.883333e-02 5.838965e+04 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0003_0.tex <==
1 6.250000e-04 1.936458e+02 4.000000e+00
2 6.500000e-04 9.682292e+01 4.000000e+00
4 6.500000e-04 4.841146e+01 4.000000e+00
8 7.000000e-04 2.420573e+01 4.000000e+00
16 7.000000e-04 1.210286e+01 4.000000e+00
32 7.250000e-04 6.051432e+00 4.000000e+00
64 7.250000e-04 3.025716e+00 4.000000e+00
128 7.500000e-04 1.512858e+00 4.000000e+00
256 7.750000e-04 7.564290e-01 4.000000e+00
512 8.250000e-04 3.782145e-01 4.000000e+00
1024 8.250000e-04 1.891073e-01 4.000000e+00
2048 8.750000e-04 9.455363e-02 4.000000e+00
3072 9.000000e-04 6.303575e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0003_1.tex <==
1 6.000000e-04 1.936458e+02 4.000000e+00
2 6.000000e-04 9.682292e+01 4.000000e+00
4 6.500000e-04 4.841146e+01 4.000000e+00
8 6.500000e-04 2.420573e+01 4.000000e+00
16 6.500000e-04 1.210286e+01 4.000000e+00
32 6.750000e-04 6.051432e+00 4.000000e+00
64 6.500000e-04 3.025716e+00 4.000000e+00
128 7.000000e-04 1.512858e+00 4.000000e+00
256 8.250000e-04 7.564290e-01 4.000000e+00
512 7.250000e-04 3.782145e-01 4.000000e+00
1024 7.250000e-04 1.891073e-01 4.000000e+00
2048 7.500000e-04 9.455363e-02 4.000000e+00
3072 7.500000e-04 6.303575e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0004_0.tex <==
1 1.125000e-03 1.053188e+03 4.000000e+00
2 1.100000e-03 5.265938e+02 4.000000e+00
4 1.225000e-03 2.632969e+02 4.000000e+00
8 1.125000e-03 1.316484e+02 4.000000e+00
16 1.250000e-03 6.582422e+01 4.000000e+00
32 1.125000e-03 3.291211e+01 4.000000e+00
64 1.175000e-03 1.645605e+01 4.000000e+00
128 1.150000e-03 8.228027e+00 4.000000e+00
256 1.200000e-03 4.114014e+00 4.000000e+00
512 1.350000e-03 2.057007e+00 4.000000e+00
1024 1.325000e-03 1.028503e+00 4.000000e+00
2048 1.400000e-03 5.142517e-01 4.000000e+00
3072 1.400000e-03 3.428345e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0004_1.tex <==
1 1.075000e-03 1.053188e+03 4.000000e+00
2 1.000000e-03 5.265938e+02 4.000000e+00
4 1.100000e-03 2.632969e+02 4.000000e+00
8 1.025000e-03 1.316484e+02 4.000000e+00
16 1.025000e-03 6.582422e+01 4.000000e+00
32 1.025000e-03 3.291211e+01 4.000000e+00
64 1.175000e-03 1.645605e+01 4.000000e+00
128 1.050000e-03 8.228027e+00 4.000000e+00
256 1.300000e-03 4.114014e+00 4.000000e+00
512 1.100000e-03 2.057007e+00 4.000000e+00
1024 1.100000e-03 1.028503e+00 4.000000e+00
2048 1.075000e-03 5.142517e-01 4.000000e+00
3072 1.125000e-03 3.428345e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0005_0.tex <==
1 2.200000e-03 6.692562e+03 4.000000e+00
2 1.825000e-03 3.346281e+03 4.000000e+00
4 1.800000e-03 1.673141e+03 4.000000e+00
8 1.825000e-03 8.365703e+02 4.000000e+00
16 2.125000e-03 4.182852e+02 4.000000e+00
32 1.675000e-03 2.091426e+02 4.000000e+00
64 1.900000e-03 1.045713e+02 4.000000e+00
128 1.700000e-03 5.228564e+01 4.000000e+00
256 1.750000e-03 2.614282e+01 4.000000e+00
512 1.825000e-03 1.307141e+01 4.000000e+00
1024 1.775000e-03 6.535706e+00 4.000000e+00
2048 1.875000e-03 3.267853e+00 4.000000e+00
3072 1.925000e-03 2.178569e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0005_1.tex <==
1 2.066667e-03 6.692562e+03 3.000000e+00
2 1.733333e-03 3.346281e+03 3.000000e+00
4 1.700000e-03 1.673141e+03 3.000000e+00
8 1.733333e-03 8.365703e+02 3.000000e+00
16 1.633333e-03 4.182852e+02 3.000000e+00
32 1.566667e-03 2.091426e+02 3.000000e+00
64 1.566667e-03 1.045713e+02 3.000000e+00
128 1.566667e-03 5.228564e+01 3.000000e+00
256 1.866667e-03 2.614282e+01 3.000000e+00
512 1.500000e-03 1.307141e+01 3.000000e+00
1024 1.533333e-03 6.535706e+00 3.000000e+00
2048 1.533333e-03 3.267853e+00 3.000000e+00
3072 1.566667e-03 2.178569e+00 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0006_0.tex <==
1 9.825000e-03 4.802960e+04 4.000000e+00
2 5.850000e-03 2.401480e+04 4.000000e+00
4 4.250000e-03 1.200740e+04 4.000000e+00
8 2.850000e-03 6.003701e+03 4.000000e+00
16 2.500000e-03 3.001850e+03 4.000000e+00
32 2.825000e-03 1.500925e+03 4.000000e+00
64 5.450000e-03 7.504626e+02 4.000000e+00
128 2.650000e-03 3.752313e+02 4.000000e+00
256 2.900000e-03 1.876156e+02 4.000000e+00
512 3.025000e-03 9.380782e+01 4.000000e+00
1024 2.975000e-03 4.690391e+01 4.000000e+00
2048 3.125000e-03 2.345196e+01 4.000000e+00
3072 3.400000e-03 1.563464e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0006_1.tex <==
1 7.433333e-03 4.802960e+04 3.000000e+00
2 4.366667e-03 2.401480e+04 3.000000e+00
4 3.500000e-03 1.200740e+04 3.000000e+00
8 2.733333e-03 6.003701e+03 3.000000e+00
16 2.400000e-03 3.001850e+03 3.000000e+00
32 2.466667e-03 1.500925e+03 3.000000e+00
64 3.066667e-03 7.504626e+02 3.000000e+00
128 2.333333e-03 3.752313e+02 3.000000e+00
256 2.733333e-03 1.876156e+02 3.000000e+00
512 2.233333e-03 9.380782e+01 3.000000e+00
1024 2.266667e-03 4.690391e+01 3.000000e+00
2048 2.466667e-03 2.345196e+01 3.000000e+00
3072 2.400000e-03 1.563464e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0007_0.tex <==
1 7.850000e-02 3.656660e+05 4.000000e+00
2 3.917500e-02 1.828330e+05 4.000000e+00
4 1.925000e-02 9.141649e+04 4.000000e+00
8 1.110000e-02 4.570825e+04 4.000000e+00
16 6.575000e-03 2.285412e+04 4.000000e+00
32 5.050000e-03 1.142706e+04 4.000000e+00
64 4.575000e-03 5.713531e+03 4.000000e+00
128 4.150000e-03 2.856765e+03 4.000000e+00
256 4.675000e-03 1.428383e+03 4.000000e+00
512 4.300000e-03 7.141914e+02 4.000000e+00
1024 4.325000e-03 3.570957e+02 4.000000e+00
2048 4.325000e-03 1.785478e+02 4.000000e+00
3072 4.250000e-03 1.190319e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0007_1.tex <==
1 6.193333e-02 3.656660e+05 3.000000e+00
2 3.116667e-02 1.828330e+05 3.000000e+00
4 1.530000e-02 9.141649e+04 3.000000e+00
8 8.333333e-03 4.570825e+04 3.000000e+00
16 5.866667e-03 2.285412e+04 3.000000e+00
32 4.833333e-03 1.142706e+04 3.000000e+00
64 4.533333e-03 5.713531e+03 3.000000e+00
128 3.133333e-03 2.856765e+03 3.000000e+00
256 3.166667e-03 1.428383e+03 3.000000e+00
512 3.533333e-03 7.141914e+02 3.000000e+00
1024 3.466667e-03 3.570957e+02 3.000000e+00
2048 3.166667e-03 1.785478e+02 3.000000e+00
3072 3.400000e-03 1.190319e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0008_0.tex <==
1 6.058000e-01 2.858333e+06 4.000000e+00
2 3.141500e-01 1.429167e+06 4.000000e+00
4 1.594750e-01 7.145833e+05 4.000000e+00
8 8.445000e-02 3.572916e+05 4.000000e+00
16 4.190000e-02 1.786458e+05 4.000000e+00
32 2.657500e-02 8.932291e+04 4.000000e+00
64 1.255000e-02 4.466145e+04 4.000000e+00
128 7.850000e-03 2.233073e+04 4.000000e+00
256 7.650000e-03 1.116536e+04 4.000000e+00
512 6.050000e-03 5.582682e+03 4.000000e+00
1024 5.475000e-03 2.791341e+03 4.000000e+00
2048 6.775000e-03 1.395670e+03 4.000000e+00
3072 5.700000e-03 9.304469e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0008_1.tex <==
1 4.725333e-01 2.858333e+06 3.000000e+00
2 2.467000e-01 1.429167e+06 3.000000e+00
4 1.270333e-01 7.145833e+05 3.000000e+00
8 6.586667e-02 3.572916e+05 3.000000e+00
16 3.250000e-02 1.786458e+05 3.000000e+00
32 2.166667e-02 8.932291e+04 3.000000e+00
64 1.086667e-02 4.466145e+04 3.000000e+00
128 7.200000e-03 2.233073e+04 3.000000e+00
256 8.966667e-03 1.116536e+04 3.000000e+00
512 4.800000e-03 5.582682e+03 3.000000e+00
1024 4.533333e-03 2.791341e+03 3.000000e+00
2048 5.400000e-03 1.395670e+03 3.000000e+00
3072 4.933333e-03 9.304469e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0009_0.tex <==
8 6.584250e-01 2.826665e+06 4.000000e+00
16 3.316750e-01 1.413332e+06 4.000000e+00
32 3.132500e-01 7.066662e+05 4.000000e+00
64 1.057750e-01 3.533331e+05 4.000000e+00
128 6.705000e-02 1.766665e+05 4.000000e+00
256 2.717500e-02 8.833327e+04 4.000000e+00
512 1.497500e-02 4.416664e+04 4.000000e+00
1024 9.600000e-03 2.208332e+04 4.000000e+00
2048 8.575000e-03 1.104166e+04 4.000000e+00
3072 8.675000e-03 7.361106e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0009_1.tex <==
8 5.064667e-01 2.826665e+06 3.000000e+00
16 2.538667e-01 1.413332e+06 3.000000e+00
32 2.292000e-01 7.066662e+05 3.000000e+00
64 7.600000e-02 3.533331e+05 3.000000e+00
128 5.003333e-02 1.766665e+05 3.000000e+00
256 2.516667e-02 8.833327e+04 3.000000e+00
512 1.323333e-02 4.416664e+04 3.000000e+00
1024 8.666667e-03 2.208332e+04 3.000000e+00
2048 7.366667e-03 1.104166e+04 3.000000e+00
3072 6.400000e-03 7.361106e+03 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0010_0.tex <==
64 8.723750e-01 2.811284e+06 4.000000e+00
128 6.072250e-01 1.405642e+06 4.000000e+00
256 2.955500e-01 7.028210e+05 4.000000e+00
512 1.322500e-01 3.514105e+05 4.000000e+00
1024 6.610000e-02 1.757053e+05 4.000000e+00
2048 3.262500e-02 8.785263e+04 4.000000e+00
3072 2.152500e-02 5.856842e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0010_1.tex <==
64 1.116633e+00 2.811284e+06 3.000000e+00
128 4.650333e-01 1.405642e+06 3.000000e+00
256 2.538667e-01 7.028210e+05 3.000000e+00
512 1.109333e-01 3.514105e+05 3.000000e+00
1024 5.393333e-02 1.757053e+05 3.000000e+00
2048 2.820000e-02 8.785263e+04 3.000000e+00
3072 1.913333e-02 5.856842e+04 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0011_0.tex <==
1024 6.153500e-01 1.401853e+06 4.000000e+00
2048 3.048500e-01 7.009266e+05 4.000000e+00
3072 1.977250e-01 4.672844e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hmg-quadrant-4/data_0011_1.tex <==
1024 4.518333e-01 1.401853e+06 3.000000e+00
2048 2.289667e-01 7.009266e+05 3.000000e+00
3072 1.522667e-01 4.672844e+05 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0003_0.tex <==
1 6.250000e-04 1.936458e+02 4.000000e+00
2 6.500000e-04 9.682292e+01 4.000000e+00
4 7.000000e-04 4.841146e+01 4.000000e+00
8 6.750000e-04 2.420573e+01 4.000000e+00
16 7.000000e-04 1.210286e+01 4.000000e+00
32 1.025000e-03 6.051432e+00 4.000000e+00
64 7.250000e-04 3.025716e+00 4.000000e+00
128 7.250000e-04 1.512858e+00 4.000000e+00
256 7.500000e-04 7.564290e-01 4.000000e+00
512 8.000000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0003_1.tex <==
1 6.250000e-04 1.936458e+02 4.000000e+00
2 6.250000e-04 9.682292e+01 4.000000e+00
4 6.250000e-04 4.841146e+01 4.000000e+00
8 6.500000e-04 2.420573e+01 4.000000e+00
16 6.750000e-04 1.210286e+01 4.000000e+00
32 7.750000e-04 6.051432e+00 4.000000e+00
64 7.000000e-04 3.025716e+00 4.000000e+00
128 6.500000e-04 1.512858e+00 4.000000e+00
256 6.500000e-04 7.564290e-01 4.000000e+00
512 7.000000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0003_2.tex <==
1 6.000000e-04 1.936458e+02 4.000000e+00
2 6.250000e-04 9.682292e+01 4.000000e+00
4 6.250000e-04 4.841146e+01 4.000000e+00
8 6.500000e-04 2.420573e+01 4.000000e+00
16 6.500000e-04 1.210286e+01 4.000000e+00
32 6.750000e-04 6.051432e+00 4.000000e+00
64 6.750000e-04 3.025716e+00 4.000000e+00
128 7.500000e-04 1.512858e+00 4.000000e+00
256 7.500000e-04 7.564290e-01 4.000000e+00
512 7.250000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0003_3.tex <==
1 5.000000e-04 1.936458e+02 4.000000e+00
2 5.000000e-04 9.682292e+01 4.000000e+00
4 5.250000e-04 4.841146e+01 4.000000e+00
8 5.500000e-04 2.420573e+01 4.000000e+00
16 5.250000e-04 1.210286e+01 4.000000e+00
32 5.500000e-04 6.051432e+00 4.000000e+00
64 5.750000e-04 3.025716e+00 4.000000e+00
128 5.750000e-04 1.512858e+00 4.000000e+00
256 6.000000e-04 7.564290e-01 4.000000e+00
512 6.500000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0004_0.tex <==
1 1.075000e-03 1.053188e+03 4.000000e+00
2 1.050000e-03 5.265938e+02 4.000000e+00
4 1.075000e-03 2.632969e+02 4.000000e+00
8 1.325000e-03 1.316484e+02 4.000000e+00
16 1.125000e-03 6.582422e+01 4.000000e+00
32 1.125000e-03 3.291211e+01 4.000000e+00
64 1.175000e-03 1.645605e+01 4.000000e+00
128 1.200000e-03 8.228027e+00 4.000000e+00
256 1.225000e-03 4.114014e+00 4.000000e+00
512 1.225000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0004_1.tex <==
1 1.025000e-03 1.053188e+03 4.000000e+00
2 9.750000e-04 5.265938e+02 4.000000e+00
4 1.025000e-03 2.632969e+02 4.000000e+00
8 1.075000e-03 1.316484e+02 4.000000e+00
16 1.025000e-03 6.582422e+01 4.000000e+00
32 1.050000e-03 3.291211e+01 4.000000e+00
64 1.050000e-03 1.645605e+01 4.000000e+00
128 1.075000e-03 8.228027e+00 4.000000e+00
256 1.050000e-03 4.114014e+00 4.000000e+00
512 1.025000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0004_2.tex <==
1 1.300000e-03 1.053188e+03 4.000000e+00
2 1.225000e-03 5.265938e+02 4.000000e+00
4 1.200000e-03 2.632969e+02 4.000000e+00
8 1.275000e-03 1.316484e+02 4.000000e+00
16 1.275000e-03 6.582422e+01 4.000000e+00
32 1.300000e-03 3.291211e+01 4.000000e+00
64 1.300000e-03 1.645605e+01 4.000000e+00
128 1.350000e-03 8.228027e+00 4.000000e+00
256 1.375000e-03 4.114014e+00 4.000000e+00
512 1.450000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0004_3.tex <==
1 1.025000e-03 1.053188e+03 4.000000e+00
2 9.250000e-04 5.265938e+02 4.000000e+00
4 9.500000e-04 2.632969e+02 4.000000e+00
8 9.750000e-04 1.316484e+02 4.000000e+00
16 9.750000e-04 6.582422e+01 4.000000e+00
32 9.750000e-04 3.291211e+01 4.000000e+00
64 9.750000e-04 1.645605e+01 4.000000e+00
128 1.025000e-03 8.228027e+00 4.000000e+00
256 1.050000e-03 4.114014e+00 4.000000e+00
512 1.075000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0005_0.tex <==
1 2.175000e-03 6.692562e+03 4.000000e+00
2 1.800000e-03 3.346281e+03 4.000000e+00
4 1.725000e-03 1.673141e+03 4.000000e+00
8 1.750000e-03 8.365703e+02 4.000000e+00
16 1.600000e-03 4.182852e+02 4.000000e+00
32 1.750000e-03 2.091426e+02 4.000000e+00
64 1.675000e-03 1.045713e+02 4.000000e+00
128 1.700000e-03 5.228564e+01 4.000000e+00
256 1.750000e-03 2.614282e+01 4.000000e+00
512 1.800000e-03 1.307141e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0005_1.tex <==
1 2.033333e-03 6.692562e+03 3.000000e+00
2 1.733333e-03 3.346281e+03 3.000000e+00
4 1.666667e-03 1.673141e+03 3.000000e+00
8 1.666667e-03 8.365703e+02 3.000000e+00
16 1.600000e-03 4.182852e+02 3.000000e+00
32 1.600000e-03 2.091426e+02 3.000000e+00
64 1.533333e-03 1.045713e+02 3.000000e+00
128 1.600000e-03 5.228564e+01 3.000000e+00
256 1.600000e-03 2.614282e+01 3.000000e+00
512 1.500000e-03 1.307141e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0005_2.tex <==
1 2.175000e-03 6.692562e+03 4.000000e+00
2 2.100000e-03 3.346281e+03 4.000000e+00
4 1.950000e-03 1.673141e+03 4.000000e+00
8 2.275000e-03 8.365703e+02 4.000000e+00
16 1.900000e-03 4.182852e+02 4.000000e+00
32 1.850000e-03 2.091426e+02 4.000000e+00
64 1.800000e-03 1.045713e+02 4.000000e+00
128 1.725000e-03 5.228564e+01 4.000000e+00
256 1.800000e-03 2.614282e+01 4.000000e+00
512 1.800000e-03 1.307141e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0005_3.tex <==
1 1.900000e-03 6.692562e+03 4.000000e+00
2 1.675000e-03 3.346281e+03 4.000000e+00
4 1.525000e-03 1.673141e+03 4.000000e+00
8 1.700000e-03 8.365703e+02 4.000000e+00
16 1.525000e-03 4.182852e+02 4.000000e+00
32 3.350000e-03 2.091426e+02 4.000000e+00
64 1.300000e-03 1.045713e+02 4.000000e+00
128 1.325000e-03 5.228564e+01 4.000000e+00
256 1.300000e-03 2.614282e+01 4.000000e+00
512 1.350000e-03 1.307141e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0006_0.tex <==
1 1.022500e-02 4.802960e+04 4.000000e+00
2 5.775000e-03 2.401480e+04 4.000000e+00
4 3.750000e-03 1.200740e+04 4.000000e+00
8 4.150000e-03 6.003701e+03 4.000000e+00
16 2.500000e-03 3.001850e+03 4.000000e+00
32 2.850000e-03 1.500925e+03 4.000000e+00
64 2.750000e-03 7.504626e+02 4.000000e+00
128 2.825000e-03 3.752313e+02 4.000000e+00
256 2.900000e-03 1.876156e+02 4.000000e+00
512 2.600000e-03 9.380782e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0006_1.tex <==
1 7.766667e-03 4.802960e+04 3.000000e+00
2 4.400000e-03 2.401480e+04 3.000000e+00
4 3.366667e-03 1.200740e+04 3.000000e+00
8 3.033333e-03 6.003701e+03 3.000000e+00
16 2.366667e-03 3.001850e+03 3.000000e+00
32 4.533333e-03 1.500925e+03 3.000000e+00
64 2.300000e-03 7.504626e+02 3.000000e+00
128 2.433333e-03 3.752313e+02 3.000000e+00
256 2.433333e-03 1.876156e+02 3.000000e+00
512 2.366667e-03 9.380782e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0006_2.tex <==
1 7.975000e-03 4.802960e+04 4.000000e+00
2 4.725000e-03 2.401480e+04 4.000000e+00
4 3.475000e-03 1.200740e+04 4.000000e+00
8 2.975000e-03 6.003701e+03 4.000000e+00
16 2.675000e-03 3.001850e+03 4.000000e+00
32 2.600000e-03 1.500925e+03 4.000000e+00
64 2.575000e-03 7.504626e+02 4.000000e+00
128 2.600000e-03 3.752313e+02 4.000000e+00
256 2.425000e-03 1.876156e+02 4.000000e+00
512 2.250000e-03 9.380782e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0006_3.tex <==
1 7.625000e-03 4.802960e+04 4.000000e+00
2 4.525000e-03 2.401480e+04 4.000000e+00
4 3.025000e-03 1.200740e+04 4.000000e+00
8 2.675000e-03 6.003701e+03 4.000000e+00
16 2.200000e-03 3.001850e+03 4.000000e+00
32 2.100000e-03 1.500925e+03 4.000000e+00
64 2.525000e-03 7.504626e+02 4.000000e+00
128 1.925000e-03 3.752313e+02 4.000000e+00
256 1.975000e-03 1.876156e+02 4.000000e+00
512 1.750000e-03 9.380782e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0007_0.tex <==
1 8.192500e-02 3.656660e+05 4.000000e+00
2 3.940000e-02 1.828330e+05 4.000000e+00
4 2.040000e-02 9.141649e+04 4.000000e+00
8 1.090000e-02 4.570825e+04 4.000000e+00
16 6.400000e-03 2.285412e+04 4.000000e+00
32 9.475000e-03 1.142706e+04 4.000000e+00
64 5.050000e-03 5.713531e+03 4.000000e+00
128 4.050000e-03 2.856765e+03 4.000000e+00
256 4.400000e-03 1.428383e+03 4.000000e+00
512 4.450000e-03 7.141914e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0007_1.tex <==
1 6.413333e-02 3.656660e+05 3.000000e+00
2 3.123333e-02 1.828330e+05 3.000000e+00
4 1.650000e-02 9.141649e+04 3.000000e+00
8 8.600000e-03 4.570825e+04 3.000000e+00
16 5.266667e-03 2.285412e+04 3.000000e+00
32 4.533333e-03 1.142706e+04 3.000000e+00
64 3.766667e-03 5.713531e+03 3.000000e+00
128 3.333333e-03 2.856765e+03 3.000000e+00
256 3.466667e-03 1.428383e+03 3.000000e+00
512 3.800000e-03 7.141914e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0007_2.tex <==
1 6.285000e-02 3.656660e+05 4.000000e+00
2 3.067500e-02 1.828330e+05 4.000000e+00
4 1.590000e-02 9.141649e+04 4.000000e+00
8 1.077500e-02 4.570825e+04 4.000000e+00
16 5.550000e-03 2.285412e+04 4.000000e+00
32 4.500000e-03 1.142706e+04 4.000000e+00
64 3.800000e-03 5.713531e+03 4.000000e+00
128 5.050000e-03 2.856765e+03 4.000000e+00
256 4.075000e-03 1.428383e+03 4.000000e+00
512 4.000000e-03 7.141914e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0007_3.tex <==
1 6.157500e-02 3.656660e+05 4.000000e+00
2 2.957500e-02 1.828330e+05 4.000000e+00
4 1.520000e-02 9.141649e+04 4.000000e+00
8 8.425000e-03 4.570825e+04 4.000000e+00
16 5.050000e-03 2.285412e+04 4.000000e+00
32 5.375000e-03 1.142706e+04 4.000000e+00
64 3.150000e-03 5.713531e+03 4.000000e+00
128 3.475000e-03 2.856765e+03 4.000000e+00
256 3.650000e-03 1.428383e+03 4.000000e+00
512 3.000000e-03 7.141914e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0008_0.tex <==
1 6.385250e-01 2.858333e+06 4.000000e+00
2 3.157500e-01 1.429167e+06 4.000000e+00
4 1.752250e-01 7.145833e+05 4.000000e+00
8 8.257500e-02 3.572916e+05 4.000000e+00
16 4.232500e-02 1.786458e+05 4.000000e+00
32 2.277500e-02 8.932291e+04 4.000000e+00
64 1.150000e-02 4.466145e+04 4.000000e+00
128 7.825000e-03 2.233073e+04 4.000000e+00
256 6.475000e-03 1.116536e+04 4.000000e+00
512 6.375000e-03 5.582682e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0008_1.tex <==
1 4.898333e-01 2.858333e+06 3.000000e+00
2 2.470000e-01 1.429167e+06 3.000000e+00
4 1.447000e-01 7.145833e+05 3.000000e+00
8 6.576667e-02 3.572916e+05 3.000000e+00
16 3.383333e-02 1.786458e+05 3.000000e+00
32 1.876667e-02 8.932291e+04 3.000000e+00
64 1.066667e-02 4.466145e+04 3.000000e+00
128 6.933333e-03 2.233073e+04 3.000000e+00
256 5.400000e-03 1.116536e+04 3.000000e+00
512 5.000000e-03 5.582682e+03 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0008_2.tex <==
1 4.810500e-01 2.858333e+06 4.000000e+00
2 2.407750e-01 1.429167e+06 4.000000e+00
4 1.356000e-01 7.145833e+05 4.000000e+00
8 6.272500e-02 3.572916e+05 4.000000e+00
16 3.192500e-02 1.786458e+05 4.000000e+00
32 2.302500e-02 8.932291e+04 4.000000e+00
64 9.900000e-03 4.466145e+04 4.000000e+00
128 7.050000e-03 2.233073e+04 4.000000e+00
256 5.375000e-03 1.116536e+04 4.000000e+00
512 5.275000e-03 5.582682e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0008_3.tex <==
1 4.723000e-01 2.858333e+06 4.000000e+00
2 2.357250e-01 1.429167e+06 4.000000e+00
4 1.325250e-01 7.145833e+05 4.000000e+00
8 6.082500e-02 3.572916e+05 4.000000e+00
16 3.050000e-02 1.786458e+05 4.000000e+00
32 1.672500e-02 8.932291e+04 4.000000e+00
64 9.050000e-03 4.466145e+04 4.000000e+00
128 6.750000e-03 2.233073e+04 4.000000e+00
256 5.650000e-03 1.116536e+04 4.000000e+00
512 4.950000e-03 5.582682e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0009_0.tex <==
8 6.511500e-01 2.826665e+06 4.000000e+00
16 3.404500e-01 1.413332e+06 4.000000e+00
32 1.854500e-01 7.066662e+05 4.000000e+00
64 8.920000e-02 3.533331e+05 4.000000e+00
128 4.935000e-02 1.766665e+05 4.000000e+00
256 2.705000e-02 8.833327e+04 4.000000e+00
512 1.610000e-02 4.416664e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0009_1.tex <==
8 5.155667e-01 2.826665e+06 3.000000e+00
16 2.739333e-01 1.413332e+06 3.000000e+00
32 1.371333e-01 7.066662e+05 3.000000e+00
64 6.980000e-02 3.533331e+05 3.000000e+00
128 3.910000e-02 1.766665e+05 3.000000e+00
256 2.473333e-02 8.833327e+04 3.000000e+00
512 1.363333e-02 4.416664e+04 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0009_2.tex <==
8 4.862000e-01 2.826665e+06 4.000000e+00
16 2.530000e-01 1.413332e+06 4.000000e+00
32 1.363250e-01 7.066662e+05 4.000000e+00
64 6.165000e-02 3.533331e+05 4.000000e+00
128 3.805000e-02 1.766665e+05 4.000000e+00
256 2.142500e-02 8.833327e+04 4.000000e+00
512 1.280000e-02 4.416664e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0009_3.tex <==
8 4.781500e-01 2.826665e+06 4.000000e+00
16 2.479000e-01 1.413332e+06 4.000000e+00
32 1.314000e-01 7.066662e+05 4.000000e+00
64 6.022500e-02 3.533331e+05 4.000000e+00
128 3.562500e-02 1.766665e+05 4.000000e+00
256 2.122500e-02 8.833327e+04 4.000000e+00
512 1.197500e-02 4.416664e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0010_0.tex <==
64 6.858500e-01 2.811284e+06 4.000000e+00
128 4.047750e-01 1.405642e+06 4.000000e+00
256 2.597250e-01 7.028210e+05 4.000000e+00
512 1.416250e-01 3.514105e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0010_1.tex <==
64 8.611000e-01 2.811284e+06 3.000000e+00
128 2.985667e-01 1.405642e+06 3.000000e+00
256 2.194333e-01 7.028210e+05 3.000000e+00
512 1.116000e-01 3.514105e+05 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0010_2.tex <==
128 3.011750e-01 1.405642e+06 4.000000e+00
256 1.926000e-01 7.028210e+05 4.000000e+00
512 9.735000e-02 3.514105e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-new/data_0010_3.tex <==
128 2.934500e-01 1.405642e+06 4.000000e+00
256 1.886000e-01 7.028210e+05 4.000000e+00
512 9.357500e-02 3.514105e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0003_0.tex <==
1 5.750000e-04 1.936458e+02 4.000000e+00
2 6.500000e-04 9.682292e+01 4.000000e+00
4 6.500000e-04 4.841146e+01 4.000000e+00
8 7.000000e-04 2.420573e+01 4.000000e+00
16 7.000000e-04 1.210286e+01 4.000000e+00
32 7.250000e-04 6.051432e+00 4.000000e+00
64 7.250000e-04 3.025716e+00 4.000000e+00
128 8.000000e-04 1.512858e+00 4.000000e+00
256 8.250000e-04 7.564290e-01 4.000000e+00
512 8.250000e-04 3.782145e-01 4.000000e+00
1024 8.750000e-04 1.891073e-01 4.000000e+00
2048 1.000000e-03 9.455363e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0003_1.tex <==
1 5.000000e-04 1.936458e+02 4.000000e+00
2 5.500000e-04 9.682292e+01 4.000000e+00
4 5.500000e-04 4.841146e+01 4.000000e+00
8 5.750000e-04 2.420573e+01 4.000000e+00
16 5.750000e-04 1.210286e+01 4.000000e+00
32 5.750000e-04 6.051432e+00 4.000000e+00
64 5.750000e-04 3.025716e+00 4.000000e+00
128 6.000000e-04 1.512858e+00 4.000000e+00
256 6.250000e-04 7.564290e-01 4.000000e+00
512 6.500000e-04 3.782145e-01 4.000000e+00
1024 7.000000e-04 1.891073e-01 4.000000e+00
2048 6.750000e-04 9.455363e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0004_0.tex <==
1 1.250000e-03 1.053188e+03 4.000000e+00
2 1.350000e-03 5.265938e+02 4.000000e+00
4 1.300000e-03 2.632969e+02 4.000000e+00
8 1.350000e-03 1.316484e+02 4.000000e+00
16 1.350000e-03 6.582422e+01 4.000000e+00
32 1.400000e-03 3.291211e+01 4.000000e+00
64 1.375000e-03 1.645605e+01 4.000000e+00
128 1.500000e-03 8.228027e+00 4.000000e+00
256 1.475000e-03 4.114014e+00 4.000000e+00
512 1.525000e-03 2.057007e+00 4.000000e+00
1024 1.500000e-03 1.028503e+00 4.000000e+00
2048 1.575000e-03 5.142517e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0004_1.tex <==
1 9.750000e-04 1.053188e+03 4.000000e+00
2 1.000000e-03 5.265938e+02 4.000000e+00
4 9.500000e-04 2.632969e+02 4.000000e+00
8 1.025000e-03 1.316484e+02 4.000000e+00
16 1.025000e-03 6.582422e+01 4.000000e+00
32 1.050000e-03 3.291211e+01 4.000000e+00
64 1.075000e-03 1.645605e+01 4.000000e+00
128 1.075000e-03 8.228027e+00 4.000000e+00
256 1.100000e-03 4.114014e+00 4.000000e+00
512 1.100000e-03 2.057007e+00 4.000000e+00
1024 1.100000e-03 1.028503e+00 4.000000e+00
2048 1.150000e-03 5.142517e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0005_0.tex <==
1 2.100000e-03 6.692562e+03 4.000000e+00
2 2.275000e-03 3.346281e+03 4.000000e+00
4 2.075000e-03 1.673141e+03 4.000000e+00
8 2.250000e-03 8.365703e+02 4.000000e+00
16 2.125000e-03 4.182852e+02 4.000000e+00
32 1.900000e-03 2.091426e+02 4.000000e+00
64 1.800000e-03 1.045713e+02 4.000000e+00
128 1.875000e-03 5.228564e+01 4.000000e+00
256 2.000000e-03 2.614282e+01 4.000000e+00
512 1.875000e-03 1.307141e+01 4.000000e+00
1024 2.000000e-03 6.535706e+00 4.000000e+00
2048 2.075000e-03 3.267853e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0005_1.tex <==
1 1.825000e-03 6.692562e+03 4.000000e+00
2 1.750000e-03 3.346281e+03 4.000000e+00
4 1.575000e-03 1.673141e+03 4.000000e+00
8 1.725000e-03 8.365703e+02 4.000000e+00
16 1.600000e-03 4.182852e+02 4.000000e+00
32 1.375000e-03 2.091426e+02 4.000000e+00
64 1.375000e-03 1.045713e+02 4.000000e+00
128 1.400000e-03 5.228564e+01 4.000000e+00
256 1.325000e-03 2.614282e+01 4.000000e+00
512 1.400000e-03 1.307141e+01 4.000000e+00
1024 1.400000e-03 6.535706e+00 4.000000e+00
2048 1.450000e-03 3.267853e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0006_0.tex <==
1 8.275000e-03 4.802960e+04 4.000000e+00
2 5.350000e-03 2.401480e+04 4.000000e+00
4 3.800000e-03 1.200740e+04 4.000000e+00
8 3.125000e-03 6.003701e+03 4.000000e+00
16 2.975000e-03 3.001850e+03 4.000000e+00
32 2.775000e-03 1.500925e+03 4.000000e+00
64 2.725000e-03 7.504626e+02 4.000000e+00
128 2.475000e-03 3.752313e+02 4.000000e+00
256 2.675000e-03 1.876156e+02 4.000000e+00
512 2.450000e-03 9.380782e+01 4.000000e+00
1024 2.500000e-03 4.690391e+01 4.000000e+00
2048 2.700000e-03 2.345196e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0006_1.tex <==
1 9.675000e-03 4.802960e+04 4.000000e+00
2 4.875000e-03 2.401480e+04 4.000000e+00
4 3.275000e-03 1.200740e+04 4.000000e+00
8 2.575000e-03 6.003701e+03 4.000000e+00
16 2.300000e-03 3.001850e+03 4.000000e+00
32 2.150000e-03 1.500925e+03 4.000000e+00
64 2.050000e-03 7.504626e+02 4.000000e+00
128 1.950000e-03 3.752313e+02 4.000000e+00
256 1.975000e-03 1.876156e+02 4.000000e+00
512 1.825000e-03 9.380782e+01 4.000000e+00
1024 1.800000e-03 4.690391e+01 4.000000e+00
2048 1.775000e-03 2.345196e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0007_0.tex <==
1 6.430000e-02 3.656660e+05 4.000000e+00
2 3.252500e-02 1.828330e+05 4.000000e+00
4 1.642500e-02 9.141649e+04 4.000000e+00
8 9.100000e-03 4.570825e+04 4.000000e+00
16 6.225000e-03 2.285412e+04 4.000000e+00
32 4.825000e-03 1.142706e+04 4.000000e+00
64 4.300000e-03 5.713531e+03 4.000000e+00
128 4.950000e-03 2.856765e+03 4.000000e+00
256 4.125000e-03 1.428383e+03 4.000000e+00
512 3.725000e-03 7.141914e+02 4.000000e+00
1024 3.125000e-03 3.570957e+02 4.000000e+00
2048 3.075000e-03 1.785478e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0007_1.tex <==
1 6.227500e-02 3.656660e+05 4.000000e+00
2 3.082500e-02 1.828330e+05 4.000000e+00
4 1.530000e-02 9.141649e+04 4.000000e+00
8 8.400000e-03 4.570825e+04 4.000000e+00
16 5.500000e-03 2.285412e+04 4.000000e+00
32 4.000000e-03 1.142706e+04 4.000000e+00
64 3.550000e-03 5.713531e+03 4.000000e+00
128 3.650000e-03 2.856765e+03 4.000000e+00
256 3.425000e-03 1.428383e+03 4.000000e+00
512 2.825000e-03 7.141914e+02 4.000000e+00
1024 3.125000e-03 3.570957e+02 4.000000e+00
2048 2.725000e-03 1.785478e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0008_0.tex <==
1 4.937250e-01 2.858333e+06 4.000000e+00
2 2.545250e-01 1.429167e+06 4.000000e+00
4 1.316000e-01 7.145833e+05 4.000000e+00
8 6.440000e-02 3.572916e+05 4.000000e+00
16 3.890000e-02 1.786458e+05 4.000000e+00
32 2.097500e-02 8.932291e+04 4.000000e+00
64 1.130000e-02 4.466145e+04 4.000000e+00
128 7.850000e-03 2.233073e+04 4.000000e+00
256 5.725000e-03 1.116536e+04 4.000000e+00
512 5.550000e-03 5.582682e+03 4.000000e+00
1024 6.600000e-03 2.791341e+03 4.000000e+00
2048 6.100000e-03 1.395670e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0008_1.tex <==
1 4.806000e-01 2.858333e+06 4.000000e+00
2 2.476000e-01 1.429167e+06 4.000000e+00
4 1.268500e-01 7.145833e+05 4.000000e+00
8 6.155000e-02 3.572916e+05 4.000000e+00
16 3.690000e-02 1.786458e+05 4.000000e+00
32 1.925000e-02 8.932291e+04 4.000000e+00
64 1.062500e-02 4.466145e+04 4.000000e+00
128 6.350000e-03 2.233073e+04 4.000000e+00
256 5.400000e-03 1.116536e+04 4.000000e+00
512 4.825000e-03 5.582682e+03 4.000000e+00
1024 4.725000e-03 2.791341e+03 4.000000e+00
2048 4.850000e-03 1.395670e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0009_0.tex <==
8 5.017750e-01 2.826665e+06 4.000000e+00
16 3.197750e-01 1.413332e+06 4.000000e+00
32 1.982250e-01 7.066662e+05 4.000000e+00
64 9.617500e-02 3.533331e+05 4.000000e+00
128 4.650000e-02 1.766665e+05 4.000000e+00
256 1.967500e-02 8.833327e+04 4.000000e+00
512 1.207500e-02 4.416664e+04 4.000000e+00
1024 9.325000e-03 2.208332e+04 4.000000e+00
2048 8.575000e-03 1.104166e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0009_1.tex <==
8 4.879750e-01 2.826665e+06 4.000000e+00
16 3.118250e-01 1.413332e+06 4.000000e+00
32 1.931000e-01 7.066662e+05 4.000000e+00
64 9.330000e-02 3.533331e+05 4.000000e+00
128 4.372500e-02 1.766665e+05 4.000000e+00
256 1.792500e-02 8.833327e+04 4.000000e+00
512 1.120000e-02 4.416664e+04 4.000000e+00
1024 7.825000e-03 2.208332e+04 4.000000e+00
2048 7.800000e-03 1.104166e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0010_0.tex <==
128 3.979000e-01 1.405642e+06 4.000000e+00
256 1.617500e-01 7.028210e+05 4.000000e+00
512 9.550000e-02 3.514105e+05 4.000000e+00
1024 3.487500e-02 1.757053e+05 4.000000e+00
2048 2.087500e-02 8.785263e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0010_1.tex <==
128 3.893750e-01 1.405642e+06 4.000000e+00
256 1.555250e-01 7.028210e+05 4.000000e+00
512 9.120000e-02 3.514105e+05 4.000000e+00
1024 3.530000e-02 1.757053e+05 4.000000e+00
2048 1.925000e-02 8.785263e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0011_0.tex <==
1024 4.165250e-01 1.401853e+06 4.000000e+00
2048 1.695500e-01 7.009266e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant-old/data_0011_1.tex <==
1024 5.022750e-01 1.401853e+06 4.000000e+00
2048 1.603250e-01 7.009266e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0003_0.tex <==
1 2.250000e-04 4.645833e+00 4.000000e+00
2 2.500000e-04 2.322917e+00 4.000000e+00
4 2.250000e-04 1.161458e+00 4.000000e+00
8 2.500000e-04 5.807292e-01 4.000000e+00
16 2.500000e-04 2.903646e-01 4.000000e+00
32 2.750000e-04 1.451823e-01 4.000000e+00
64 3.000000e-04 7.259115e-02 4.000000e+00
128 3.000000e-04 3.629557e-02 4.000000e+00
256 3.000000e-04 1.814779e-02 4.000000e+00
512 3.250000e-04 9.073893e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0003_1.tex <==
1 5.750000e-04 1.936458e+02 4.000000e+00
2 6.250000e-04 9.682292e+01 4.000000e+00
4 6.250000e-04 4.841146e+01 4.000000e+00
8 6.750000e-04 2.420573e+01 4.000000e+00
16 6.750000e-04 1.210286e+01 4.000000e+00
32 7.250000e-04 6.051432e+00 4.000000e+00
64 7.250000e-04 3.025716e+00 4.000000e+00
128 8.000000e-04 1.512858e+00 4.000000e+00
256 7.750000e-04 7.564290e-01 4.000000e+00
512 7.750000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0003_2.tex <==
1 5.750000e-04 1.936458e+02 4.000000e+00
2 6.250000e-04 9.682292e+01 4.000000e+00
4 6.250000e-04 4.841146e+01 4.000000e+00
8 6.500000e-04 2.420573e+01 4.000000e+00
16 6.500000e-04 1.210286e+01 4.000000e+00
32 6.750000e-04 6.051432e+00 4.000000e+00
64 7.000000e-04 3.025716e+00 4.000000e+00
128 8.250000e-04 1.512858e+00 4.000000e+00
256 6.750000e-04 7.564290e-01 4.000000e+00
512 6.750000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0003_3.tex <==
1 5.750000e-04 1.936458e+02 4.000000e+00
2 6.250000e-04 9.682292e+01 4.000000e+00
4 6.500000e-04 4.841146e+01 4.000000e+00
8 6.500000e-04 2.420573e+01 4.000000e+00
16 6.500000e-04 1.210286e+01 4.000000e+00
32 7.000000e-04 6.051432e+00 4.000000e+00
64 7.250000e-04 3.025716e+00 4.000000e+00
128 7.500000e-04 1.512858e+00 4.000000e+00
256 7.750000e-04 7.564290e-01 4.000000e+00
512 7.750000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0003_4.tex <==
1 5.000000e-04 1.936458e+02 4.000000e+00
2 5.250000e-04 9.682292e+01 4.000000e+00
4 5.250000e-04 4.841146e+01 4.000000e+00
8 5.500000e-04 2.420573e+01 4.000000e+00
16 5.250000e-04 1.210286e+01 4.000000e+00
32 5.500000e-04 6.051432e+00 4.000000e+00
64 5.750000e-04 3.025716e+00 4.000000e+00
128 5.750000e-04 1.512858e+00 4.000000e+00
256 6.750000e-04 7.564290e-01 4.000000e+00
512 6.000000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0004_0.tex <==
1 4.000000e-04 2.100000e+01 4.000000e+00
2 4.000000e-04 1.050000e+01 4.000000e+00
4 4.000000e-04 5.250000e+00 4.000000e+00
8 4.250000e-04 2.625000e+00 4.000000e+00
16 4.500000e-04 1.312500e+00 4.000000e+00
32 4.750000e-04 6.562500e-01 4.000000e+00
64 4.750000e-04 3.281250e-01 4.000000e+00
128 4.750000e-04 1.640625e-01 4.000000e+00
256 4.750000e-04 8.203125e-02 4.000000e+00
512 5.000000e-04 4.101562e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0004_1.tex <==
1 1.075000e-03 1.053188e+03 4.000000e+00
2 1.075000e-03 5.265938e+02 4.000000e+00
4 1.050000e-03 2.632969e+02 4.000000e+00
8 1.100000e-03 1.316484e+02 4.000000e+00
16 1.125000e-03 6.582422e+01 4.000000e+00
32 1.150000e-03 3.291211e+01 4.000000e+00
64 1.150000e-03 1.645605e+01 4.000000e+00
128 1.200000e-03 8.228027e+00 4.000000e+00
256 1.275000e-03 4.114014e+00 4.000000e+00
512 1.175000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0004_2.tex <==
1 1.050000e-03 1.053188e+03 4.000000e+00
2 9.750000e-04 5.265938e+02 4.000000e+00
4 9.500000e-04 2.632969e+02 4.000000e+00
8 1.000000e-03 1.316484e+02 4.000000e+00
16 1.025000e-03 6.582422e+01 4.000000e+00
32 1.025000e-03 3.291211e+01 4.000000e+00
64 1.075000e-03 1.645605e+01 4.000000e+00
128 1.050000e-03 8.228027e+00 4.000000e+00
256 1.025000e-03 4.114014e+00 4.000000e+00
512 1.050000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0004_3.tex <==
1 1.300000e-03 1.053188e+03 4.000000e+00
2 1.250000e-03 5.265938e+02 4.000000e+00
4 1.175000e-03 2.632969e+02 4.000000e+00
8 1.375000e-03 1.316484e+02 4.000000e+00
16 1.300000e-03 6.582422e+01 4.000000e+00
32 1.325000e-03 3.291211e+01 4.000000e+00
64 1.325000e-03 1.645605e+01 4.000000e+00
128 1.375000e-03 8.228027e+00 4.000000e+00
256 1.400000e-03 4.114014e+00 4.000000e+00
512 1.375000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0004_4.tex <==
1 1.000000e-03 1.053188e+03 4.000000e+00
2 9.250000e-04 5.265938e+02 4.000000e+00
4 9.000000e-04 2.632969e+02 4.000000e+00
8 1.000000e-03 1.316484e+02 4.000000e+00
16 1.000000e-03 6.582422e+01 4.000000e+00
32 1.100000e-03 3.291211e+01 4.000000e+00
64 1.000000e-03 1.645605e+01 4.000000e+00
128 1.050000e-03 8.228027e+00 4.000000e+00
256 1.175000e-03 4.114014e+00 4.000000e+00
512 1.050000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0005_0.tex <==
1 6.000000e-04 1.188125e+02 4.000000e+00
2 6.250000e-04 5.940625e+01 4.000000e+00
4 6.250000e-04 2.970312e+01 4.000000e+00
8 6.750000e-04 1.485156e+01 4.000000e+00
16 6.500000e-04 7.425781e+00 4.000000e+00
32 6.500000e-04 3.712891e+00 4.000000e+00
64 6.750000e-04 1.856445e+00 4.000000e+00
128 7.000000e-04 9.282227e-01 4.000000e+00
256 7.000000e-04 4.641113e-01 4.000000e+00
512 7.250000e-04 2.320557e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0005_1.tex <==
1 2.175000e-03 6.692562e+03 4.000000e+00
2 1.850000e-03 3.346281e+03 4.000000e+00
4 1.725000e-03 1.673141e+03 4.000000e+00
8 1.725000e-03 8.365703e+02 4.000000e+00
16 1.600000e-03 4.182852e+02 4.000000e+00
32 1.675000e-03 2.091426e+02 4.000000e+00
64 1.625000e-03 1.045713e+02 4.000000e+00
128 1.800000e-03 5.228564e+01 4.000000e+00
256 1.775000e-03 2.614282e+01 4.000000e+00
512 1.700000e-03 1.307141e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0005_2.tex <==
1 1.966667e-03 6.692562e+03 3.000000e+00
2 1.766667e-03 3.346281e+03 3.000000e+00
4 1.633333e-03 1.673141e+03 3.000000e+00
8 1.666667e-03 8.365703e+02 3.000000e+00
16 1.600000e-03 4.182852e+02 3.000000e+00
32 1.533333e-03 2.091426e+02 3.000000e+00
64 1.633333e-03 1.045713e+02 3.000000e+00
128 1.866667e-03 5.228564e+01 3.000000e+00
256 1.666667e-03 2.614282e+01 3.000000e+00
512 1.500000e-03 1.307141e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0005_3.tex <==
1 2.125000e-03 6.692562e+03 4.000000e+00
2 2.100000e-03 3.346281e+03 4.000000e+00
4 2.000000e-03 1.673141e+03 4.000000e+00
8 2.125000e-03 8.365703e+02 4.000000e+00
16 1.900000e-03 4.182852e+02 4.000000e+00
32 1.750000e-03 2.091426e+02 4.000000e+00
64 1.675000e-03 1.045713e+02 4.000000e+00
128 1.750000e-03 5.228564e+01 4.000000e+00
256 1.750000e-03 2.614282e+01 4.000000e+00
512 1.775000e-03 1.307141e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0005_4.tex <==
1 1.875000e-03 6.692562e+03 4.000000e+00
2 1.675000e-03 3.346281e+03 4.000000e+00
4 1.525000e-03 1.673141e+03 4.000000e+00
8 1.675000e-03 8.365703e+02 4.000000e+00
16 1.525000e-03 4.182852e+02 4.000000e+00
32 1.325000e-03 2.091426e+02 4.000000e+00
64 1.275000e-03 1.045713e+02 4.000000e+00
128 1.350000e-03 5.228564e+01 4.000000e+00
256 1.275000e-03 2.614282e+01 4.000000e+00
512 1.300000e-03 1.307141e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0006_0.tex <==
1 1.125000e-03 8.000417e+02 4.000000e+00
2 1.025000e-03 4.000208e+02 4.000000e+00
4 9.500000e-04 2.000104e+02 4.000000e+00
8 9.750000e-04 1.000052e+02 4.000000e+00
16 1.000000e-03 5.000260e+01 4.000000e+00
32 1.025000e-03 2.500130e+01 4.000000e+00
64 1.125000e-03 1.250065e+01 4.000000e+00
128 1.075000e-03 6.250326e+00 4.000000e+00
256 1.000000e-03 3.125163e+00 4.000000e+00
512 1.050000e-03 1.562581e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0006_1.tex <==
1 9.750000e-03 4.802960e+04 4.000000e+00
2 5.875000e-03 2.401480e+04 4.000000e+00
4 3.725000e-03 1.200740e+04 4.000000e+00
8 2.850000e-03 6.003701e+03 4.000000e+00
16 2.475000e-03 3.001850e+03 4.000000e+00
32 2.775000e-03 1.500925e+03 4.000000e+00
64 2.775000e-03 7.504626e+02 4.000000e+00
128 2.950000e-03 3.752313e+02 4.000000e+00
256 2.500000e-03 1.876156e+02 4.000000e+00
512 2.750000e-03 9.380782e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0006_2.tex <==
1 7.366667e-03 4.802960e+04 3.000000e+00
2 4.400000e-03 2.401480e+04 3.000000e+00
4 3.300000e-03 1.200740e+04 3.000000e+00
8 2.733333e-03 6.003701e+03 3.000000e+00
16 2.400000e-03 3.001850e+03 3.000000e+00
32 2.200000e-03 1.500925e+03 3.000000e+00
64 2.466667e-03 7.504626e+02 3.000000e+00
128 2.300000e-03 3.752313e+02 3.000000e+00
256 2.133333e-03 1.876156e+02 3.000000e+00
512 2.233333e-03 9.380782e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0006_3.tex <==
1 7.925000e-03 4.802960e+04 4.000000e+00
2 4.800000e-03 2.401480e+04 4.000000e+00
4 3.475000e-03 1.200740e+04 4.000000e+00
8 2.925000e-03 6.003701e+03 4.000000e+00
16 2.750000e-03 3.001850e+03 4.000000e+00
32 2.675000e-03 1.500925e+03 4.000000e+00
64 2.600000e-03 7.504626e+02 4.000000e+00
128 2.350000e-03 3.752313e+02 4.000000e+00
256 2.400000e-03 1.876156e+02 4.000000e+00
512 2.300000e-03 9.380782e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0006_4.tex <==
1 7.675000e-03 4.802960e+04 4.000000e+00
2 4.525000e-03 2.401480e+04 4.000000e+00
4 3.025000e-03 1.200740e+04 4.000000e+00
8 2.450000e-03 6.003701e+03 4.000000e+00
16 2.300000e-03 3.001850e+03 4.000000e+00
32 2.200000e-03 1.500925e+03 4.000000e+00
64 2.100000e-03 7.504626e+02 4.000000e+00
128 1.875000e-03 3.752313e+02 4.000000e+00
256 1.950000e-03 1.876156e+02 4.000000e+00
512 1.825000e-03 9.380782e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0007_0.tex <==
1 3.700000e-03 5.898104e+03 3.000000e+00
2 2.433333e-03 2.949052e+03 3.000000e+00
4 1.833333e-03 1.474526e+03 3.000000e+00
8 1.600000e-03 7.372630e+02 3.000000e+00
16 1.566667e-03 3.686315e+02 3.000000e+00
32 1.533333e-03 1.843158e+02 3.000000e+00
64 1.666667e-03 9.215788e+01 3.000000e+00
128 1.800000e-03 4.607894e+01 3.000000e+00
256 2.566667e-03 2.303947e+01 3.000000e+00
512 2.133333e-03 1.151973e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0007_1.tex <==
1 7.792500e-02 3.656660e+05 4.000000e+00
2 3.917500e-02 1.828330e+05 4.000000e+00
4 1.922500e-02 9.141649e+04 4.000000e+00
8 1.085000e-02 4.570825e+04 4.000000e+00
16 6.900000e-03 2.285412e+04 4.000000e+00
32 4.800000e-03 1.142706e+04 4.000000e+00
64 4.300000e-03 5.713531e+03 4.000000e+00
128 4.300000e-03 2.856765e+03 4.000000e+00
256 4.225000e-03 1.428383e+03 4.000000e+00
512 4.175000e-03 7.141914e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0007_2.tex <==
1 6.166667e-02 3.656660e+05 3.000000e+00
2 3.126667e-02 1.828330e+05 3.000000e+00
4 1.506667e-02 9.141649e+04 3.000000e+00
8 8.066667e-03 4.570825e+04 3.000000e+00
16 5.966667e-03 2.285412e+04 3.000000e+00
32 4.600000e-03 1.142706e+04 3.000000e+00
64 3.900000e-03 5.713531e+03 3.000000e+00
128 3.333333e-03 2.856765e+03 3.000000e+00
256 3.433333e-03 1.428383e+03 3.000000e+00
512 3.600000e-03 7.141914e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0007_3.tex <==
1 6.050000e-02 3.656660e+05 4.000000e+00
2 3.057500e-02 1.828330e+05 4.000000e+00
4 1.492500e-02 9.141649e+04 4.000000e+00
8 8.625000e-03 4.570825e+04 4.000000e+00
16 5.875000e-03 2.285412e+04 4.000000e+00
32 4.500000e-03 1.142706e+04 4.000000e+00
64 3.800000e-03 5.713531e+03 4.000000e+00
128 5.150000e-03 2.856765e+03 4.000000e+00
256 4.000000e-03 1.428383e+03 4.000000e+00
512 3.550000e-03 7.141914e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0007_4.tex <==
1 5.912500e-02 3.656660e+05 4.000000e+00
2 2.955000e-02 1.828330e+05 4.000000e+00
4 1.427500e-02 9.141649e+04 4.000000e+00
8 8.150000e-03 4.570825e+04 4.000000e+00
16 5.325000e-03 2.285412e+04 4.000000e+00
32 3.925000e-03 1.142706e+04 4.000000e+00
64 3.275000e-03 5.713531e+03 4.000000e+00
128 3.550000e-03 2.856765e+03 4.000000e+00
256 3.900000e-03 1.428383e+03 4.000000e+00
512 3.025000e-03 7.141914e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0008_0.tex <==
1 2.120000e-02 4.537383e+04 3.000000e+00
2 1.173333e-02 2.268692e+04 3.000000e+00
4 6.733333e-03 1.134346e+04 3.000000e+00
8 4.233333e-03 5.671729e+03 3.000000e+00
16 3.133333e-03 2.835865e+03 3.000000e+00
32 2.433333e-03 1.417932e+03 3.000000e+00
64 2.633333e-03 7.089661e+02 3.000000e+00
128 2.433333e-03 3.544831e+02 3.000000e+00
256 2.566667e-03 1.772415e+02 3.000000e+00
512 2.966667e-03 8.862077e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0008_1.tex <==
1 6.057750e-01 2.858333e+06 4.000000e+00
2 3.138250e-01 1.429167e+06 4.000000e+00
4 1.595250e-01 7.145833e+05 4.000000e+00
8 8.065000e-02 3.572916e+05 4.000000e+00
16 5.857500e-02 1.786458e+05 4.000000e+00
32 2.450000e-02 8.932291e+04 4.000000e+00
64 1.372500e-02 4.466145e+04 4.000000e+00
128 8.900000e-03 2.233073e+04 4.000000e+00
256 6.675000e-03 1.116536e+04 4.000000e+00
512 6.650000e-03 5.582682e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0008_2.tex <==
1 4.714333e-01 2.858333e+06 3.000000e+00
2 2.468000e-01 1.429167e+06 3.000000e+00
4 1.259667e-01 7.145833e+05 3.000000e+00
8 6.400000e-02 3.572916e+05 3.000000e+00
16 4.450000e-02 1.786458e+05 3.000000e+00
32 2.066667e-02 8.932291e+04 3.000000e+00
64 1.260000e-02 4.466145e+04 3.000000e+00
128 7.466667e-03 2.233073e+04 3.000000e+00
256 6.233333e-03 1.116536e+04 3.000000e+00
512 4.866667e-03 5.582682e+03 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0008_3.tex <==
1 4.630750e-01 2.858333e+06 4.000000e+00
2 2.401250e-01 1.429167e+06 4.000000e+00
4 1.217250e-01 7.145833e+05 4.000000e+00
8 6.145000e-02 3.572916e+05 4.000000e+00
16 4.457500e-02 1.786458e+05 4.000000e+00
32 1.920000e-02 8.932291e+04 4.000000e+00
64 1.085000e-02 4.466145e+04 4.000000e+00
128 8.375000e-03 2.233073e+04 4.000000e+00
256 5.850000e-03 1.116536e+04 4.000000e+00
512 5.800000e-03 5.582682e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0008_4.tex <==
1 4.558750e-01 2.858333e+06 4.000000e+00
2 2.352000e-01 1.429167e+06 4.000000e+00
4 1.184000e-01 7.145833e+05 4.000000e+00
8 5.910000e-02 3.572916e+05 4.000000e+00
16 4.302500e-02 1.786458e+05 4.000000e+00
32 1.817500e-02 8.932291e+04 4.000000e+00
64 1.017500e-02 4.466145e+04 4.000000e+00
128 6.800000e-03 2.233073e+04 4.000000e+00
256 5.225000e-03 1.116536e+04 4.000000e+00
512 5.350000e-03 5.582682e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0009_0.tex <==
1 1.476000e-01 3.561329e+05 3.000000e+00
2 7.826667e-02 1.780664e+05 3.000000e+00
4 3.993333e-02 8.903322e+04 3.000000e+00
8 2.123333e-02 4.451661e+04 3.000000e+00
16 1.300000e-02 2.225831e+04 3.000000e+00
32 7.733333e-03 1.112915e+04 3.000000e+00
64 5.133333e-03 5.564576e+03 3.000000e+00
128 4.200000e-03 2.782288e+03 3.000000e+00
256 3.366667e-03 1.391144e+03 3.000000e+00
512 3.766667e-03 6.955721e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0009_1.tex <==
8 6.298000e-01 2.826665e+06 4.000000e+00
16 4.989750e-01 1.413332e+06 4.000000e+00
32 2.401250e-01 7.066662e+05 4.000000e+00
64 1.387000e-01 3.533331e+05 4.000000e+00
128 5.967500e-02 1.766665e+05 4.000000e+00
256 3.172500e-02 8.833327e+04 4.000000e+00
512 1.535000e-02 4.416664e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0009_2.tex <==
8 4.952000e-01 2.826665e+06 3.000000e+00
16 4.030333e-01 1.413332e+06 3.000000e+00
32 2.035000e-01 7.066662e+05 3.000000e+00
64 1.053667e-01 3.533331e+05 3.000000e+00
128 4.900000e-02 1.766665e+05 3.000000e+00
256 2.566667e-02 8.833327e+04 3.000000e+00
512 1.370000e-02 4.416664e+04 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0009_3.tex <==
8 4.747750e-01 2.826665e+06 4.000000e+00
16 3.827250e-01 1.413332e+06 4.000000e+00
32 1.872000e-01 7.066662e+05 4.000000e+00
64 9.572500e-02 3.533331e+05 4.000000e+00
128 4.487500e-02 1.766665e+05 4.000000e+00
256 2.352500e-02 8.833327e+04 4.000000e+00
512 1.385000e-02 4.416664e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0009_4.tex <==
8 4.659000e-01 2.826665e+06 4.000000e+00
16 3.765000e-01 1.413332e+06 4.000000e+00
32 1.838000e-01 7.066662e+05 4.000000e+00
64 9.245000e-02 3.533331e+05 4.000000e+00
128 4.372500e-02 1.766665e+05 4.000000e+00
256 2.050000e-02 8.833327e+04 4.000000e+00
512 1.240000e-02 4.416664e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0010_0.tex <==
8 1.608500e-01 3.527983e+05 2.000000e+00
16 9.635000e-02 1.763992e+05 2.000000e+00
32 4.455000e-02 8.819958e+04 2.000000e+00
64 2.495000e-02 4.409979e+04 2.000000e+00
128 1.470000e-02 2.204990e+04 2.000000e+00
256 9.800000e-03 1.102495e+04 2.000000e+00
512 7.050000e-03 5.512474e+03 2.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0010_1.tex <==
64 1.102175e+00 2.811284e+06 4.000000e+00
128 5.123250e-01 1.405642e+06 4.000000e+00
256 2.623250e-01 7.028210e+05 4.000000e+00
512 1.441250e-01 3.514105e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0010_2.tex <==
64 1.476133e+00 2.811284e+06 3.000000e+00
128 4.231333e-01 1.405642e+06 3.000000e+00
256 2.197667e-01 7.028210e+05 3.000000e+00
512 1.121000e-01 3.514105e+05 3.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0010_3.tex <==
128 3.846750e-01 1.405642e+06 4.000000e+00
256 1.977000e-01 7.028210e+05 4.000000e+00
512 9.690000e-02 3.514105e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0010_4.tex <==
128 3.761500e-01 1.405642e+06 4.000000e+00
256 1.903500e-01 7.028210e+05 4.000000e+00
512 9.697500e-02 3.514105e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-new/hpmg-quadrant/data_0011_0.tex <==
128 9.570000e-02 1.755771e+05 2.000000e+00
256 5.130000e-02 8.778855e+04 2.000000e+00
512 2.895000e-02 4.389428e+04 2.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0005_0.tex <==
1 7.000000e-04 4.093750e+01 5.000000e+00
2 8.400000e-04 2.046875e+01 5.000000e+00
4 9.000000e-04 1.023438e+01 5.000000e+00
8 1.140000e-03 5.117188e+00 5.000000e+00
16 9.200000e-04 2.558594e+00 5.000000e+00
32 9.200000e-04 1.279297e+00 5.000000e+00
64 9.600000e-04 6.396484e-01 5.000000e+00
128 1.160000e-03 3.198242e-01 5.000000e+00
256 1.020000e-03 1.599121e-01 5.000000e+00
512 1.060000e-03 7.995605e-02 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0005_1.tex <==
1 5.750000e-04 4.093750e+01 4.000000e+00
2 7.000000e-04 2.046875e+01 4.000000e+00
4 7.500000e-04 1.023438e+01 4.000000e+00
8 7.250000e-04 5.117188e+00 4.000000e+00
16 7.000000e-04 2.558594e+00 4.000000e+00
32 7.250000e-04 1.279297e+00 4.000000e+00
64 7.250000e-04 6.396484e-01 4.000000e+00
128 1.000000e-03 3.198242e-01 4.000000e+00
256 7.750000e-04 1.599121e-01 4.000000e+00
512 8.000000e-04 7.995605e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0005_2.tex <==
1 7.250000e-04 4.093750e+01 4.000000e+00
2 8.000000e-04 2.046875e+01 4.000000e+00
4 9.750000e-04 1.023438e+01 4.000000e+00
8 1.800000e-03 5.117188e+00 4.000000e+00
16 1.050000e-03 2.558594e+00 4.000000e+00
32 1.000000e-03 1.279297e+00 4.000000e+00
64 1.050000e-03 6.396484e-01 4.000000e+00
128 2.925000e-03 3.198242e-01 4.000000e+00
256 1.000000e-03 1.599121e-01 4.000000e+00
512 1.025000e-03 7.995605e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0006_0.tex <==
1 9.800000e-04 2.033958e+02 5.000000e+00
2 1.120000e-03 1.016979e+02 5.000000e+00
4 1.320000e-03 5.084896e+01 5.000000e+00
8 1.340000e-03 2.542448e+01 5.000000e+00
16 1.340000e-03 1.271224e+01 5.000000e+00
32 1.460000e-03 6.356120e+00 5.000000e+00
64 1.300000e-03 3.178060e+00 5.000000e+00
128 1.400000e-03 1.589030e+00 5.000000e+00
256 1.400000e-03 7.945150e-01 5.000000e+00
512 1.420000e-03 3.972575e-01 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0006_1.tex <==
1 8.500000e-04 2.033958e+02 4.000000e+00
2 9.250000e-04 1.016979e+02 4.000000e+00
4 1.000000e-03 5.084896e+01 4.000000e+00
8 1.050000e-03 2.542448e+01 4.000000e+00
16 1.025000e-03 1.271224e+01 4.000000e+00
32 1.050000e-03 6.356120e+00 4.000000e+00
64 1.025000e-03 3.178060e+00 4.000000e+00
128 1.175000e-03 1.589030e+00 4.000000e+00
256 1.050000e-03 7.945150e-01 4.000000e+00
512 1.075000e-03 3.972575e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0006_2.tex <==
1 1.025000e-03 2.033958e+02 4.000000e+00
2 1.100000e-03 1.016979e+02 4.000000e+00
4 1.525000e-03 5.084896e+01 4.000000e+00
8 1.550000e-03 2.542448e+01 4.000000e+00
16 1.400000e-03 1.271224e+01 4.000000e+00
32 1.325000e-03 6.356120e+00 4.000000e+00
64 1.250000e-03 3.178060e+00 4.000000e+00
128 2.200000e-03 1.589030e+00 4.000000e+00
256 1.275000e-03 7.945150e-01 4.000000e+00
512 1.250000e-03 3.972575e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0007_0.tex <==
1 1.560000e-03 1.000854e+03 5.000000e+00
2 1.740000e-03 5.004271e+02 5.000000e+00
4 1.780000e-03 2.502135e+02 5.000000e+00
8 3.160000e-03 1.251068e+02 5.000000e+00
16 1.980000e-03 6.255339e+01 5.000000e+00
32 1.920000e-03 3.127669e+01 5.000000e+00
64 1.840000e-03 1.563835e+01 5.000000e+00
128 1.900000e-03 7.819173e+00 5.000000e+00
256 1.840000e-03 3.909587e+00 5.000000e+00
512 1.880000e-03 1.954793e+00 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0007_1.tex <==
1 1.625000e-03 1.000854e+03 4.000000e+00
2 1.475000e-03 5.004271e+02 4.000000e+00
4 1.425000e-03 2.502135e+02 4.000000e+00
8 1.775000e-03 1.251068e+02 4.000000e+00
16 1.500000e-03 6.255339e+01 4.000000e+00
32 1.425000e-03 3.127669e+01 4.000000e+00
64 1.450000e-03 1.563835e+01 4.000000e+00
128 1.425000e-03 7.819173e+00 4.000000e+00
256 1.425000e-03 3.909587e+00 4.000000e+00
512 1.425000e-03 1.954793e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0007_2.tex <==
1 1.975000e-03 1.000854e+03 4.000000e+00
2 1.800000e-03 5.004271e+02 4.000000e+00
4 1.800000e-03 2.502135e+02 4.000000e+00
8 1.850000e-03 1.251068e+02 4.000000e+00
16 1.900000e-03 6.255339e+01 4.000000e+00
32 1.800000e-03 3.127669e+01 4.000000e+00
64 1.775000e-03 1.563835e+01 4.000000e+00
128 2.425000e-03 7.819173e+00 4.000000e+00
256 1.675000e-03 3.909587e+00 4.000000e+00
512 1.625000e-03 1.954793e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0008_0.tex <==
1 5.040000e-03 6.605479e+03 5.000000e+00
2 4.140000e-03 3.302740e+03 5.000000e+00
4 3.200000e-03 1.651370e+03 5.000000e+00
8 4.800000e-03 8.256849e+02 5.000000e+00
16 2.660000e-03 4.128424e+02 5.000000e+00
32 2.580000e-03 2.064212e+02 5.000000e+00
64 2.460000e-03 1.032106e+02 5.000000e+00
128 2.840000e-03 5.160531e+01 5.000000e+00
256 2.980000e-03 2.580265e+01 5.000000e+00
512 2.720000e-03 1.290133e+01 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0008_1.tex <==
1 5.225000e-03 6.605479e+03 4.000000e+00
2 3.375000e-03 3.302740e+03 4.000000e+00
4 2.550000e-03 1.651370e+03 4.000000e+00
8 3.175000e-03 8.256849e+02 4.000000e+00
16 2.425000e-03 4.128424e+02 4.000000e+00
32 1.975000e-03 2.064212e+02 4.000000e+00
64 1.875000e-03 1.032106e+02 4.000000e+00
128 2.700000e-03 5.160531e+01 4.000000e+00
256 2.075000e-03 2.580265e+01 4.000000e+00
512 2.025000e-03 1.290133e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0008_2.tex <==
1 5.675000e-03 6.605479e+03 4.000000e+00
2 3.725000e-03 3.302740e+03 4.000000e+00
4 4.125000e-03 1.651370e+03 4.000000e+00
8 3.825000e-03 8.256849e+02 4.000000e+00
16 3.150000e-03 4.128424e+02 4.000000e+00
32 2.500000e-03 2.064212e+02 4.000000e+00
64 2.350000e-03 1.032106e+02 4.000000e+00
128 3.500000e-03 5.160531e+01 4.000000e+00
256 2.325000e-03 2.580265e+01 4.000000e+00
512 2.300000e-03 1.290133e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0009_0.tex <==
1 3.096000e-02 4.869377e+04 5.000000e+00
2 2.124000e-02 2.434689e+04 5.000000e+00
4 1.248000e-02 1.217344e+04 5.000000e+00
8 7.740000e-03 6.086721e+03 5.000000e+00
16 5.240000e-03 3.043361e+03 5.000000e+00
32 4.360000e-03 1.521680e+03 5.000000e+00
64 3.600000e-03 7.608402e+02 5.000000e+00
128 3.720000e-03 3.804201e+02 5.000000e+00
256 3.600000e-03 1.902100e+02 5.000000e+00
512 3.840000e-03 9.510502e+01 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0009_1.tex <==
1 2.640000e-02 4.869377e+04 4.000000e+00
2 1.527500e-02 2.434689e+04 4.000000e+00
4 8.925000e-03 1.217344e+04 4.000000e+00
8 6.375000e-03 6.086721e+03 4.000000e+00
16 3.825000e-03 3.043361e+03 4.000000e+00
32 3.050000e-03 1.521680e+03 4.000000e+00
64 2.525000e-03 7.608402e+02 4.000000e+00
128 2.525000e-03 3.804201e+02 4.000000e+00
256 2.775000e-03 1.902100e+02 4.000000e+00
512 2.650000e-03 9.510502e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0009_2.tex <==
1 2.682500e-02 4.869377e+04 4.000000e+00
2 1.572500e-02 2.434689e+04 4.000000e+00
4 9.150000e-03 1.217344e+04 4.000000e+00
8 6.075000e-03 6.086721e+03 4.000000e+00
16 4.725000e-03 3.043361e+03 4.000000e+00
32 3.650000e-03 1.521680e+03 4.000000e+00
64 3.000000e-03 7.608402e+02 4.000000e+00
128 5.725000e-03 3.804201e+02 4.000000e+00
256 2.750000e-03 1.902100e+02 4.000000e+00
512 2.600000e-03 9.510502e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0010_0.tex <==
1 2.302200e-01 3.747775e+05 5.000000e+00
2 1.383400e-01 1.873888e+05 5.000000e+00
4 7.796000e-02 9.369438e+04 5.000000e+00
8 4.506000e-02 4.684719e+04 5.000000e+00
16 2.726000e-02 2.342360e+04 5.000000e+00
32 1.540000e-02 1.171180e+04 5.000000e+00
64 9.420000e-03 5.855899e+03 5.000000e+00
128 6.560000e-03 2.927949e+03 5.000000e+00
256 5.380000e-03 1.463975e+03 5.000000e+00
512 5.100000e-03 7.319873e+02 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0010_1.tex <==
1 1.819000e-01 3.747775e+05 4.000000e+00
2 8.940000e-02 1.873888e+05 4.000000e+00
4 4.730000e-02 9.369438e+04 4.000000e+00
8 2.690000e-02 4.684719e+04 4.000000e+00
16 1.472500e-02 2.342360e+04 4.000000e+00
32 9.125000e-03 1.171180e+04 4.000000e+00
64 5.750000e-03 5.855899e+03 4.000000e+00
128 4.750000e-03 2.927949e+03 4.000000e+00
256 3.775000e-03 1.463975e+03 4.000000e+00
512 3.775000e-03 7.319873e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0010_2.tex <==
1 1.807250e-01 3.747775e+05 4.000000e+00
2 8.972500e-02 1.873888e+05 4.000000e+00
4 4.800000e-02 9.369438e+04 4.000000e+00
8 2.692500e-02 4.684719e+04 4.000000e+00
16 1.522500e-02 2.342360e+04 4.000000e+00
32 9.325000e-03 1.171180e+04 4.000000e+00
64 6.050000e-03 5.855899e+03 4.000000e+00
128 4.600000e-03 2.927949e+03 4.000000e+00
256 3.800000e-03 1.463975e+03 4.000000e+00
512 3.300000e-03 7.319873e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0011_0.tex <==
8 3.387000e-01 3.674826e+05 5.000000e+00
16 1.698200e-01 1.837413e+05 5.000000e+00
32 1.015200e-01 9.187066e+04 5.000000e+00
64 5.296000e-02 4.593533e+04 5.000000e+00
128 3.022000e-02 2.296766e+04 5.000000e+00
256 1.726000e-02 1.148383e+04 5.000000e+00
512 1.078000e-02 5.741916e+03 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0011_1.tex <==
8 1.986500e-01 3.674826e+05 4.000000e+00
16 8.767500e-02 1.837413e+05 4.000000e+00
32 4.955000e-02 9.187066e+04 4.000000e+00
64 2.485000e-02 4.593533e+04 4.000000e+00
128 1.572500e-02 2.296766e+04 4.000000e+00
256 9.925000e-03 1.148383e+04 4.000000e+00
512 7.250000e-03 5.741916e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0011_2.tex <==
8 1.971000e-01 3.674826e+05 4.000000e+00
16 8.782500e-02 1.837413e+05 4.000000e+00
32 4.947500e-02 9.187066e+04 4.000000e+00
64 2.537500e-02 4.593533e+04 4.000000e+00
128 1.657500e-02 2.296766e+04 4.000000e+00
256 9.625000e-03 1.148383e+04 4.000000e+00
512 6.575000e-03 5.741916e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0012_0.tex <==
64 3.908750e-01 3.638852e+05 4.000000e+00
128 2.170500e-01 1.819426e+05 4.000000e+00
256 1.142250e-01 9.097131e+04 4.000000e+00
512 6.010000e-02 4.548565e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0012_1.tex <==
64 1.759250e-01 3.638852e+05 4.000000e+00
128 9.477500e-02 1.819426e+05 4.000000e+00
256 4.977500e-02 9.097131e+04 4.000000e+00
512 2.830000e-02 4.548565e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0012_2.tex <==
64 1.735250e-01 3.638852e+05 4.000000e+00
128 9.247500e-02 1.819426e+05 4.000000e+00
256 4.907500e-02 9.097131e+04 4.000000e+00
512 2.880000e-02 4.548565e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-1/data_0013_0.tex <==
512 4.778750e-01 3.620633e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0005_0.tex <==
1 1.425000e-03 1.928688e+03 4.000000e+00
2 1.650000e-03 9.643438e+02 4.000000e+00
4 1.575000e-03 4.821719e+02 4.000000e+00
8 1.500000e-03 2.410859e+02 4.000000e+00
16 1.550000e-03 1.205430e+02 4.000000e+00
32 1.550000e-03 6.027148e+01 4.000000e+00
64 1.600000e-03 3.013574e+01 4.000000e+00
128 1.600000e-03 1.506787e+01 4.000000e+00
256 1.600000e-03 7.533936e+00 4.000000e+00
512 1.750000e-03 3.766968e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0005_1.tex <==
1 1.475000e-03 1.928688e+03 4.000000e+00
2 1.550000e-03 9.643438e+02 4.000000e+00
4 1.550000e-03 4.821719e+02 4.000000e+00
8 1.575000e-03 2.410859e+02 4.000000e+00
16 1.575000e-03 1.205430e+02 4.000000e+00
32 1.575000e-03 6.027148e+01 4.000000e+00
64 1.600000e-03 3.013574e+01 4.000000e+00
128 1.650000e-03 1.506787e+01 4.000000e+00
256 1.575000e-03 7.533936e+00 4.000000e+00
512 1.600000e-03 3.766968e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0005_2.tex <==
1 1.525000e-03 1.928688e+03 4.000000e+00
2 1.575000e-03 9.643438e+02 4.000000e+00
4 1.750000e-03 4.821719e+02 4.000000e+00
8 1.700000e-03 2.410859e+02 4.000000e+00
16 1.725000e-03 1.205430e+02 4.000000e+00
32 1.800000e-03 6.027148e+01 4.000000e+00
64 1.800000e-03 3.013574e+01 4.000000e+00
128 1.750000e-03 1.506787e+01 4.000000e+00
256 1.800000e-03 7.533936e+00 4.000000e+00
512 1.725000e-03 3.766968e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0006_0.tex <==
1 2.975000e-03 1.062652e+04 4.000000e+00
2 2.525000e-03 5.313260e+03 4.000000e+00
4 2.250000e-03 2.656630e+03 4.000000e+00
8 2.125000e-03 1.328315e+03 4.000000e+00
16 2.175000e-03 6.641576e+02 4.000000e+00
32 2.175000e-03 3.320788e+02 4.000000e+00
64 2.250000e-03 1.660394e+02 4.000000e+00
128 2.175000e-03 8.301969e+01 4.000000e+00
256 2.175000e-03 4.150985e+01 4.000000e+00
512 2.325000e-03 2.075492e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0006_1.tex <==
1 2.950000e-03 1.062652e+04 4.000000e+00
2 2.475000e-03 5.313260e+03 4.000000e+00
4 2.275000e-03 2.656630e+03 4.000000e+00
8 2.200000e-03 1.328315e+03 4.000000e+00
16 2.175000e-03 6.641576e+02 4.000000e+00
32 2.250000e-03 3.320788e+02 4.000000e+00
64 2.100000e-03 1.660394e+02 4.000000e+00
128 2.200000e-03 8.301969e+01 4.000000e+00
256 2.050000e-03 4.150985e+01 4.000000e+00
512 2.100000e-03 2.075492e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0006_2.tex <==
1 3.075000e-03 1.062652e+04 4.000000e+00
2 2.650000e-03 5.313260e+03 4.000000e+00
4 2.375000e-03 2.656630e+03 4.000000e+00
8 2.425000e-03 1.328315e+03 4.000000e+00
16 2.500000e-03 6.641576e+02 4.000000e+00
32 2.550000e-03 3.320788e+02 4.000000e+00
64 2.375000e-03 1.660394e+02 4.000000e+00
128 2.350000e-03 8.301969e+01 4.000000e+00
256 2.325000e-03 4.150985e+01 4.000000e+00
512 2.175000e-03 2.075492e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0007_0.tex <==
1 1.095000e-02 5.512835e+04 4.000000e+00
2 8.275000e-03 2.756418e+04 4.000000e+00
4 5.750000e-03 1.378209e+04 4.000000e+00
8 4.075000e-03 6.891044e+03 4.000000e+00
16 3.375000e-03 3.445522e+03 4.000000e+00
32 3.225000e-03 1.722761e+03 4.000000e+00
64 3.650000e-03 8.613805e+02 4.000000e+00
128 3.200000e-03 4.306903e+02 4.000000e+00
256 3.100000e-03 2.153451e+02 4.000000e+00
512 3.025000e-03 1.076726e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0007_1.tex <==
1 1.002500e-02 5.512835e+04 4.000000e+00
2 6.250000e-03 2.756418e+04 4.000000e+00
4 4.525000e-03 1.378209e+04 4.000000e+00
8 3.725000e-03 6.891044e+03 4.000000e+00
16 3.350000e-03 3.445522e+03 4.000000e+00
32 3.050000e-03 1.722761e+03 4.000000e+00
64 3.325000e-03 8.613805e+02 4.000000e+00
128 3.250000e-03 4.306903e+02 4.000000e+00
256 3.125000e-03 2.153451e+02 4.000000e+00
512 3.000000e-03 1.076726e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0007_2.tex <==
1 1.142500e-02 5.512835e+04 4.000000e+00
2 7.500000e-03 2.756418e+04 4.000000e+00
4 5.100000e-03 1.378209e+04 4.000000e+00
8 4.100000e-03 6.891044e+03 4.000000e+00
16 3.725000e-03 3.445522e+03 4.000000e+00
32 3.350000e-03 1.722761e+03 4.000000e+00
64 3.325000e-03 8.613805e+02 4.000000e+00
128 3.400000e-03 4.306903e+02 4.000000e+00
256 2.975000e-03 2.153451e+02 4.000000e+00
512 3.025000e-03 1.076726e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0008_0.tex <==
1 8.602500e-02 3.870539e+05 4.000000e+00
2 5.197500e-02 1.935269e+05 4.000000e+00
4 2.672500e-02 9.676346e+04 4.000000e+00
8 1.717500e-02 4.838173e+04 4.000000e+00
16 1.010000e-02 2.419087e+04 4.000000e+00
32 6.525000e-03 1.209543e+04 4.000000e+00
64 6.950000e-03 6.047716e+03 4.000000e+00
128 4.425000e-03 3.023858e+03 4.000000e+00
256 4.750000e-03 1.511929e+03 4.000000e+00
512 5.000000e-03 7.559646e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0008_1.tex <==
1 7.085000e-02 3.870539e+05 4.000000e+00
2 3.545000e-02 1.935269e+05 4.000000e+00
4 1.715000e-02 9.676346e+04 4.000000e+00
8 1.170000e-02 4.838173e+04 4.000000e+00
16 7.000000e-03 2.419087e+04 4.000000e+00
32 5.400000e-03 1.209543e+04 4.000000e+00
64 4.350000e-03 6.047716e+03 4.000000e+00
128 4.350000e-03 3.023858e+03 4.000000e+00
256 4.025000e-03 1.511929e+03 4.000000e+00
512 4.075000e-03 7.559646e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0008_2.tex <==
1 6.962500e-02 3.870539e+05 4.000000e+00
2 3.505000e-02 1.935269e+05 4.000000e+00
4 1.752500e-02 9.676346e+04 4.000000e+00
8 1.215000e-02 4.838173e+04 4.000000e+00
16 7.750000e-03 2.419087e+04 4.000000e+00
32 5.800000e-03 1.209543e+04 4.000000e+00
64 5.300000e-03 6.047716e+03 4.000000e+00
128 5.050000e-03 3.023858e+03 4.000000e+00
256 4.775000e-03 1.511929e+03 4.000000e+00
512 4.425000e-03 7.559646e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0009_0.tex <==
1 6.800500e-01 2.974569e+06 4.000000e+00
2 4.074750e-01 1.487285e+06 4.000000e+00
4 2.102750e-01 7.436423e+05 4.000000e+00
8 1.436250e-01 3.718211e+05 4.000000e+00
16 7.387500e-02 1.859106e+05 4.000000e+00
32 4.157500e-02 9.295528e+04 4.000000e+00
64 2.080000e-02 4.647764e+04 4.000000e+00
128 1.190000e-02 2.323882e+04 4.000000e+00
256 7.725000e-03 1.161941e+04 4.000000e+00
512 6.900000e-03 5.809705e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0009_1.tex <==
1 5.208000e-01 2.974569e+06 4.000000e+00
2 2.627250e-01 1.487285e+06 4.000000e+00
4 1.297250e-01 7.436423e+05 4.000000e+00
8 1.014500e-01 3.718211e+05 4.000000e+00
16 4.692500e-02 1.859106e+05 4.000000e+00
32 2.277500e-02 9.295528e+04 4.000000e+00
64 1.082500e-02 4.647764e+04 4.000000e+00
128 7.900000e-03 2.323882e+04 4.000000e+00
256 5.825000e-03 1.161941e+04 4.000000e+00
512 5.325000e-03 5.809705e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0009_2.tex <==
1 5.002500e-01 2.974569e+06 4.000000e+00
2 2.544000e-01 1.487285e+06 4.000000e+00
4 1.262500e-01 7.436423e+05 4.000000e+00
8 9.760000e-02 3.718211e+05 4.000000e+00
16 4.557500e-02 1.859106e+05 4.000000e+00
32 2.200000e-02 9.295528e+04 4.000000e+00
64 1.215000e-02 4.647764e+04 4.000000e+00
128 8.075000e-03 2.323882e+04 4.000000e+00
256 6.250000e-03 1.161941e+04 4.000000e+00
512 5.625000e-03 5.809705e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0010_0.tex <==
8 1.169650e+00 2.927377e+06 4.000000e+00
16 6.315000e-01 1.463688e+06 4.000000e+00
32 3.832000e-01 7.318442e+05 4.000000e+00
64 1.628500e-01 3.659221e+05 4.000000e+00
128 1.023250e-01 1.829610e+05 4.000000e+00
256 4.730000e-02 9.148052e+04 4.000000e+00
512 2.592500e-02 4.574026e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0010_1.tex <==
8 8.133500e-01 2.927377e+06 4.000000e+00
16 4.067000e-01 1.463688e+06 4.000000e+00
32 2.053500e-01 7.318442e+05 4.000000e+00
64 8.242500e-02 3.659221e+05 4.000000e+00
128 4.967500e-02 1.829610e+05 4.000000e+00
256 2.392500e-02 9.148052e+04 4.000000e+00
512 1.342500e-02 4.574026e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0010_2.tex <==
8 7.788250e-01 2.927377e+06 4.000000e+00
16 3.892500e-01 1.463688e+06 4.000000e+00
32 1.949000e-01 7.318442e+05 4.000000e+00
64 7.827500e-02 3.659221e+05 4.000000e+00
128 4.640000e-02 1.829610e+05 4.000000e+00
256 2.195000e-02 9.148052e+04 4.000000e+00
512 1.275000e-02 4.574026e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0011_0.tex <==
64 1.278725e+00 2.904492e+06 4.000000e+00
128 8.950750e-01 1.452246e+06 4.000000e+00
256 4.575000e-01 7.261231e+05 4.000000e+00
512 2.514500e-01 3.630615e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0011_1.tex <==
64 6.311250e-01 2.904492e+06 4.000000e+00
128 4.133000e-01 1.452246e+06 4.000000e+00
256 2.072750e-01 7.261231e+05 4.000000e+00
512 1.078500e-01 3.630615e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0011_2.tex <==
64 5.974750e-01 2.904492e+06 4.000000e+00
128 3.907000e-01 1.452246e+06 4.000000e+00
256 1.919750e-01 7.261231e+05 4.000000e+00
512 9.762500e-02 3.630615e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0012_0.tex <==
512 2.120740e+00 2.893403e+06 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0012_1.tex <==
512 8.356200e-01 2.893403e+06 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-annulus-4/data_0012_2.tex <==
512 7.905400e-01 2.893403e+06 5.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0003_0.tex <==
1 2.750000e-04 4.645833e+00 4.000000e+00
2 3.000000e-04 2.322917e+00 4.000000e+00
4 3.000000e-04 1.161458e+00 4.000000e+00
8 3.250000e-04 5.807292e-01 4.000000e+00
16 3.250000e-04 2.903646e-01 4.000000e+00
32 3.750000e-04 1.451823e-01 4.000000e+00
64 3.750000e-04 7.259115e-02 4.000000e+00
128 4.000000e-04 3.629557e-02 4.000000e+00
256 4.250000e-04 1.814779e-02 4.000000e+00
512 4.750000e-04 9.073893e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0003_1.tex <==
1 2.250000e-04 4.645833e+00 4.000000e+00
2 2.250000e-04 2.322917e+00 4.000000e+00
4 2.500000e-04 1.161458e+00 4.000000e+00
8 2.750000e-04 5.807292e-01 4.000000e+00
16 2.500000e-04 2.903646e-01 4.000000e+00
32 2.750000e-04 1.451823e-01 4.000000e+00
64 2.750000e-04 7.259115e-02 4.000000e+00
128 3.000000e-04 3.629557e-02 4.000000e+00
256 3.500000e-04 1.814779e-02 4.000000e+00
512 3.250000e-04 9.073893e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0003_2.tex <==
1 4.000000e-04 4.645833e+00 4.000000e+00
2 3.750000e-04 2.322917e+00 4.000000e+00
4 4.000000e-04 1.161458e+00 4.000000e+00
8 4.000000e-04 5.807292e-01 4.000000e+00
16 4.250000e-04 2.903646e-01 4.000000e+00
32 5.250000e-04 1.451823e-01 4.000000e+00
64 4.500000e-04 7.259115e-02 4.000000e+00
128 4.250000e-04 3.629557e-02 4.000000e+00
256 4.750000e-04 1.814779e-02 4.000000e+00
512 5.000000e-04 9.073893e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0004_0.tex <==
1 6.500000e-04 2.100000e+01 4.000000e+00
2 6.500000e-04 1.050000e+01 4.000000e+00
4 6.500000e-04 5.250000e+00 4.000000e+00
8 7.000000e-04 2.625000e+00 4.000000e+00
16 1.000000e-03 1.312500e+00 4.000000e+00
32 7.250000e-04 6.562500e-01 4.000000e+00
64 7.500000e-04 3.281250e-01 4.000000e+00
128 7.750000e-04 1.640625e-01 4.000000e+00
256 7.500000e-04 8.203125e-02 4.000000e+00
512 8.500000e-04 4.101562e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0004_1.tex <==
1 4.000000e-04 2.100000e+01 4.000000e+00
2 4.000000e-04 1.050000e+01 4.000000e+00
4 4.000000e-04 5.250000e+00 4.000000e+00
8 5.250000e-04 2.625000e+00 4.000000e+00
16 4.750000e-04 1.312500e+00 4.000000e+00
32 4.750000e-04 6.562500e-01 4.000000e+00
64 4.500000e-04 3.281250e-01 4.000000e+00
128 4.750000e-04 1.640625e-01 4.000000e+00
256 4.750000e-04 8.203125e-02 4.000000e+00
512 5.000000e-04 4.101562e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0004_2.tex <==
1 6.500000e-04 2.100000e+01 4.000000e+00
2 6.500000e-04 1.050000e+01 4.000000e+00
4 5.750000e-04 5.250000e+00 4.000000e+00
8 1.025000e-03 2.625000e+00 4.000000e+00
16 1.000000e-03 1.312500e+00 4.000000e+00
32 6.500000e-04 6.562500e-01 4.000000e+00
64 6.750000e-04 3.281250e-01 4.000000e+00
128 7.000000e-04 1.640625e-01 4.000000e+00
256 6.750000e-04 8.203125e-02 4.000000e+00
512 7.000000e-04 4.101562e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0005_0.tex <==
1 8.750000e-04 1.188125e+02 4.000000e+00
2 1.000000e-03 5.940625e+01 4.000000e+00
4 1.025000e-03 2.970312e+01 4.000000e+00
8 1.325000e-03 1.485156e+01 4.000000e+00
16 1.325000e-03 7.425781e+00 4.000000e+00
32 1.025000e-03 3.712891e+00 4.000000e+00
64 1.200000e-03 1.856445e+00 4.000000e+00
128 1.075000e-03 9.282227e-01 4.000000e+00
256 1.150000e-03 4.641113e-01 4.000000e+00
512 1.100000e-03 2.320557e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0005_1.tex <==
1 6.250000e-04 1.188125e+02 4.000000e+00
2 6.250000e-04 5.940625e+01 4.000000e+00
4 6.250000e-04 2.970312e+01 4.000000e+00
8 1.125000e-03 1.485156e+01 4.000000e+00
16 7.000000e-04 7.425781e+00 4.000000e+00
32 6.500000e-04 3.712891e+00 4.000000e+00
64 6.500000e-04 1.856445e+00 4.000000e+00
128 6.750000e-04 9.282227e-01 4.000000e+00
256 7.000000e-04 4.641113e-01 4.000000e+00
512 7.250000e-04 2.320557e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0005_2.tex <==
1 8.000000e-04 1.188125e+02 4.000000e+00
2 8.750000e-04 5.940625e+01 4.000000e+00
4 9.000000e-04 2.970312e+01 4.000000e+00
8 1.200000e-03 1.485156e+01 4.000000e+00
16 1.025000e-03 7.425781e+00 4.000000e+00
32 9.500000e-04 3.712891e+00 4.000000e+00
64 9.250000e-04 1.856445e+00 4.000000e+00
128 1.000000e-03 9.282227e-01 4.000000e+00
256 9.250000e-04 4.641113e-01 4.000000e+00
512 9.500000e-04 2.320557e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0006_0.tex <==
1 1.550000e-03 8.000417e+02 4.000000e+00
2 1.400000e-03 4.000208e+02 4.000000e+00
4 1.350000e-03 2.000104e+02 4.000000e+00
8 1.825000e-03 1.000052e+02 4.000000e+00
16 1.425000e-03 5.000260e+01 4.000000e+00
32 3.325000e-03 2.500130e+01 4.000000e+00
64 1.525000e-03 1.250065e+01 4.000000e+00
128 1.475000e-03 6.250326e+00 4.000000e+00
256 1.525000e-03 3.125163e+00 4.000000e+00
512 1.575000e-03 1.562581e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0006_1.tex <==
1 1.125000e-03 8.000417e+02 4.000000e+00
2 1.025000e-03 4.000208e+02 4.000000e+00
4 9.750000e-04 2.000104e+02 4.000000e+00
8 1.550000e-03 1.000052e+02 4.000000e+00
16 1.025000e-03 5.000260e+01 4.000000e+00
32 1.100000e-03 2.500130e+01 4.000000e+00
64 1.050000e-03 1.250065e+01 4.000000e+00
128 1.000000e-03 6.250326e+00 4.000000e+00
256 1.150000e-03 3.125163e+00 4.000000e+00
512 1.175000e-03 1.562581e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0006_2.tex <==
1 1.350000e-03 8.000417e+02 4.000000e+00
2 1.250000e-03 4.000208e+02 4.000000e+00
4 1.275000e-03 2.000104e+02 4.000000e+00
8 3.050000e-03 1.000052e+02 4.000000e+00
16 2.000000e-03 5.000260e+01 4.000000e+00
32 3.200000e-03 2.500130e+01 4.000000e+00
64 1.375000e-03 1.250065e+01 4.000000e+00
128 1.325000e-03 6.250326e+00 4.000000e+00
256 1.325000e-03 3.125163e+00 4.000000e+00
512 1.325000e-03 1.562581e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0007_0.tex <==
1 5.075000e-03 5.898104e+03 4.000000e+00
2 3.450000e-03 2.949052e+03 4.000000e+00
4 2.575000e-03 1.474526e+03 4.000000e+00
8 3.375000e-03 7.372630e+02 4.000000e+00
16 3.400000e-03 3.686315e+02 4.000000e+00
32 2.025000e-03 1.843158e+02 4.000000e+00
64 1.925000e-03 9.215788e+01 4.000000e+00
128 2.825000e-03 4.607894e+01 4.000000e+00
256 2.475000e-03 2.303947e+01 4.000000e+00
512 2.375000e-03 1.151973e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0007_1.tex <==
1 3.700000e-03 5.898104e+03 3.000000e+00
2 2.466667e-03 2.949052e+03 3.000000e+00
4 1.833333e-03 1.474526e+03 3.000000e+00
8 1.600000e-03 7.372630e+02 3.000000e+00
16 1.500000e-03 3.686315e+02 3.000000e+00
32 1.966667e-03 1.843158e+02 3.000000e+00
64 1.500000e-03 9.215788e+01 3.000000e+00
128 2.100000e-03 4.607894e+01 3.000000e+00
256 2.233333e-03 2.303947e+01 3.000000e+00
512 1.933333e-03 1.151973e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0007_2.tex <==
1 4.500000e-03 5.898104e+03 3.000000e+00
2 2.966667e-03 2.949052e+03 3.000000e+00
4 2.300000e-03 1.474526e+03 3.000000e+00
8 2.033333e-03 7.372630e+02 3.000000e+00
16 1.766667e-03 3.686315e+02 3.000000e+00
32 1.866667e-03 1.843158e+02 3.000000e+00
64 1.766667e-03 9.215788e+01 3.000000e+00
128 1.866667e-03 4.607894e+01 3.000000e+00
256 1.966667e-03 2.303947e+01 3.000000e+00
512 1.900000e-03 1.151973e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0008_0.tex <==
1 2.742500e-02 4.537383e+04 4.000000e+00
2 1.632500e-02 2.268692e+04 4.000000e+00
4 9.500000e-03 1.134346e+04 4.000000e+00
8 6.475000e-03 5.671729e+03 4.000000e+00
16 4.275000e-03 2.835865e+03 4.000000e+00
32 3.475000e-03 1.417932e+03 4.000000e+00
64 3.000000e-03 7.089661e+02 4.000000e+00
128 2.750000e-03 3.544831e+02 4.000000e+00
256 2.600000e-03 1.772415e+02 4.000000e+00
512 2.750000e-03 8.862077e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0008_1.tex <==
1 2.120000e-02 4.537383e+04 3.000000e+00
2 1.176667e-02 2.268692e+04 3.000000e+00
4 6.800000e-03 1.134346e+04 3.000000e+00
8 4.300000e-03 5.671729e+03 3.000000e+00
16 4.500000e-03 2.835865e+03 3.000000e+00
32 2.933333e-03 1.417932e+03 3.000000e+00
64 2.466667e-03 7.089661e+02 3.000000e+00
128 2.366667e-03 3.544831e+02 3.000000e+00
256 2.733333e-03 1.772415e+02 3.000000e+00
512 2.600000e-03 8.862077e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0008_2.tex <==
1 2.543333e-02 4.537383e+04 3.000000e+00
2 1.410000e-02 2.268692e+04 3.000000e+00
4 8.233333e-03 1.134346e+04 3.000000e+00
8 5.833333e-03 5.671729e+03 3.000000e+00
16 3.766667e-03 2.835865e+03 3.000000e+00
32 3.033333e-03 1.417932e+03 3.000000e+00
64 2.800000e-03 7.089661e+02 3.000000e+00
128 2.400000e-03 3.544831e+02 3.000000e+00
256 2.366667e-03 1.772415e+02 3.000000e+00
512 2.433333e-03 8.862077e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0009_0.tex <==
1 1.744250e-01 3.561329e+05 4.000000e+00
2 1.026000e-01 1.780664e+05 4.000000e+00
4 5.487500e-02 8.903322e+04 4.000000e+00
8 3.097500e-02 4.451661e+04 4.000000e+00
16 1.722500e-02 2.225831e+04 4.000000e+00
32 1.057500e-02 1.112915e+04 4.000000e+00
64 6.750000e-03 5.564576e+03 4.000000e+00
128 5.300000e-03 2.782288e+03 4.000000e+00
256 4.100000e-03 1.391144e+03 4.000000e+00
512 5.550000e-03 6.955721e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0009_1.tex <==
1 1.487667e-01 3.561329e+05 3.000000e+00
2 7.840000e-02 1.780664e+05 3.000000e+00
4 4.096667e-02 8.903322e+04 3.000000e+00
8 2.153333e-02 4.451661e+04 3.000000e+00
16 1.226667e-02 2.225831e+04 3.000000e+00
32 7.766667e-03 1.112915e+04 3.000000e+00
64 4.833333e-03 5.564576e+03 3.000000e+00
128 4.166667e-03 2.782288e+03 3.000000e+00
256 3.300000e-03 1.391144e+03 3.000000e+00
512 3.500000e-03 6.955721e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0009_2.tex <==
1 1.601667e-01 3.561329e+05 3.000000e+00
2 9.240000e-02 1.780664e+05 3.000000e+00
4 4.783333e-02 8.903322e+04 3.000000e+00
8 2.606667e-02 4.451661e+04 3.000000e+00
16 1.550000e-02 2.225831e+04 3.000000e+00
32 9.866667e-03 1.112915e+04 3.000000e+00
64 6.333333e-03 5.564576e+03 3.000000e+00
128 5.000000e-03 2.782288e+03 3.000000e+00
256 3.600000e-03 1.391144e+03 3.000000e+00
512 3.300000e-03 6.955721e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0010_0.tex <==
8 2.135750e-01 3.527983e+05 4.000000e+00
16 1.084000e-01 1.763992e+05 4.000000e+00
32 5.722500e-02 8.819958e+04 4.000000e+00
64 3.262500e-02 4.409979e+04 4.000000e+00
128 1.920000e-02 2.204990e+04 4.000000e+00
256 1.197500e-02 1.102495e+04 4.000000e+00
512 1.007500e-02 5.512474e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0010_1.tex <==
8 1.643500e-01 3.527983e+05 2.000000e+00
16 7.985000e-02 1.763992e+05 2.000000e+00
32 4.125000e-02 8.819958e+04 2.000000e+00
64 2.265000e-02 4.409979e+04 2.000000e+00
128 1.400000e-02 2.204990e+04 2.000000e+00
256 1.005000e-02 1.102495e+04 2.000000e+00
512 7.100000e-03 5.512474e+03 2.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0010_2.tex <==
8 1.856000e-01 3.527983e+05 2.000000e+00
16 9.430000e-02 1.763992e+05 2.000000e+00
32 4.955000e-02 8.819958e+04 2.000000e+00
64 2.800000e-02 4.409979e+04 2.000000e+00
128 1.745000e-02 2.204990e+04 2.000000e+00
256 1.180000e-02 1.102495e+04 2.000000e+00
512 8.800000e-03 5.512474e+03 2.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0011_0.tex <==
64 2.302500e-01 3.511542e+05 4.000000e+00
128 1.307250e-01 1.755771e+05 4.000000e+00
256 6.602500e-02 8.778855e+04 4.000000e+00
512 3.835000e-02 4.389428e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0011_1.tex <==
128 9.575000e-02 1.755771e+05 2.000000e+00
256 4.790000e-02 8.778855e+04 2.000000e+00
512 2.960000e-02 4.389428e+04 2.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-1/data_0011_2.tex <==
128 1.055000e-01 1.755771e+05 2.000000e+00
256 5.425000e-02 8.778855e+04 2.000000e+00
512 3.420000e-02 4.389428e+04 2.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0003_0.tex <==
1 6.250000e-04 1.936458e+02 4.000000e+00
2 6.250000e-04 9.682292e+01 4.000000e+00
4 6.750000e-04 4.841146e+01 4.000000e+00
8 6.500000e-04 2.420573e+01 4.000000e+00
16 7.000000e-04 1.210286e+01 4.000000e+00
32 7.500000e-04 6.051432e+00 4.000000e+00
64 7.250000e-04 3.025716e+00 4.000000e+00
128 7.500000e-04 1.512858e+00 4.000000e+00
256 7.500000e-04 7.564290e-01 4.000000e+00
512 8.000000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0003_1.tex <==
1 6.000000e-04 1.936458e+02 4.000000e+00
2 6.000000e-04 9.682292e+01 4.000000e+00
4 6.500000e-04 4.841146e+01 4.000000e+00
8 6.250000e-04 2.420573e+01 4.000000e+00
16 7.000000e-04 1.210286e+01 4.000000e+00
32 7.750000e-04 6.051432e+00 4.000000e+00
64 6.750000e-04 3.025716e+00 4.000000e+00
128 7.000000e-04 1.512858e+00 4.000000e+00
256 6.750000e-04 7.564290e-01 4.000000e+00
512 7.000000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0003_2.tex <==
1 7.000000e-04 1.936458e+02 4.000000e+00
2 7.000000e-04 9.682292e+01 4.000000e+00
4 7.250000e-04 4.841146e+01 4.000000e+00
8 1.175000e-03 2.420573e+01 4.000000e+00
16 8.000000e-04 1.210286e+01 4.000000e+00
32 1.025000e-03 6.051432e+00 4.000000e+00
64 8.250000e-04 3.025716e+00 4.000000e+00
128 7.500000e-04 1.512858e+00 4.000000e+00
256 8.500000e-04 7.564290e-01 4.000000e+00
512 8.500000e-04 3.782145e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0004_0.tex <==
1 1.100000e-03 1.053188e+03 4.000000e+00
2 1.075000e-03 5.265938e+02 4.000000e+00
4 1.050000e-03 2.632969e+02 4.000000e+00
8 1.550000e-03 1.316484e+02 4.000000e+00
16 1.100000e-03 6.582422e+01 4.000000e+00
32 1.300000e-03 3.291211e+01 4.000000e+00
64 1.125000e-03 1.645605e+01 4.000000e+00
128 1.200000e-03 8.228027e+00 4.000000e+00
256 1.200000e-03 4.114014e+00 4.000000e+00
512 1.225000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0004_1.tex <==
1 1.025000e-03 1.053188e+03 4.000000e+00
2 9.750000e-04 5.265938e+02 4.000000e+00
4 9.750000e-04 2.632969e+02 4.000000e+00
8 1.150000e-03 1.316484e+02 4.000000e+00
16 1.250000e-03 6.582422e+01 4.000000e+00
32 1.175000e-03 3.291211e+01 4.000000e+00
64 1.000000e-03 1.645605e+01 4.000000e+00
128 1.050000e-03 8.228027e+00 4.000000e+00
256 1.075000e-03 4.114014e+00 4.000000e+00
512 1.050000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0004_2.tex <==
1 1.175000e-03 1.053188e+03 4.000000e+00
2 1.150000e-03 5.265938e+02 4.000000e+00
4 1.125000e-03 2.632969e+02 4.000000e+00
8 1.500000e-03 1.316484e+02 4.000000e+00
16 2.450000e-03 6.582422e+01 4.000000e+00
32 1.200000e-03 3.291211e+01 4.000000e+00
64 1.225000e-03 1.645605e+01 4.000000e+00
128 1.250000e-03 8.228027e+00 4.000000e+00
256 1.225000e-03 4.114014e+00 4.000000e+00
512 1.200000e-03 2.057007e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0005_0.tex <==
1 2.175000e-03 6.692562e+03 4.000000e+00
2 1.825000e-03 3.346281e+03 4.000000e+00
4 1.700000e-03 1.673141e+03 4.000000e+00
8 2.425000e-03 8.365703e+02 4.000000e+00
16 1.700000e-03 4.182852e+02 4.000000e+00
32 1.875000e-03 2.091426e+02 4.000000e+00
64 1.675000e-03 1.045713e+02 4.000000e+00
128 1.775000e-03 5.228564e+01 4.000000e+00
256 1.825000e-03 2.614282e+01 4.000000e+00
512 1.725000e-03 1.307141e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0005_1.tex <==
1 2.000000e-03 6.692562e+03 3.000000e+00
2 1.733333e-03 3.346281e+03 3.000000e+00
4 1.666667e-03 1.673141e+03 3.000000e+00
8 1.800000e-03 8.365703e+02 3.000000e+00
16 1.566667e-03 4.182852e+02 3.000000e+00
32 1.633333e-03 2.091426e+02 3.000000e+00
64 1.533333e-03 1.045713e+02 3.000000e+00
128 1.600000e-03 5.228564e+01 3.000000e+00
256 1.533333e-03 2.614282e+01 3.000000e+00
512 1.533333e-03 1.307141e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0005_2.tex <==
1 2.033333e-03 6.692562e+03 3.000000e+00
2 1.966667e-03 3.346281e+03 3.000000e+00
4 1.800000e-03 1.673141e+03 3.000000e+00
8 2.000000e-03 8.365703e+02 3.000000e+00
16 3.866667e-03 4.182852e+02 3.000000e+00
32 2.066667e-03 2.091426e+02 3.000000e+00
64 1.700000e-03 1.045713e+02 3.000000e+00
128 1.833333e-03 5.228564e+01 3.000000e+00
256 1.733333e-03 2.614282e+01 3.000000e+00
512 1.566667e-03 1.307141e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0006_0.tex <==
1 1.002500e-02 4.802960e+04 4.000000e+00
2 6.525000e-03 2.401480e+04 4.000000e+00
4 3.775000e-03 1.200740e+04 4.000000e+00
8 3.500000e-03 6.003701e+03 4.000000e+00
16 4.325000e-03 3.001850e+03 4.000000e+00
32 2.625000e-03 1.500925e+03 4.000000e+00
64 2.925000e-03 7.504626e+02 4.000000e+00
128 2.650000e-03 3.752313e+02 4.000000e+00
256 2.650000e-03 1.876156e+02 4.000000e+00
512 3.300000e-03 9.380782e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0006_1.tex <==
1 7.733333e-03 4.802960e+04 3.000000e+00
2 4.366667e-03 2.401480e+04 3.000000e+00
4 3.433333e-03 1.200740e+04 3.000000e+00
8 2.900000e-03 6.003701e+03 3.000000e+00
16 2.300000e-03 3.001850e+03 3.000000e+00
32 2.366667e-03 1.500925e+03 3.000000e+00
64 2.600000e-03 7.504626e+02 3.000000e+00
128 2.233333e-03 3.752313e+02 3.000000e+00
256 2.500000e-03 1.876156e+02 3.000000e+00
512 2.200000e-03 9.380782e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0006_2.tex <==
1 7.866667e-03 4.802960e+04 3.000000e+00
2 4.866667e-03 2.401480e+04 3.000000e+00
4 3.500000e-03 1.200740e+04 3.000000e+00
8 4.066667e-03 6.003701e+03 3.000000e+00
16 2.800000e-03 3.001850e+03 3.000000e+00
32 3.033333e-03 1.500925e+03 3.000000e+00
64 2.766667e-03 7.504626e+02 3.000000e+00
128 2.433333e-03 3.752313e+02 3.000000e+00
256 2.366667e-03 1.876156e+02 3.000000e+00
512 2.233333e-03 9.380782e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0007_0.tex <==
1 8.170000e-02 3.656660e+05 4.000000e+00
2 3.950000e-02 1.828330e+05 4.000000e+00
4 2.490000e-02 9.141649e+04 4.000000e+00
8 1.247500e-02 4.570825e+04 4.000000e+00
16 7.225000e-03 2.285412e+04 4.000000e+00
32 7.725000e-03 1.142706e+04 4.000000e+00
64 3.900000e-03 5.713531e+03 4.000000e+00
128 4.200000e-03 2.856765e+03 4.000000e+00
256 4.250000e-03 1.428383e+03 4.000000e+00
512 4.525000e-03 7.141914e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0007_1.tex <==
1 6.390000e-02 3.656660e+05 3.000000e+00
2 3.153333e-02 1.828330e+05 3.000000e+00
4 2.000000e-02 9.141649e+04 3.000000e+00
8 1.016667e-02 4.570825e+04 3.000000e+00
16 5.266667e-03 2.285412e+04 3.000000e+00
32 4.633333e-03 1.142706e+04 3.000000e+00
64 3.833333e-03 5.713531e+03 3.000000e+00
128 3.100000e-03 2.856765e+03 3.000000e+00
256 3.333333e-03 1.428383e+03 3.000000e+00
512 3.666667e-03 7.141914e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0007_2.tex <==
1 6.176667e-02 3.656660e+05 3.000000e+00
2 3.003333e-02 1.828330e+05 3.000000e+00
4 1.926667e-02 9.141649e+04 3.000000e+00
8 1.020000e-02 4.570825e+04 3.000000e+00
16 5.600000e-03 2.285412e+04 3.000000e+00
32 5.033333e-03 1.142706e+04 3.000000e+00
64 3.966667e-03 5.713531e+03 3.000000e+00
128 4.166667e-03 2.856765e+03 3.000000e+00
256 4.100000e-03 1.428383e+03 3.000000e+00
512 4.666667e-03 7.141914e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0008_0.tex <==
1 6.380750e-01 2.858333e+06 4.000000e+00
2 3.174000e-01 1.429167e+06 4.000000e+00
4 2.351250e-01 7.145833e+05 4.000000e+00
8 1.154250e-01 3.572916e+05 4.000000e+00
16 4.365000e-02 1.786458e+05 4.000000e+00
32 2.647500e-02 8.932291e+04 4.000000e+00
64 1.195000e-02 4.466145e+04 4.000000e+00
128 8.175000e-03 2.233073e+04 4.000000e+00
256 6.450000e-03 1.116536e+04 4.000000e+00
512 6.350000e-03 5.582682e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0008_1.tex <==
1 4.881333e-01 2.858333e+06 3.000000e+00
2 2.498667e-01 1.429167e+06 3.000000e+00
4 1.940667e-01 7.145833e+05 3.000000e+00
8 1.005000e-01 3.572916e+05 3.000000e+00
16 3.323333e-02 1.786458e+05 3.000000e+00
32 2.183333e-02 8.932291e+04 3.000000e+00
64 1.113333e-02 4.466145e+04 3.000000e+00
128 7.433333e-03 2.233073e+04 3.000000e+00
256 5.466667e-03 1.116536e+04 3.000000e+00
512 4.966667e-03 5.582682e+03 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0008_2.tex <==
1 4.728333e-01 2.858333e+06 3.000000e+00
2 2.352667e-01 1.429167e+06 3.000000e+00
4 1.843667e-01 7.145833e+05 3.000000e+00
8 9.116667e-02 3.572916e+05 3.000000e+00
16 3.320000e-02 1.786458e+05 3.000000e+00
32 2.033333e-02 8.932291e+04 3.000000e+00
64 1.016667e-02 4.466145e+04 3.000000e+00
128 6.900000e-03 2.233073e+04 3.000000e+00
256 5.666667e-03 1.116536e+04 3.000000e+00
512 6.666667e-03 5.582682e+03 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0009_0.tex <==
8 9.248500e-01 2.826665e+06 4.000000e+00
16 3.423500e-01 1.413332e+06 4.000000e+00
32 2.473750e-01 7.066662e+05 4.000000e+00
64 1.042500e-01 3.533331e+05 4.000000e+00
128 6.072500e-02 1.766665e+05 4.000000e+00
256 2.840000e-02 8.833327e+04 4.000000e+00
512 1.522500e-02 4.416664e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0009_1.tex <==
8 7.906333e-01 2.826665e+06 3.000000e+00
16 2.724667e-01 1.413332e+06 3.000000e+00
32 2.079000e-01 7.066662e+05 3.000000e+00
64 8.503333e-02 3.533331e+05 3.000000e+00
128 5.136667e-02 1.766665e+05 3.000000e+00
256 2.473333e-02 8.833327e+04 3.000000e+00
512 1.373333e-02 4.416664e+04 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0009_2.tex <==
8 7.229000e-01 2.826665e+06 3.000000e+00
16 2.504667e-01 1.413332e+06 3.000000e+00
32 1.882000e-01 7.066662e+05 3.000000e+00
64 7.673333e-02 3.533331e+05 3.000000e+00
128 4.640000e-02 1.766665e+05 3.000000e+00
256 2.233333e-02 8.833327e+04 3.000000e+00
512 1.273333e-02 4.416664e+04 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0010_0.tex <==
64 8.141500e-01 2.811284e+06 4.000000e+00
128 5.355500e-01 1.405642e+06 4.000000e+00
256 2.600250e-01 7.028210e+05 4.000000e+00
512 1.416250e-01 3.514105e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0010_1.tex <==
64 8.552000e-01 2.811284e+06 3.000000e+00
128 4.259333e-01 1.405642e+06 3.000000e+00
256 2.183000e-01 7.028210e+05 3.000000e+00
512 1.129333e-01 3.514105e+05 3.000000e+00


==> global-coarsening-paper-data/large-scaling-partitioning/hmg-quadrant-4/data_0010_2.tex <==
64 8.493333e-01 2.811284e+06 3.000000e+00
128 3.836667e-01 1.405642e+06 3.000000e+00
256 1.952333e-01 7.028210e+05 3.000000e+00
512 1.011000e-01 3.514105e+05 3.000000e+00


==> global-coarsening-paper-data/large-scaling/comp.tex <==
8 & 4 & 8.31e-1 & 3 & 5.42e-1 & 4 & 8.76e-1 & 4 & 8.63e-1\\
16 & 4 & 4.24e-1 & 3 & 2.75e-1 & 4 & 4.35e-1 & 4 & 4.28e-1\\
32 & 4 & 3.03e-1 & 3 & 2.26e-1 & 4 & 2.20e-1 & 4 & 2.17e-1\\
64 & 4 & 1.60e-1 & 3 & 1.14e-1 & 4 & 1.07e-1 & 4 & 1.06e-1\\
128 & 4 & 8.11e-2 & 3 & 5.66e-2 & 4 & 5.02e-2 & 4 & 5.02e-2\\
256 & 4 & 3.49e-2 & 3 & 2.77e-2 & 4 & 2.43e-2 & 4 & 2.52e-2\\
512 & 4 & 1.86e-2 & 3 & 1.49e-2 & 4 & 1.49e-2 & 4 & 1.47e-2\\
1024 & 4 & 1.25e-2 & 3 & 1.06e-2 & 4 & 1.37e-2 & 4 & 1.26e-2\\


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0003_gc_1.tex <==
1 1.000000e-04 2.083300e-02 1.000000e+02 5.625000e-01 1.000000e+00
2 1.000000e-04 1.041700e-02 1.000000e+02 2.812500e-01 1.000000e+00
4 1.000000e-04 5.208300e-03 1.000000e+02 1.406250e-01 1.000000e+00
8 1.000000e-04 2.604200e-03 1.000000e+02 7.031250e-02 1.000000e+00
16 1.000000e-04 1.302100e-03 1.000000e+02 3.515625e-02 1.000000e+00
32 1.000000e-04 6.510400e-04 1.000000e+02 1.757812e-02 1.000000e+00
64 1.000000e-04 3.255200e-04 1.000000e+02 8.789062e-03 1.000000e+00
128 1.000000e-04 1.627600e-04 2.000000e+02 4.394531e-03 1.000000e+00
256 2.000000e-04 8.138000e-05 1.000000e+02 2.197266e-03 1.000000e+00
512 2.000000e-04 4.069000e-05 1.000000e+02 1.098633e-03 1.000000e+00
1024 3.000000e-04 2.034500e-05 1.333333e+02 5.493164e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0003_gc_4.tex <==
1 1.750000e-04 2.083300e-02 8.571429e+01 1.518750e+01 4.000000e+00
2 1.750000e-04 1.041700e-02 1.000000e+02 7.593750e+00 4.000000e+00
4 1.750000e-04 5.208300e-03 1.000000e+02 3.796875e+00 4.000000e+00
8 2.000000e-04 2.604200e-03 8.750000e+01 1.898438e+00 4.000000e+00
16 2.000000e-04 1.302100e-03 8.750000e+01 9.492188e-01 4.000000e+00
32 2.250000e-04 6.510400e-04 8.888889e+01 4.746094e-01 4.000000e+00
64 2.250000e-04 3.255200e-04 8.888889e+01 2.373047e-01 4.000000e+00
128 2.250000e-04 1.627600e-04 8.888889e+01 1.186523e-01 4.000000e+00
256 2.500000e-04 8.138000e-05 1.000000e+02 5.932617e-02 4.000000e+00
512 2.750000e-04 4.069000e-05 1.090909e+02 2.966309e-02 4.000000e+00
1024 3.000000e-04 2.034500e-05 1.083333e+02 1.483154e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0003_ls_1.tex <==
1 1.000000e-04 2.083300e-02 0.000000e+00 5.625000e-01 1.000000e+00
2 1.000000e-04 1.041700e-02 0.000000e+00 2.812500e-01 1.000000e+00
4 1.000000e-04 5.208300e-03 0.000000e+00 1.406250e-01 1.000000e+00
8 1.000000e-04 2.604200e-03 0.000000e+00 7.031250e-02 1.000000e+00
16 1.000000e-04 1.302100e-03 0.000000e+00 3.515625e-02 1.000000e+00
32 1.000000e-04 6.510400e-04 0.000000e+00 1.757812e-02 1.000000e+00
64 1.000000e-04 3.255200e-04 0.000000e+00 8.789062e-03 1.000000e+00
128 2.000000e-04 1.627600e-04 0.000000e+00 4.394531e-03 1.000000e+00
256 2.000000e-04 8.138000e-05 0.000000e+00 2.197266e-03 1.000000e+00
512 2.000000e-04 4.069000e-05 0.000000e+00 1.098633e-03 1.000000e+00
1024 4.000000e-04 2.034500e-05 0.000000e+00 5.493164e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0003_ls_4.tex <==
1 1.500000e-04 0.000000e+00 0.000000e+00 1.518750e+01 4.000000e+00
2 1.750000e-04 0.000000e+00 0.000000e+00 7.593750e+00 4.000000e+00
4 1.750000e-04 0.000000e+00 0.000000e+00 3.796875e+00 4.000000e+00
8 1.750000e-04 0.000000e+00 0.000000e+00 1.898438e+00 4.000000e+00
16 1.750000e-04 0.000000e+00 0.000000e+00 9.492188e-01 4.000000e+00
32 2.000000e-04 0.000000e+00 0.000000e+00 4.746094e-01 4.000000e+00
64 2.000000e-04 0.000000e+00 0.000000e+00 2.373047e-01 4.000000e+00
128 2.000000e-04 0.000000e+00 0.000000e+00 1.186523e-01 4.000000e+00
256 2.500000e-04 0.000000e+00 0.000000e+00 5.932617e-02 4.000000e+00
512 3.000000e-04 0.000000e+00 0.000000e+00 2.966309e-02 4.000000e+00
1024 3.250000e-04 0.000000e+00 0.000000e+00 1.483154e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0004_gc_1.tex <==
1 1.000000e-04 2.083300e-02 1.000000e+02 5.625000e-01 1.000000e+00
2 1.000000e-04 1.041700e-02 1.000000e+02 2.812500e-01 1.000000e+00
4 1.000000e-04 5.208300e-03 1.000000e+02 1.406250e-01 1.000000e+00
8 1.000000e-04 2.604200e-03 1.000000e+02 7.031250e-02 1.000000e+00
16 1.000000e-04 1.302100e-03 1.000000e+02 3.515625e-02 1.000000e+00
32 1.000000e-04 6.510400e-04 1.000000e+02 1.757812e-02 1.000000e+00
64 1.000000e-04 3.255200e-04 2.000000e+02 8.789062e-03 1.000000e+00
128 2.000000e-04 1.627600e-04 1.000000e+02 4.394531e-03 1.000000e+00
256 2.000000e-04 8.138000e-05 1.000000e+02 2.197266e-03 1.000000e+00
512 2.000000e-04 4.069000e-05 1.000000e+02 1.098633e-03 1.000000e+00
1024 2.000000e-04 2.034500e-05 2.000000e+02 5.493164e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0004_gc_4.tex <==
1 1.750000e-04 2.083300e-02 8.571429e+01 1.518750e+01 4.000000e+00
2 1.750000e-04 1.041700e-02 1.000000e+02 7.593750e+00 4.000000e+00
4 1.750000e-04 5.208300e-03 1.000000e+02 3.796875e+00 4.000000e+00
8 2.000000e-04 2.604200e-03 8.750000e+01 1.898438e+00 4.000000e+00
16 2.000000e-04 1.302100e-03 8.750000e+01 9.492188e-01 4.000000e+00
32 2.250000e-04 6.510400e-04 1.000000e+02 4.746094e-01 4.000000e+00
64 2.250000e-04 3.255200e-04 8.888889e+01 2.373047e-01 4.000000e+00
128 2.250000e-04 1.627600e-04 8.888889e+01 1.186523e-01 4.000000e+00
256 2.500000e-04 8.138000e-05 1.100000e+02 5.932617e-02 4.000000e+00
512 2.750000e-04 4.069000e-05 1.000000e+02 2.966309e-02 4.000000e+00
1024 2.750000e-04 2.034500e-05 1.454545e+02 1.483154e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0004_ls_1.tex <==
1 1.000000e-04 2.083300e-02 0.000000e+00 5.625000e-01 1.000000e+00
2 1.000000e-04 1.041700e-02 0.000000e+00 2.812500e-01 1.000000e+00
4 1.000000e-04 5.208300e-03 0.000000e+00 1.406250e-01 1.000000e+00
8 1.000000e-04 2.604200e-03 0.000000e+00 7.031250e-02 1.000000e+00
16 1.000000e-04 1.302100e-03 0.000000e+00 3.515625e-02 1.000000e+00
32 1.000000e-04 6.510400e-04 0.000000e+00 1.757812e-02 1.000000e+00
64 2.000000e-04 3.255200e-04 0.000000e+00 8.789062e-03 1.000000e+00
128 2.000000e-04 1.627600e-04 0.000000e+00 4.394531e-03 1.000000e+00
256 2.000000e-04 8.138000e-05 0.000000e+00 2.197266e-03 1.000000e+00
512 2.000000e-04 4.069000e-05 0.000000e+00 1.098633e-03 1.000000e+00
1024 4.000000e-04 2.034500e-05 0.000000e+00 5.493164e-04 1.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0004_ls_4.tex <==
1 1.500000e-04 0.000000e+00 0.000000e+00 1.518750e+01 4.000000e+00
2 1.750000e-04 0.000000e+00 0.000000e+00 7.593750e+00 4.000000e+00
4 1.750000e-04 0.000000e+00 0.000000e+00 3.796875e+00 4.000000e+00
8 1.750000e-04 0.000000e+00 0.000000e+00 1.898438e+00 4.000000e+00
16 1.750000e-04 0.000000e+00 0.000000e+00 9.492188e-01 4.000000e+00
32 2.250000e-04 0.000000e+00 0.000000e+00 4.746094e-01 4.000000e+00
64 2.000000e-04 0.000000e+00 0.000000e+00 2.373047e-01 4.000000e+00
128 2.000000e-04 0.000000e+00 0.000000e+00 1.186523e-01 4.000000e+00
256 2.750000e-04 0.000000e+00 0.000000e+00 5.932617e-02 4.000000e+00
512 2.750000e-04 0.000000e+00 0.000000e+00 2.966309e-02 4.000000e+00
1024 4.000000e-04 0.000000e+00 0.000000e+00 1.483154e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0005_gc_1.tex <==
1 6.250000e-04 5.699600e-01 1.120000e+02 4.093750e+01 4.000000e+00
2 7.250000e-04 3.602600e-01 1.213793e+02 2.046875e+01 4.000000e+00
4 7.500000e-04 1.871900e-01 1.200000e+02 1.023438e+01 4.000000e+00
8 7.750000e-04 1.136500e-01 1.187097e+02 5.117188e+00 4.000000e+00
16 7.750000e-04 5.821300e-02 1.135484e+02 2.558594e+00 4.000000e+00
32 7.750000e-04 2.841300e-02 1.212903e+02 1.279297e+00 4.000000e+00
64 8.250000e-04 1.455300e-02 1.187879e+02 6.396484e-01 4.000000e+00
128 8.000000e-04 7.276600e-03 1.250000e+02 3.198242e-01 4.000000e+00
256 8.000000e-04 3.638300e-03 1.275000e+02 1.599121e-01 4.000000e+00
512 8.250000e-04 1.819100e-03 1.284848e+02 7.995605e-02 4.000000e+00
1024 8.250000e-04 9.095700e-04 1.600000e+02 3.997803e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0005_gc_4.tex <==
1 1.475000e-03 5.699600e-01 8.644068e+01 1.928688e+03 4.000000e+00
2 1.575000e-03 3.535900e-01 8.888889e+01 9.643438e+02 4.000000e+00
4 1.600000e-03 2.169700e-01 8.750000e+01 4.821719e+02 4.000000e+00
8 1.625000e-03 1.136500e-01 8.769231e+01 2.410859e+02 4.000000e+00
16 1.600000e-03 5.821300e-02 8.906250e+01 1.205430e+02 4.000000e+00
32 1.625000e-03 2.841300e-02 9.384615e+01 6.027148e+01 4.000000e+00
64 1.725000e-03 1.455300e-02 9.130435e+01 3.013574e+01 4.000000e+00
128 1.650000e-03 7.276600e-03 1.030303e+02 1.506787e+01 4.000000e+00
256 1.700000e-03 3.638300e-03 9.264706e+01 7.533936e+00 4.000000e+00
512 1.700000e-03 1.819100e-03 9.411765e+01 3.766968e+00 4.000000e+00
1024 1.700000e-03 9.095700e-04 9.705882e+01 1.883484e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0005_ls_1.tex <==
1 7.000000e-04 3.568000e-01 0.000000e+00 4.093750e+01 5.000000e+00
2 8.800000e-04 2.659200e-01 0.000000e+00 2.046875e+01 5.000000e+00
4 9.000000e-04 2.202100e-01 0.000000e+00 1.023438e+01 5.000000e+00
8 9.200000e-04 1.258400e-01 0.000000e+00 5.117188e+00 5.000000e+00
16 8.800000e-04 6.291900e-02 0.000000e+00 2.558594e+00 5.000000e+00
32 9.400000e-04 3.262400e-02 0.000000e+00 1.279297e+00 5.000000e+00
64 9.800000e-04 1.631200e-02 0.000000e+00 6.396484e-01 5.000000e+00
128 1.000000e-03 8.156100e-03 0.000000e+00 3.198242e-01 5.000000e+00
256 1.020000e-03 4.078100e-03 0.000000e+00 1.599121e-01 5.000000e+00
512 1.060000e-03 2.039000e-03 0.000000e+00 7.995605e-02 5.000000e+00
1024 1.320000e-03 1.019500e-03 0.000000e+00 3.997803e-02 5.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0005_ls_4.tex <==
1 1.275000e-03 0.000000e+00 0.000000e+00 1.928688e+03 4.000000e+00
2 1.400000e-03 0.000000e+00 0.000000e+00 9.643438e+02 4.000000e+00
4 1.400000e-03 0.000000e+00 0.000000e+00 4.821719e+02 4.000000e+00
8 1.425000e-03 0.000000e+00 0.000000e+00 2.410859e+02 4.000000e+00
16 1.425000e-03 0.000000e+00 0.000000e+00 1.205430e+02 4.000000e+00
32 1.525000e-03 0.000000e+00 0.000000e+00 6.027148e+01 4.000000e+00
64 1.575000e-03 0.000000e+00 0.000000e+00 3.013574e+01 4.000000e+00
128 1.700000e-03 0.000000e+00 0.000000e+00 1.506787e+01 4.000000e+00
256 1.575000e-03 0.000000e+00 0.000000e+00 7.533936e+00 4.000000e+00
512 1.600000e-03 0.000000e+00 0.000000e+00 3.766968e+00 4.000000e+00
1024 1.650000e-03 0.000000e+00 0.000000e+00 1.883484e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0006_gc_1.tex <==
1 8.750000e-04 8.327000e-01 1.074286e+02 2.033958e+02 4.000000e+00
2 9.750000e-04 6.919200e-01 1.128205e+02 1.016979e+02 4.000000e+00
4 1.050000e-03 5.227000e-01 1.219048e+02 5.084896e+01 4.000000e+00
8 1.125000e-03 3.588700e-01 1.191111e+02 2.542448e+01 4.000000e+00
16 1.125000e-03 2.072800e-01 1.208889e+02 1.271224e+01 4.000000e+00
32 1.100000e-03 1.134200e-01 1.254545e+02 6.356120e+00 4.000000e+00
64 1.200000e-03 6.011100e-02 1.166667e+02 3.178060e+00 4.000000e+00
128 1.125000e-03 3.005500e-02 1.280000e+02 1.589030e+00 4.000000e+00
256 1.150000e-03 1.533400e-02 1.234783e+02 7.945150e-01 4.000000e+00
512 1.150000e-03 7.667200e-03 1.217391e+02 3.972575e-01 4.000000e+00
1024 1.150000e-03 3.833600e-03 1.304348e+02 1.986287e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0006_gc_4.tex <==
1 3.250000e-03 8.327000e-01 9.692308e+01 1.062652e+04 4.000000e+00
2 2.650000e-03 7.020200e-01 9.528302e+01 5.313260e+03 4.000000e+00
4 2.400000e-03 5.227000e-01 9.062500e+01 2.656630e+03 4.000000e+00
8 2.350000e-03 3.588700e-01 9.042553e+01 1.328315e+03 4.000000e+00
16 2.275000e-03 2.072800e-01 9.120879e+01 6.641576e+02 4.000000e+00
32 2.375000e-03 1.134200e-01 8.736842e+01 3.320788e+02 4.000000e+00
64 2.350000e-03 6.011100e-02 8.829787e+01 1.660394e+02 4.000000e+00
128 2.450000e-03 3.005500e-02 8.571429e+01 8.301969e+01 4.000000e+00
256 2.350000e-03 1.533400e-02 8.829787e+01 4.150985e+01 4.000000e+00
512 2.275000e-03 7.667200e-03 9.120879e+01 2.075492e+01 4.000000e+00
1024 2.250000e-03 3.833600e-03 1.011111e+02 1.037746e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0006_ls_1.tex <==
1 9.400000e-04 4.389600e-01 0.000000e+00 2.033958e+02 5.000000e+00
2 1.100000e-03 3.435700e-01 0.000000e+00 1.016979e+02 5.000000e+00
4 1.280000e-03 2.827300e-01 0.000000e+00 5.084896e+01 5.000000e+00
8 1.340000e-03 2.261900e-01 0.000000e+00 2.542448e+01 5.000000e+00
16 1.360000e-03 1.754900e-01 0.000000e+00 1.271224e+01 5.000000e+00
32 1.380000e-03 1.375500e-01 0.000000e+00 6.356120e+00 5.000000e+00
64 1.400000e-03 6.696300e-02 0.000000e+00 3.178060e+00 5.000000e+00
128 1.440000e-03 3.534200e-02 0.000000e+00 1.589030e+00 5.000000e+00
256 1.420000e-03 1.817600e-02 0.000000e+00 7.945150e-01 5.000000e+00
512 1.400000e-03 9.087800e-03 0.000000e+00 3.972575e-01 5.000000e+00
1024 1.500000e-03 4.543900e-03 0.000000e+00 1.986287e-01 5.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0006_ls_4.tex <==
1 3.150000e-03 0.000000e+00 0.000000e+00 1.062652e+04 4.000000e+00
2 2.525000e-03 0.000000e+00 0.000000e+00 5.313260e+03 4.000000e+00
4 2.175000e-03 0.000000e+00 0.000000e+00 2.656630e+03 4.000000e+00
8 2.125000e-03 0.000000e+00 0.000000e+00 1.328315e+03 4.000000e+00
16 2.075000e-03 0.000000e+00 0.000000e+00 6.641576e+02 4.000000e+00
32 2.075000e-03 0.000000e+00 0.000000e+00 3.320788e+02 4.000000e+00
64 2.075000e-03 0.000000e+00 0.000000e+00 1.660394e+02 4.000000e+00
128 2.100000e-03 0.000000e+00 0.000000e+00 8.301969e+01 4.000000e+00
256 2.075000e-03 0.000000e+00 0.000000e+00 4.150985e+01 4.000000e+00
512 2.075000e-03 0.000000e+00 0.000000e+00 2.075492e+01 4.000000e+00
1024 2.275000e-03 0.000000e+00 0.000000e+00 1.037746e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0007_gc_1.tex <==
1 1.550000e-03 9.568600e-01 9.677419e+01 1.000854e+03 4.000000e+00
2 1.475000e-03 9.105600e-01 1.071186e+02 5.004271e+02 4.000000e+00
4 1.500000e-03 8.356800e-01 1.133333e+02 2.502135e+02 4.000000e+00
8 1.550000e-03 7.136100e-01 1.161290e+02 1.251068e+02 4.000000e+00
16 1.675000e-03 5.428400e-01 1.086567e+02 6.255339e+01 4.000000e+00
32 1.925000e-03 3.826000e-01 1.018182e+02 3.127669e+01 4.000000e+00
64 1.900000e-03 2.335000e-01 1.136842e+02 1.563835e+01 4.000000e+00
128 1.700000e-03 1.202900e-01 1.141176e+02 7.819173e+00 4.000000e+00
256 1.750000e-03 6.843900e-02 1.154286e+02 3.909587e+00 4.000000e+00
512 1.750000e-03 3.482000e-02 1.200000e+02 1.954793e+00 4.000000e+00
1024 1.700000e-03 1.741000e-02 1.258824e+02 9.773966e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0007_gc_4.tex <==
1 1.110000e-02 9.568600e-01 1.042793e+02 5.512835e+04 4.000000e+00
2 6.775000e-03 9.105600e-01 1.140221e+02 2.756418e+04 4.000000e+00
4 4.700000e-03 8.356800e-01 1.122340e+02 1.378209e+04 4.000000e+00
8 4.075000e-03 7.217200e-01 9.263804e+01 6.891044e+03 4.000000e+00
16 3.650000e-03 5.475100e-01 8.424658e+01 3.445522e+03 4.000000e+00
32 3.400000e-03 3.826000e-01 9.558824e+01 1.722761e+03 4.000000e+00
64 3.650000e-03 2.335000e-01 9.246575e+01 8.613805e+02 4.000000e+00
128 3.250000e-03 1.323200e-01 9.461538e+01 4.306903e+02 4.000000e+00
256 2.950000e-03 6.843900e-02 1.186441e+02 2.153451e+02 4.000000e+00
512 3.150000e-03 3.482000e-02 8.571429e+01 1.076726e+02 4.000000e+00
1024 2.975000e-03 1.741000e-02 1.042017e+02 5.383628e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0007_ls_1.tex <==
1 1.500000e-03 5.358800e-01 0.000000e+00 1.000854e+03 5.000000e+00
2 1.580000e-03 3.836000e-01 0.000000e+00 5.004271e+02 5.000000e+00
4 1.700000e-03 3.427400e-01 0.000000e+00 2.502135e+02 5.000000e+00
8 1.800000e-03 3.130400e-01 0.000000e+00 1.251068e+02 5.000000e+00
16 1.820000e-03 2.598800e-01 0.000000e+00 6.255339e+01 5.000000e+00
32 1.960000e-03 2.334500e-01 0.000000e+00 3.127669e+01 5.000000e+00
64 2.160000e-03 1.996200e-01 0.000000e+00 1.563835e+01 5.000000e+00
128 1.940000e-03 1.601600e-01 0.000000e+00 7.819173e+00 5.000000e+00
256 2.020000e-03 9.306600e-02 0.000000e+00 3.909587e+00 5.000000e+00
512 2.100000e-03 4.782600e-02 0.000000e+00 1.954793e+00 5.000000e+00
1024 2.140000e-03 2.391300e-02 0.000000e+00 9.773966e-01 5.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0007_ls_4.tex <==
1 1.157500e-02 0.000000e+00 0.000000e+00 5.512835e+04 4.000000e+00
2 7.725000e-03 0.000000e+00 0.000000e+00 2.756418e+04 4.000000e+00
4 5.275000e-03 0.000000e+00 0.000000e+00 1.378209e+04 4.000000e+00
8 3.775000e-03 0.000000e+00 0.000000e+00 6.891044e+03 4.000000e+00
16 3.075000e-03 0.000000e+00 0.000000e+00 3.445522e+03 4.000000e+00
32 3.250000e-03 0.000000e+00 0.000000e+00 1.722761e+03 4.000000e+00
64 3.375000e-03 0.000000e+00 0.000000e+00 8.613805e+02 4.000000e+00
128 3.075000e-03 0.000000e+00 0.000000e+00 4.306903e+02 4.000000e+00
256 3.500000e-03 0.000000e+00 0.000000e+00 2.153451e+02 4.000000e+00
512 2.700000e-03 0.000000e+00 0.000000e+00 1.076726e+02 4.000000e+00
1024 3.100000e-03 0.000000e+00 0.000000e+00 5.383628e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0008_gc_1.tex <==
1 4.625000e-03 9.427400e-01 1.020541e+02 6.605479e+03 4.000000e+00
2 3.175000e-03 9.837400e-01 1.159055e+02 3.302740e+03 4.000000e+00
4 2.525000e-03 8.514300e-01 1.164356e+02 1.651370e+03 4.000000e+00
8 2.300000e-03 9.383100e-01 1.147826e+02 8.256849e+02 4.000000e+00
16 2.350000e-03 8.788400e-01 1.131915e+02 4.128424e+02 4.000000e+00
32 2.875000e-03 7.912700e-01 8.765217e+01 2.064212e+02 4.000000e+00
64 3.575000e-03 6.461300e-01 7.720280e+01 1.032106e+02 4.000000e+00
128 3.950000e-03 3.714100e-01 9.215190e+01 5.160531e+01 4.000000e+00
256 3.100000e-03 3.102100e-01 1.116129e+02 2.580265e+01 4.000000e+00
512 2.550000e-03 1.796000e-01 1.247059e+02 1.290133e+01 4.000000e+00
1024 2.350000e-03 1.018600e-01 1.302128e+02 6.450663e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0008_gc_4.tex <==
1 8.105000e-02 9.926900e-01 1.106107e+02 3.870539e+05 4.000000e+00
2 3.985000e-02 8.647000e-01 1.255960e+02 1.935269e+05 4.000000e+00
4 2.015000e-02 8.514300e-01 1.310174e+02 9.676346e+04 4.000000e+00
8 1.122500e-02 9.383100e-01 1.360802e+02 4.838173e+04 4.000000e+00
16 8.475000e-03 7.044900e-01 1.176991e+02 2.419087e+04 4.000000e+00
32 6.325000e-03 6.442200e-01 1.039526e+02 1.209543e+04 4.000000e+00
64 5.675000e-03 6.461300e-01 9.162996e+01 6.047716e+03 4.000000e+00
128 4.550000e-03 4.831700e-01 1.120879e+02 3.023858e+03 4.000000e+00
256 4.475000e-03 3.102100e-01 1.184358e+02 1.511929e+03 4.000000e+00
512 4.875000e-03 1.664600e-01 1.071795e+02 7.559646e+02 4.000000e+00
1024 3.975000e-03 1.018600e-01 1.050314e+02 3.779823e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0008_ls_1.tex <==
1 4.720000e-03 5.555800e-01 0.000000e+00 6.605479e+03 5.000000e+00
2 3.680000e-03 4.324800e-01 0.000000e+00 3.302740e+03 5.000000e+00
4 2.940000e-03 4.029700e-01 0.000000e+00 1.651370e+03 5.000000e+00
8 2.640000e-03 3.632300e-01 0.000000e+00 8.256849e+02 5.000000e+00
16 2.660000e-03 3.288200e-01 0.000000e+00 4.128424e+02 5.000000e+00
32 2.520000e-03 2.913200e-01 0.000000e+00 2.064212e+02 5.000000e+00
64 2.760000e-03 2.685800e-01 0.000000e+00 1.032106e+02 5.000000e+00
128 3.640000e-03 2.513000e-01 0.000000e+00 5.160531e+01 5.000000e+00
256 3.460000e-03 2.307400e-01 0.000000e+00 2.580265e+01 5.000000e+00
512 3.180000e-03 1.812900e-01 0.000000e+00 1.290133e+01 5.000000e+00
1024 3.060000e-03 1.442100e-01 0.000000e+00 6.450663e+00 5.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0008_ls_4.tex <==
1 8.965000e-02 0.000000e+00 0.000000e+00 3.870539e+05 4.000000e+00
2 5.005000e-02 0.000000e+00 0.000000e+00 1.935269e+05 4.000000e+00
4 2.640000e-02 0.000000e+00 0.000000e+00 9.676346e+04 4.000000e+00
8 1.527500e-02 0.000000e+00 0.000000e+00 4.838173e+04 4.000000e+00
16 9.975000e-03 0.000000e+00 0.000000e+00 2.419087e+04 4.000000e+00
32 6.575000e-03 0.000000e+00 0.000000e+00 1.209543e+04 4.000000e+00
64 5.200000e-03 0.000000e+00 0.000000e+00 6.047716e+03 4.000000e+00
128 5.100000e-03 0.000000e+00 0.000000e+00 3.023858e+03 4.000000e+00
256 5.300000e-03 0.000000e+00 0.000000e+00 1.511929e+03 4.000000e+00
512 5.225000e-03 0.000000e+00 0.000000e+00 7.559646e+02 4.000000e+00
1024 4.175000e-03 0.000000e+00 0.000000e+00 3.779823e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0009_gc_1.tex <==
1 2.302500e-02 9.734100e-01 1.226493e+02 4.869377e+04 4.000000e+00
2 1.362500e-02 8.756900e-01 1.378349e+02 2.434689e+04 4.000000e+00
4 8.125000e-03 8.124600e-01 1.363692e+02 1.217344e+04 4.000000e+00
8 5.400000e-03 8.088000e-01 1.266667e+02 6.086721e+03 4.000000e+00
16 4.050000e-03 9.143000e-01 1.219753e+02 3.043361e+03 4.000000e+00
32 4.300000e-03 7.893500e-01 9.302326e+01 1.521680e+03 4.000000e+00
64 4.550000e-03 9.239800e-01 8.967033e+01 7.608402e+02 4.000000e+00
128 6.200000e-03 8.125600e-01 7.322581e+01 3.804201e+02 4.000000e+00
256 7.675000e-03 7.562200e-01 6.228013e+01 1.902100e+02 4.000000e+00
512 6.775000e-03 5.988500e-01 7.084871e+01 9.510502e+01 4.000000e+00
1024 5.925000e-03 4.316700e-01 9.822785e+01 4.755251e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0009_gc_4.tex <==
1 5.828250e-01 9.520900e-01 1.238022e+02 2.974569e+06 4.000000e+00
2 2.949750e-01 9.306600e-01 1.405289e+02 1.487285e+06 4.000000e+00
4 1.501750e-01 9.265000e-01 1.447811e+02 7.436423e+05 4.000000e+00
8 7.507500e-02 9.224400e-01 1.570763e+02 3.718211e+05 4.000000e+00
16 5.562500e-02 8.551100e-01 1.419326e+02 1.859106e+05 4.000000e+00
32 2.717500e-02 8.418600e-01 1.638454e+02 9.295528e+04 4.000000e+00
64 1.600000e-02 8.133600e-01 1.439062e+02 4.647764e+04 4.000000e+00
128 9.575000e-03 7.660000e-01 1.274151e+02 2.323882e+04 4.000000e+00
256 7.225000e-03 6.838400e-01 1.231834e+02 1.161941e+04 4.000000e+00
512 6.075000e-03 5.368000e-01 1.168724e+02 5.809705e+03 4.000000e+00
1024 5.450000e-03 4.316700e-01 1.376147e+02 2.904853e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0009_ls_1.tex <==
1 2.824000e-02 5.538400e-01 0.000000e+00 4.869377e+04 5.000000e+00
2 1.878000e-02 4.337600e-01 0.000000e+00 2.434689e+04 5.000000e+00
4 1.108000e-02 4.064700e-01 0.000000e+00 1.217344e+04 5.000000e+00
8 6.840000e-03 3.675800e-01 0.000000e+00 6.086721e+03 5.000000e+00
16 4.940000e-03 3.384200e-01 0.000000e+00 3.043361e+03 5.000000e+00
32 4.000000e-03 2.993400e-01 0.000000e+00 1.521680e+03 5.000000e+00
64 4.080000e-03 2.880300e-01 0.000000e+00 7.608402e+02 5.000000e+00
128 4.540000e-03 2.780700e-01 0.000000e+00 3.804201e+02 5.000000e+00
256 4.780000e-03 2.739000e-01 0.000000e+00 1.902100e+02 5.000000e+00
512 4.800000e-03 2.652300e-01 0.000000e+00 9.510502e+01 5.000000e+00
1024 5.820000e-03 2.475900e-01 0.000000e+00 4.755251e+01 5.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0009_ls_4.tex <==
1 7.215500e-01 0.000000e+00 0.000000e+00 2.974569e+06 4.000000e+00
2 4.145250e-01 0.000000e+00 0.000000e+00 1.487285e+06 4.000000e+00
4 2.174250e-01 0.000000e+00 0.000000e+00 7.436423e+05 4.000000e+00
8 1.179250e-01 0.000000e+00 0.000000e+00 3.718211e+05 4.000000e+00
16 7.895000e-02 0.000000e+00 0.000000e+00 1.859106e+05 4.000000e+00
32 4.452500e-02 0.000000e+00 0.000000e+00 9.295528e+04 4.000000e+00
64 2.302500e-02 0.000000e+00 0.000000e+00 4.647764e+04 4.000000e+00
128 1.220000e-02 0.000000e+00 0.000000e+00 2.323882e+04 4.000000e+00
256 8.900000e-03 0.000000e+00 0.000000e+00 1.161941e+04 4.000000e+00
512 7.100000e-03 0.000000e+00 0.000000e+00 5.809705e+03 4.000000e+00
1024 7.500000e-03 0.000000e+00 0.000000e+00 2.904853e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0010_gc_1.tex <==
1 1.560500e-01 9.998500e-01 1.340852e+02 3.747775e+05 4.000000e+00
2 7.952500e-02 9.318500e-01 1.593964e+02 1.873888e+05 4.000000e+00
4 4.132500e-02 8.969400e-01 1.695342e+02 9.369438e+04 4.000000e+00
8 2.215000e-02 8.963200e-01 1.822122e+02 4.684719e+04 4.000000e+00
16 1.415000e-02 8.658100e-01 1.683392e+02 2.342360e+04 4.000000e+00
32 1.007500e-02 9.944200e-01 1.455087e+02 1.171180e+04 4.000000e+00
64 8.200000e-03 9.532500e-01 1.134146e+02 5.855899e+03 4.000000e+00
128 8.325000e-03 9.770800e-01 8.120120e+01 2.927949e+03 4.000000e+00
256 7.250000e-03 9.564600e-01 8.055172e+01 1.463975e+03 4.000000e+00
512 6.900000e-03 9.136200e-01 8.550725e+01 7.319873e+02 4.000000e+00
1024 9.975000e-03 8.445800e-01 6.656642e+01 3.659937e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0010_gc_4.tex <==
8 5.566000e-01 9.280900e-01 1.698123e+02 2.927377e+06 4.000000e+00
16 4.716750e-01 9.607900e-01 1.481211e+02 1.463688e+06 4.000000e+00
32 2.349250e-01 9.246900e-01 1.906672e+02 7.318442e+05 4.000000e+00
64 1.179500e-01 9.196700e-01 1.980924e+02 3.659221e+05 4.000000e+00
128 5.662500e-02 9.388500e-01 1.922737e+02 1.829610e+05 4.000000e+00
256 2.815000e-02 9.105600e-01 1.827709e+02 9.148052e+04 4.000000e+00
512 1.575000e-02 8.570000e-01 1.679365e+02 4.574026e+04 4.000000e+00
1024 1.027500e-02 7.998700e-01 1.476886e+02 2.287013e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0010_ls_1.tex <==
1 2.092400e-01 5.535500e-01 0.000000e+00 3.747775e+05 5.000000e+00
2 1.267600e-01 4.334000e-01 0.000000e+00 1.873888e+05 5.000000e+00
4 7.006000e-02 4.049300e-01 0.000000e+00 9.369438e+04 5.000000e+00
8 4.036000e-02 3.658600e-01 0.000000e+00 4.684719e+04 5.000000e+00
16 2.382000e-02 3.348800e-01 0.000000e+00 2.342360e+04 5.000000e+00
32 1.466000e-02 2.998800e-01 0.000000e+00 1.171180e+04 5.000000e+00
64 9.300000e-03 2.864100e-01 0.000000e+00 5.855899e+03 5.000000e+00
128 6.760000e-03 2.786000e-01 0.000000e+00 2.927949e+03 5.000000e+00
256 5.840000e-03 2.758200e-01 0.000000e+00 1.463975e+03 5.000000e+00
512 5.900000e-03 2.750200e-01 0.000000e+00 7.319873e+02 5.000000e+00
1024 6.640000e-03 2.732500e-01 0.000000e+00 3.659937e+02 5.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0010_ls_4.tex <==
8 9.451750e-01 0.000000e+00 0.000000e+00 2.927377e+06 4.000000e+00
16 6.986500e-01 0.000000e+00 0.000000e+00 1.463688e+06 4.000000e+00
32 4.479250e-01 0.000000e+00 0.000000e+00 7.318442e+05 4.000000e+00
64 2.336500e-01 0.000000e+00 0.000000e+00 3.659221e+05 4.000000e+00
128 1.088750e-01 0.000000e+00 0.000000e+00 1.829610e+05 4.000000e+00
256 5.145000e-02 0.000000e+00 0.000000e+00 9.148052e+04 4.000000e+00
512 2.645000e-02 0.000000e+00 0.000000e+00 4.574026e+04 4.000000e+00
1024 1.517500e-02 0.000000e+00 0.000000e+00 2.287013e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-annulus/data_0011_ls_1.tex <==
8 2.891400e-01 3.660900e-01 0.000000e+00 3.674826e+05 5.000000e+00
16 1.714200e-01 3.354100e-01 0.000000e+00 1.837413e+05 5.000000e+00
32 1.000600e-01 3.000900e-01 0.000000e+00 9.187066e+04 5.000000e+00
64 5.464000e-02 2.869100e-01 0.000000e+00 4.593533e+04 5.000000e+00
128 2.992000e-02 2.788300e-01 0.000000e+00 2.296766e+04 5.000000e+00
256 1.704000e-02 2.764000e-01 0.000000e+00 1.148383e+04 5.000000e+00
512 1.072000e-02 2.756900e-01 0.000000e+00 5.741916e+03 5.000000e+00
1024 8.480000e-03 2.755400e-01 0.000000e+00 2.870958e+03 5.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0003_gc_1.tex <==
1 2.250000e-04 1.200000e-01 1.444444e+02 4.645833e+00 4.000000e+00
2 2.250000e-04 6.000000e-02 1.666667e+02 2.322917e+00 4.000000e+00
4 2.250000e-04 3.000000e-02 1.666667e+02 1.161458e+00 4.000000e+00
8 2.500000e-04 1.500000e-02 1.600000e+02 5.807292e-01 4.000000e+00
16 2.500000e-04 7.500000e-03 1.600000e+02 2.903646e-01 4.000000e+00
32 2.750000e-04 3.750000e-03 1.545455e+02 1.451823e-01 4.000000e+00
64 2.500000e-04 1.875000e-03 1.900000e+02 7.259115e-02 4.000000e+00
128 2.750000e-04 9.375000e-04 1.818182e+02 3.629557e-02 4.000000e+00
256 3.000000e-04 4.687500e-04 1.833333e+02 1.814779e-02 4.000000e+00
512 3.250000e-04 2.343700e-04 1.615385e+02 9.073893e-03 4.000000e+00
1024 3.250000e-04 1.171900e-04 1.923077e+02 4.536947e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0003_gc_4.tex <==
1 5.750000e-04 1.200000e-01 1.086957e+02 1.936458e+02 4.000000e+00
2 6.000000e-04 6.000000e-02 1.125000e+02 9.682292e+01 4.000000e+00
4 6.000000e-04 3.000000e-02 1.125000e+02 4.841146e+01 4.000000e+00
8 6.000000e-04 1.500000e-02 1.083333e+02 2.420573e+01 4.000000e+00
16 6.000000e-04 7.500000e-03 1.083333e+02 1.210286e+01 4.000000e+00
32 6.500000e-04 3.750000e-03 1.038462e+02 6.051432e+00 4.000000e+00
64 6.500000e-04 1.875000e-03 1.153846e+02 3.025716e+00 4.000000e+00
128 6.750000e-04 9.375000e-04 1.111111e+02 1.512858e+00 4.000000e+00
256 6.750000e-04 4.687500e-04 1.259259e+02 7.564290e-01 4.000000e+00
512 7.000000e-04 2.343700e-04 1.250000e+02 3.782145e-01 4.000000e+00
1024 7.250000e-04 1.171900e-04 1.172414e+02 1.891073e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0003_ls_1.tex <==
1 3.250000e-04 1.585600e-01 0.000000e+00 4.645833e+00 4.000000e+00
2 3.750000e-04 7.928200e-02 0.000000e+00 2.322917e+00 4.000000e+00
4 3.750000e-04 3.964100e-02 0.000000e+00 1.161458e+00 4.000000e+00
8 4.000000e-04 1.982100e-02 0.000000e+00 5.807292e-01 4.000000e+00
16 4.000000e-04 9.910300e-03 0.000000e+00 2.903646e-01 4.000000e+00
32 4.250000e-04 4.955200e-03 0.000000e+00 1.451823e-01 4.000000e+00
64 4.750000e-04 2.477600e-03 0.000000e+00 7.259115e-02 4.000000e+00
128 5.000000e-04 1.238800e-03 0.000000e+00 3.629557e-02 4.000000e+00
256 5.500000e-04 6.193900e-04 0.000000e+00 1.814779e-02 4.000000e+00
512 5.250000e-04 3.097000e-04 0.000000e+00 9.073893e-03 4.000000e+00
1024 6.250000e-04 1.548500e-04 0.000000e+00 4.536947e-03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0003_ls_4.tex <==
1 6.250000e-04 0.000000e+00 0.000000e+00 1.936458e+02 4.000000e+00
2 6.750000e-04 0.000000e+00 0.000000e+00 9.682292e+01 4.000000e+00
4 6.750000e-04 0.000000e+00 0.000000e+00 4.841146e+01 4.000000e+00
8 6.500000e-04 0.000000e+00 0.000000e+00 2.420573e+01 4.000000e+00
16 6.500000e-04 0.000000e+00 0.000000e+00 1.210286e+01 4.000000e+00
32 6.750000e-04 0.000000e+00 0.000000e+00 6.051432e+00 4.000000e+00
64 7.500000e-04 0.000000e+00 0.000000e+00 3.025716e+00 4.000000e+00
128 7.500000e-04 0.000000e+00 0.000000e+00 1.512858e+00 4.000000e+00
256 8.500000e-04 0.000000e+00 0.000000e+00 7.564290e-01 4.000000e+00
512 8.750000e-04 0.000000e+00 0.000000e+00 3.782145e-01 4.000000e+00
1024 8.500000e-04 0.000000e+00 0.000000e+00 1.891073e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0004_gc_1.tex <==
1 3.750000e-04 4.000900e-01 1.666667e+02 2.100000e+01 4.000000e+00
2 4.000000e-04 2.146800e-01 1.562500e+02 1.050000e+01 4.000000e+00
4 4.000000e-04 1.333600e-01 1.625000e+02 5.250000e+00 4.000000e+00
8 4.000000e-04 6.472100e-02 1.687500e+02 2.625000e+00 4.000000e+00
16 4.250000e-04 3.334100e-02 1.588235e+02 1.312500e+00 4.000000e+00
32 4.250000e-04 1.667100e-02 1.705882e+02 6.562500e-01 4.000000e+00
64 4.250000e-04 8.335300e-03 1.823529e+02 3.281250e-01 4.000000e+00
128 4.500000e-04 4.167700e-03 1.833333e+02 1.640625e-01 4.000000e+00
256 4.750000e-04 2.083800e-03 2.052632e+02 8.203125e-02 4.000000e+00
512 4.750000e-04 1.041900e-03 2.263158e+02 4.101562e-02 4.000000e+00
1024 5.000000e-04 5.209600e-04 1.900000e+02 2.050781e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0004_gc_4.tex <==
1 1.050000e-03 3.592700e-01 9.523810e+01 1.053188e+03 4.000000e+00
2 1.025000e-03 2.146800e-01 9.268293e+01 5.265938e+02 4.000000e+00
4 1.025000e-03 1.294400e-01 1.000000e+02 2.632969e+02 4.000000e+00
8 1.025000e-03 6.668200e-02 1.024390e+02 1.316484e+02 4.000000e+00
16 1.050000e-03 3.334100e-02 1.047619e+02 6.582422e+01 4.000000e+00
32 1.050000e-03 1.667100e-02 1.071429e+02 3.291211e+01 4.000000e+00
64 1.050000e-03 8.335300e-03 1.309524e+02 1.645605e+01 4.000000e+00
128 1.100000e-03 4.167700e-03 1.181818e+02 8.228027e+00 4.000000e+00
256 1.075000e-03 2.083800e-03 1.186047e+02 4.114014e+00 4.000000e+00
512 1.100000e-03 1.041900e-03 1.181818e+02 2.057007e+00 4.000000e+00
1024 1.100000e-03 5.209600e-04 1.204545e+02 1.028503e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0004_ls_1.tex <==
1 6.250000e-04 3.973200e-01 0.000000e+00 2.100000e+01 4.000000e+00
2 6.250000e-04 3.337500e-01 0.000000e+00 1.050000e+01 4.000000e+00
4 6.500000e-04 1.896300e-01 0.000000e+00 5.250000e+00 4.000000e+00
8 6.750000e-04 1.043000e-01 0.000000e+00 2.625000e+00 4.000000e+00
16 6.750000e-04 5.489300e-02 0.000000e+00 1.312500e+00 4.000000e+00
32 7.250000e-04 2.744700e-02 0.000000e+00 6.562500e-01 4.000000e+00
64 7.750000e-04 1.372300e-02 0.000000e+00 3.281250e-01 4.000000e+00
128 8.250000e-04 6.861600e-03 0.000000e+00 1.640625e-01 4.000000e+00
256 9.750000e-04 3.430800e-03 0.000000e+00 8.203125e-02 4.000000e+00
512 1.075000e-03 1.715400e-03 0.000000e+00 4.101562e-02 4.000000e+00
1024 9.500000e-04 8.577000e-04 0.000000e+00 2.050781e-02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0004_ls_4.tex <==
1 1.000000e-03 0.000000e+00 0.000000e+00 1.053188e+03 4.000000e+00
2 9.500000e-04 0.000000e+00 0.000000e+00 5.265938e+02 4.000000e+00
4 1.025000e-03 0.000000e+00 0.000000e+00 2.632969e+02 4.000000e+00
8 1.050000e-03 0.000000e+00 0.000000e+00 1.316484e+02 4.000000e+00
16 1.100000e-03 0.000000e+00 0.000000e+00 6.582422e+01 4.000000e+00
32 1.125000e-03 0.000000e+00 0.000000e+00 3.291211e+01 4.000000e+00
64 1.375000e-03 0.000000e+00 0.000000e+00 1.645605e+01 4.000000e+00
128 1.300000e-03 0.000000e+00 0.000000e+00 8.228027e+00 4.000000e+00
256 1.275000e-03 0.000000e+00 0.000000e+00 4.114014e+00 4.000000e+00
512 1.300000e-03 0.000000e+00 0.000000e+00 2.057007e+00 4.000000e+00
1024 1.325000e-03 0.000000e+00 0.000000e+00 1.028503e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0005_gc_1.tex <==
1 6.250000e-04 7.469100e-01 1.440000e+02 1.188125e+02 4.000000e+00
2 6.500000e-04 6.224200e-01 1.461538e+02 5.940625e+01 4.000000e+00
4 6.500000e-04 4.385300e-01 1.500000e+02 2.970312e+01 4.000000e+00
8 6.750000e-04 2.894300e-01 1.481481e+02 1.485156e+01 4.000000e+00
16 6.750000e-04 1.682700e-01 1.444444e+02 7.425781e+00 4.000000e+00
32 6.750000e-04 8.413600e-02 1.518519e+02 3.712891e+00 4.000000e+00
64 7.000000e-04 4.412000e-02 1.500000e+02 1.856445e+00 4.000000e+00
128 7.250000e-04 2.206000e-02 2.068966e+02 9.282227e-01 4.000000e+00
256 7.000000e-04 1.103000e-02 1.714286e+02 4.641113e-01 4.000000e+00
512 7.500000e-04 5.515000e-03 1.633333e+02 2.320557e-01 4.000000e+00
1024 7.500000e-04 2.757500e-03 1.633333e+02 1.160278e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0005_gc_4.tex <==
1 2.133333e-03 7.469100e-01 1.148438e+02 6.692562e+03 3.000000e+00
2 1.800000e-03 6.224200e-01 1.041667e+02 3.346281e+03 3.000000e+00
4 1.700000e-03 4.319800e-01 1.014706e+02 1.673141e+03 3.000000e+00
8 1.666667e-03 2.894300e-01 9.900000e+01 8.365703e+02 3.000000e+00
16 1.600000e-03 1.682700e-01 9.687500e+01 4.182852e+02 3.000000e+00
32 1.600000e-03 8.824000e-02 1.031250e+02 2.091426e+02 3.000000e+00
64 1.666667e-03 4.412000e-02 9.900000e+01 1.045713e+02 3.000000e+00
128 1.733333e-03 2.206000e-02 9.807692e+01 5.228564e+01 3.000000e+00
256 1.666667e-03 1.103000e-02 1.035000e+02 2.614282e+01 3.000000e+00
512 1.700000e-03 5.515000e-03 1.205882e+02 1.307141e+01 3.000000e+00
1024 1.700000e-03 2.757500e-03 1.029412e+02 6.535706e+00 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0005_ls_1.tex <==
1 9.000000e-04 4.505500e-01 0.000000e+00 1.188125e+02 4.000000e+00
2 9.500000e-04 4.094400e-01 0.000000e+00 5.940625e+01 4.000000e+00
4 9.750000e-04 3.642500e-01 0.000000e+00 2.970312e+01 4.000000e+00
8 1.000000e-03 2.921500e-01 0.000000e+00 1.485156e+01 4.000000e+00
16 9.750000e-04 2.261800e-01 0.000000e+00 7.425781e+00 4.000000e+00
32 1.025000e-03 1.402300e-01 0.000000e+00 3.712891e+00 4.000000e+00
64 1.050000e-03 7.967900e-02 0.000000e+00 1.856445e+00 4.000000e+00
128 1.500000e-03 4.382300e-02 0.000000e+00 9.282227e-01 4.000000e+00
256 1.200000e-03 2.191200e-02 0.000000e+00 4.641113e-01 4.000000e+00
512 1.225000e-03 1.095600e-02 0.000000e+00 2.320557e-01 4.000000e+00
1024 1.225000e-03 5.477900e-03 0.000000e+00 1.160278e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0005_ls_4.tex <==
1 2.450000e-03 0.000000e+00 0.000000e+00 6.692562e+03 4.000000e+00
2 1.875000e-03 0.000000e+00 0.000000e+00 3.346281e+03 4.000000e+00
4 1.725000e-03 0.000000e+00 0.000000e+00 1.673141e+03 4.000000e+00
8 1.650000e-03 0.000000e+00 0.000000e+00 8.365703e+02 4.000000e+00
16 1.550000e-03 0.000000e+00 0.000000e+00 4.182852e+02 4.000000e+00
32 1.650000e-03 0.000000e+00 0.000000e+00 2.091426e+02 4.000000e+00
64 1.650000e-03 0.000000e+00 0.000000e+00 1.045713e+02 4.000000e+00
128 1.700000e-03 0.000000e+00 0.000000e+00 5.228564e+01 4.000000e+00
256 1.725000e-03 0.000000e+00 0.000000e+00 2.614282e+01 4.000000e+00
512 2.050000e-03 0.000000e+00 0.000000e+00 1.307141e+01 4.000000e+00
1024 1.750000e-03 0.000000e+00 0.000000e+00 6.535706e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0006_gc_1.tex <==
1 1.075000e-03 7.974600e-01 1.511628e+02 8.000417e+02 4.000000e+00
2 1.025000e-03 7.733200e-01 1.512195e+02 4.000208e+02 4.000000e+00
4 9.750000e-04 7.266500e-01 1.512821e+02 2.000104e+02 4.000000e+00
8 1.025000e-03 7.216800e-01 1.414634e+02 1.000052e+02 4.000000e+00
16 1.050000e-03 5.545500e-01 1.452381e+02 5.000260e+01 4.000000e+00
32 1.100000e-03 3.873700e-01 1.818182e+02 2.500130e+01 4.000000e+00
64 1.100000e-03 2.232300e-01 1.613636e+02 1.250065e+01 4.000000e+00
128 1.100000e-03 1.266400e-01 1.500000e+02 6.250326e+00 4.000000e+00
256 1.075000e-03 6.456200e-02 1.441860e+02 3.125163e+00 4.000000e+00
512 1.050000e-03 3.292600e-02 1.785714e+02 1.562581e+00 4.000000e+00
1024 1.075000e-03 1.679900e-02 1.488372e+02 7.812907e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0006_gc_4.tex <==
1 8.400000e-03 8.698800e-01 1.410714e+02 4.802960e+04 3.000000e+00
2 4.866667e-03 8.345700e-01 1.464041e+02 2.401480e+04 3.000000e+00
4 3.500000e-03 7.662900e-01 1.264286e+02 1.200740e+04 3.000000e+00
8 3.033333e-03 6.886600e-01 1.046703e+02 6.003701e+03 3.000000e+00
16 2.533333e-03 5.545500e-01 1.026316e+02 3.001850e+03 3.000000e+00
32 2.800000e-03 3.817600e-01 1.125000e+02 1.500925e+03 3.000000e+00
64 2.700000e-03 2.270800e-01 1.138889e+02 7.504626e+02 3.000000e+00
128 2.566667e-03 1.291200e-01 1.022727e+02 3.752313e+02 3.000000e+00
256 2.333333e-03 6.719700e-02 9.857143e+01 1.876156e+02 3.000000e+00
512 2.300000e-03 3.359800e-02 1.010870e+02 9.380782e+01 3.000000e+00
1024 2.300000e-03 1.679900e-02 1.097826e+02 4.690391e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0006_ls_1.tex <==
1 1.625000e-03 5.168000e-01 0.000000e+00 8.000417e+02 4.000000e+00
2 1.550000e-03 4.792500e-01 0.000000e+00 4.000208e+02 4.000000e+00
4 1.475000e-03 4.576100e-01 0.000000e+00 2.000104e+02 4.000000e+00
8 1.450000e-03 4.222700e-01 0.000000e+00 1.000052e+02 4.000000e+00
16 1.525000e-03 3.657700e-01 0.000000e+00 5.000260e+01 4.000000e+00
32 2.000000e-03 3.557500e-01 0.000000e+00 2.500130e+01 4.000000e+00
64 1.775000e-03 2.360900e-01 0.000000e+00 1.250065e+01 4.000000e+00
128 1.650000e-03 1.855000e-01 0.000000e+00 6.250326e+00 4.000000e+00
256 1.550000e-03 1.202300e-01 0.000000e+00 3.125163e+00 4.000000e+00
512 1.875000e-03 6.762900e-02 0.000000e+00 1.562581e+00 4.000000e+00
1024 1.600000e-03 3.864500e-02 0.000000e+00 7.812907e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0006_ls_4.tex <==
1 1.185000e-02 0.000000e+00 0.000000e+00 4.802960e+04 4.000000e+00
2 7.125000e-03 0.000000e+00 0.000000e+00 2.401480e+04 4.000000e+00
4 4.425000e-03 0.000000e+00 0.000000e+00 1.200740e+04 4.000000e+00
8 3.175000e-03 0.000000e+00 0.000000e+00 6.003701e+03 4.000000e+00
16 2.600000e-03 0.000000e+00 0.000000e+00 3.001850e+03 4.000000e+00
32 3.150000e-03 0.000000e+00 0.000000e+00 1.500925e+03 4.000000e+00
64 3.075000e-03 0.000000e+00 0.000000e+00 7.504626e+02 4.000000e+00
128 2.625000e-03 0.000000e+00 0.000000e+00 3.752313e+02 4.000000e+00
256 2.300000e-03 0.000000e+00 0.000000e+00 1.876156e+02 4.000000e+00
512 2.325000e-03 0.000000e+00 0.000000e+00 9.380782e+01 4.000000e+00
1024 2.525000e-03 0.000000e+00 0.000000e+00 4.690391e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0007_gc_1.tex <==
1 3.200000e-03 8.981900e-01 1.679688e+02 5.898104e+03 3.000000e+00
2 2.233333e-03 8.921200e-01 1.656716e+02 2.949052e+03 3.000000e+00
4 1.733333e-03 8.816600e-01 1.716346e+02 1.474526e+03 3.000000e+00
8 1.600000e-03 8.619200e-01 1.578125e+02 7.372630e+02 3.000000e+00
16 1.600000e-03 8.492500e-01 1.359375e+02 3.686315e+02 3.000000e+00
32 2.733333e-03 5.065700e-01 8.871951e+01 1.843158e+02 3.000000e+00
64 3.100000e-03 6.648700e-01 9.677419e+01 9.215788e+01 3.000000e+00
128 2.766667e-03 4.722500e-01 1.391566e+02 4.607894e+01 3.000000e+00
256 2.533333e-03 3.081100e-01 1.332237e+02 2.303947e+01 3.000000e+00
512 1.966667e-03 1.885500e-01 1.538136e+02 1.151973e+01 3.000000e+00
1024 1.800000e-03 1.070600e-01 1.347222e+02 5.759867e+00 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0007_gc_4.tex <==
1 6.840000e-02 9.432500e-01 1.419956e+02 3.656660e+05 3.000000e+00
2 3.460000e-02 9.376400e-01 1.398844e+02 1.828330e+05 3.000000e+00
4 1.703333e-02 9.255700e-01 1.414873e+02 9.141649e+04 3.000000e+00
8 9.333333e-03 9.094300e-01 1.411607e+02 4.570825e+04 3.000000e+00
16 5.900000e-03 8.674700e-01 1.338983e+02 2.285412e+04 3.000000e+00
32 5.333333e-03 8.020700e-01 1.078125e+02 1.142706e+04 3.000000e+00
64 4.200000e-03 6.562400e-01 1.380952e+02 5.713531e+03 3.000000e+00
128 3.833333e-03 4.953900e-01 1.304348e+02 2.856765e+03 3.000000e+00
256 3.900000e-03 3.281200e-01 1.320513e+02 1.428383e+03 3.000000e+00
512 3.933333e-03 1.914000e-01 1.347458e+02 7.141914e+02 3.000000e+00
1024 3.500000e-03 1.089000e-01 1.185714e+02 3.570957e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0007_ls_1.tex <==
1 5.375000e-03 5.329600e-01 0.000000e+00 5.898104e+03 4.000000e+00
2 3.700000e-03 5.259800e-01 0.000000e+00 2.949052e+03 4.000000e+00
4 2.975000e-03 5.069800e-01 0.000000e+00 1.474526e+03 4.000000e+00
8 2.525000e-03 4.843700e-01 0.000000e+00 7.372630e+02 4.000000e+00
16 2.175000e-03 4.591800e-01 0.000000e+00 3.686315e+02 4.000000e+00
32 2.425000e-03 4.376700e-01 0.000000e+00 1.843158e+02 4.000000e+00
64 3.000000e-03 4.150600e-01 0.000000e+00 9.215788e+01 4.000000e+00
128 3.850000e-03 3.665900e-01 0.000000e+00 4.607894e+01 4.000000e+00
256 3.375000e-03 3.178700e-01 0.000000e+00 2.303947e+01 4.000000e+00
512 3.025000e-03 2.025100e-01 0.000000e+00 1.151973e+01 4.000000e+00
1024 2.425000e-03 1.531200e-01 0.000000e+00 5.759867e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0007_ls_4.tex <==
1 9.712500e-02 0.000000e+00 0.000000e+00 3.656660e+05 4.000000e+00
2 4.840000e-02 0.000000e+00 0.000000e+00 1.828330e+05 4.000000e+00
4 2.410000e-02 0.000000e+00 0.000000e+00 9.141649e+04 4.000000e+00
8 1.317500e-02 0.000000e+00 0.000000e+00 4.570825e+04 4.000000e+00
16 7.900000e-03 0.000000e+00 0.000000e+00 2.285412e+04 4.000000e+00
32 5.750000e-03 0.000000e+00 0.000000e+00 1.142706e+04 4.000000e+00
64 5.800000e-03 0.000000e+00 0.000000e+00 5.713531e+03 4.000000e+00
128 5.000000e-03 0.000000e+00 0.000000e+00 2.856765e+03 4.000000e+00
256 5.150000e-03 0.000000e+00 0.000000e+00 1.428383e+03 4.000000e+00
512 5.300000e-03 0.000000e+00 0.000000e+00 7.141914e+02 4.000000e+00
1024 4.150000e-03 0.000000e+00 0.000000e+00 3.570957e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0008_gc_1.tex <==
1 1.763333e-02 9.478800e-01 1.691399e+02 4.537383e+04 3.000000e+00
2 9.900000e-03 9.594600e-01 1.896465e+02 2.268692e+04 3.000000e+00
4 5.866667e-03 9.450700e-01 1.853693e+02 1.134346e+04 3.000000e+00
8 3.700000e-03 9.421300e-01 1.959459e+02 5.671729e+03 3.000000e+00
16 2.766667e-03 9.343600e-01 1.734940e+02 2.835865e+03 3.000000e+00
32 4.000000e-03 9.340800e-01 9.187500e+01 1.417932e+03 3.000000e+00
64 3.766667e-03 5.576300e-01 8.960177e+01 7.089661e+02 3.000000e+00
128 4.500000e-03 8.719800e-01 1.011111e+02 3.544831e+02 3.000000e+00
256 5.300000e-03 7.935000e-01 9.245283e+01 1.772415e+02 3.000000e+00
512 6.133333e-03 6.122700e-01 8.885870e+01 8.862077e+01 3.000000e+00
1024 5.466667e-03 4.549900e-01 1.010671e+02 4.431038e+01 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0008_gc_4.tex <==
1 5.233000e-01 9.727100e-01 1.357252e+02 2.858333e+06 3.000000e+00
2 2.734667e-01 9.718000e-01 1.482539e+02 1.429167e+06 3.000000e+00
4 1.392000e-01 9.698300e-01 1.477550e+02 7.145833e+05 3.000000e+00
8 7.063333e-02 9.663600e-01 1.474516e+02 3.572916e+05 3.000000e+00
16 3.513333e-02 9.600800e-01 1.492884e+02 1.786458e+05 3.000000e+00
32 2.510000e-02 9.560300e-01 1.311753e+02 8.932291e+04 3.000000e+00
64 1.410000e-02 9.248300e-01 1.184397e+02 4.466145e+04 3.000000e+00
128 9.200000e-03 8.495800e-01 1.152174e+02 2.233073e+04 3.000000e+00
256 6.466667e-03 7.689000e-01 1.128866e+02 1.116536e+04 3.000000e+00
512 5.233333e-03 6.482900e-01 1.366242e+02 5.582682e+03 3.000000e+00
1024 4.833333e-03 4.549900e-01 1.515517e+02 2.791341e+03 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0008_ls_1.tex <==
1 2.982500e-02 6.277100e-01 0.000000e+00 4.537383e+04 4.000000e+00
2 1.877500e-02 5.332900e-01 0.000000e+00 2.268692e+04 4.000000e+00
4 1.087500e-02 5.243000e-01 0.000000e+00 1.134346e+04 4.000000e+00
8 7.250000e-03 5.205100e-01 0.000000e+00 5.671729e+03 4.000000e+00
16 4.800000e-03 5.076900e-01 0.000000e+00 2.835865e+03 4.000000e+00
32 3.675000e-03 4.841600e-01 0.000000e+00 1.417932e+03 4.000000e+00
64 3.375000e-03 4.638700e-01 0.000000e+00 7.089661e+02 4.000000e+00
128 4.550000e-03 4.486200e-01 0.000000e+00 3.544831e+02 4.000000e+00
256 4.900000e-03 4.182700e-01 0.000000e+00 1.772415e+02 4.000000e+00
512 5.450000e-03 3.849100e-01 0.000000e+00 8.862077e+01 4.000000e+00
1024 5.525000e-03 3.558300e-01 0.000000e+00 4.431038e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0008_ls_4.tex <==
1 7.102500e-01 0.000000e+00 0.000000e+00 2.858333e+06 4.000000e+00
2 4.054250e-01 0.000000e+00 0.000000e+00 1.429167e+06 4.000000e+00
4 2.056750e-01 0.000000e+00 0.000000e+00 7.145833e+05 4.000000e+00
8 1.041500e-01 0.000000e+00 0.000000e+00 3.572916e+05 4.000000e+00
16 5.245000e-02 0.000000e+00 0.000000e+00 1.786458e+05 4.000000e+00
32 3.292500e-02 0.000000e+00 0.000000e+00 8.932291e+04 4.000000e+00
64 1.670000e-02 0.000000e+00 0.000000e+00 4.466145e+04 4.000000e+00
128 1.060000e-02 0.000000e+00 0.000000e+00 2.233073e+04 4.000000e+00
256 7.300000e-03 0.000000e+00 0.000000e+00 1.116536e+04 4.000000e+00
512 7.150000e-03 0.000000e+00 0.000000e+00 5.582682e+03 4.000000e+00
1024 7.325000e-03 0.000000e+00 0.000000e+00 2.791341e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0009_gc_1.tex <==
1 1.290333e-01 9.735700e-01 1.360501e+02 3.561329e+05 3.000000e+00
2 6.576667e-02 9.734400e-01 1.633806e+02 1.780664e+05 3.000000e+00
4 3.370000e-02 9.731600e-01 1.910237e+02 8.903322e+04 3.000000e+00
8 1.800000e-02 9.792700e-01 2.018056e+02 4.451661e+04 3.000000e+00
16 1.053333e-02 9.715600e-01 2.012658e+02 2.225831e+04 3.000000e+00
32 8.100000e-03 9.757400e-01 1.506173e+02 1.112915e+04 3.000000e+00
64 6.500000e-03 9.708500e-01 1.253846e+02 5.564576e+03 3.000000e+00
128 5.833333e-03 9.631200e-01 1.157143e+02 2.782288e+03 3.000000e+00
256 5.300000e-03 9.443400e-01 1.084906e+02 1.391144e+03 3.000000e+00
512 5.533333e-03 9.211100e-01 9.036145e+01 6.955721e+02 3.000000e+00
1024 7.300000e-03 8.569000e-01 8.835616e+01 3.477860e+02 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0009_gc_4.tex <==
8 5.423333e-01 9.792700e-01 1.531530e+02 2.826665e+06 3.000000e+00
16 2.749000e-01 9.782500e-01 1.543834e+02 1.413332e+06 3.000000e+00
32 2.264667e-01 7.895900e-01 1.336952e+02 7.066662e+05 3.000000e+00
64 1.139333e-01 9.842100e-01 1.400161e+02 3.533331e+05 3.000000e+00
128 5.656667e-02 9.705500e-01 1.434148e+02 1.766665e+05 3.000000e+00
256 2.773333e-02 9.581400e-01 1.258413e+02 8.833327e+04 3.000000e+00
512 1.493333e-02 9.178900e-01 1.248884e+02 4.416664e+04 3.000000e+00
1024 1.060000e-02 8.550300e-01 1.179245e+02 2.208332e+04 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0009_ls_1.tex <==
1 1.755500e-01 7.740700e-01 0.000000e+00 3.561329e+05 4.000000e+00
2 1.074500e-01 6.314100e-01 0.000000e+00 1.780664e+05 4.000000e+00
4 6.437500e-02 5.333300e-01 0.000000e+00 8.903322e+04 4.000000e+00
8 3.632500e-02 5.288800e-01 0.000000e+00 4.451661e+04 4.000000e+00
16 2.120000e-02 5.272500e-01 0.000000e+00 2.225831e+04 4.000000e+00
32 1.220000e-02 5.212300e-01 0.000000e+00 1.112915e+04 4.000000e+00
64 8.150000e-03 5.092900e-01 0.000000e+00 5.564576e+03 4.000000e+00
128 6.750000e-03 4.868500e-01 0.000000e+00 2.782288e+03 4.000000e+00
256 5.750000e-03 4.673700e-01 0.000000e+00 1.391144e+03 4.000000e+00
512 5.000000e-03 4.581100e-01 0.000000e+00 6.955721e+02 4.000000e+00
1024 6.450000e-03 4.428700e-01 0.000000e+00 3.477860e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0009_ls_4.tex <==
8 8.306000e-01 0.000000e+00 0.000000e+00 2.826665e+06 4.000000e+00
16 4.244000e-01 0.000000e+00 0.000000e+00 1.413332e+06 4.000000e+00
32 3.027750e-01 0.000000e+00 0.000000e+00 7.066662e+05 4.000000e+00
64 1.595250e-01 0.000000e+00 0.000000e+00 3.533331e+05 4.000000e+00
128 8.112500e-02 0.000000e+00 0.000000e+00 1.766665e+05 4.000000e+00
256 3.490000e-02 0.000000e+00 0.000000e+00 8.833327e+04 4.000000e+00
512 1.865000e-02 0.000000e+00 0.000000e+00 4.416664e+04 4.000000e+00
1024 1.250000e-02 0.000000e+00 0.000000e+00 2.208332e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0010_gc_1.tex <==
8 2.087500e-01 9.998600e-01 1.227425e+02 3.527983e+05 2.000000e+00
16 6.720000e-02 9.863800e-01 1.958705e+02 1.763992e+05 2.000000e+00
32 4.405000e-02 9.893700e-01 1.728150e+02 8.819958e+04 2.000000e+00
64 2.360000e-02 9.854700e-01 1.719280e+02 4.409979e+04 2.000000e+00
128 1.530000e-02 9.843100e-01 1.573529e+02 2.204990e+04 2.000000e+00
256 1.110000e-02 9.858200e-01 1.274775e+02 1.102495e+04 2.000000e+00
512 9.000000e-03 9.802700e-01 1.155556e+02 5.512474e+03 2.000000e+00
1024 7.800000e-03 9.680000e-01 1.086538e+02 2.756237e+03 2.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0010_gc_4.tex <==
128 4.722667e-01 9.912000e-01 1.511434e+02 1.405642e+06 3.000000e+00
256 2.402333e-01 9.941900e-01 1.424657e+02 7.028210e+05 3.000000e+00
512 1.200333e-01 9.802700e-01 1.413149e+02 3.514105e+05 3.000000e+00
1024 5.873333e-02 9.761500e-01 1.371027e+02 1.757053e+05 3.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0010_ls_1.tex <==
8 2.562250e-01 5.333400e-01 0.000000e+00 3.527983e+05 4.000000e+00
16 1.316250e-01 5.311100e-01 0.000000e+00 1.763992e+05 4.000000e+00
32 7.612500e-02 5.303200e-01 0.000000e+00 8.819958e+04 4.000000e+00
64 4.057500e-02 5.272900e-01 0.000000e+00 4.409979e+04 4.000000e+00
128 2.407500e-02 5.214600e-01 0.000000e+00 2.204990e+04 4.000000e+00
256 1.415000e-02 5.099400e-01 0.000000e+00 1.102495e+04 4.000000e+00
512 1.040000e-02 4.882400e-01 0.000000e+00 5.512474e+03 4.000000e+00
1024 8.475000e-03 4.679500e-01 0.000000e+00 2.756237e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0010_ls_4.tex <==
64 1.419100e+00 0.000000e+00 0.000000e+00 2.811284e+06 4.000000e+00
128 7.138000e-01 0.000000e+00 0.000000e+00 1.405642e+06 4.000000e+00
256 3.422500e-01 0.000000e+00 0.000000e+00 7.028210e+05 4.000000e+00
512 1.696250e-01 0.000000e+00 0.000000e+00 3.514105e+05 4.000000e+00
1024 8.052500e-02 0.000000e+00 0.000000e+00 1.757053e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0011_gc_1.tex <==
128 9.550000e-02 9.963400e-01 1.717277e+02 1.755771e+05 2.000000e+00
256 4.665000e-02 9.944300e-01 1.757771e+02 8.778855e+04 2.000000e+00
512 2.590000e-02 9.920400e-01 1.780888e+02 4.389428e+04 2.000000e+00
1024 1.750000e-02 9.906700e-01 1.621429e+02 2.194714e+04 2.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0011_ls_1.tex <==
128 1.640000e-01 5.303700e-01 0.000000e+00 1.755771e+05 4.000000e+00
256 8.200000e-02 5.274200e-01 0.000000e+00 8.778855e+04 4.000000e+00
512 4.612500e-02 5.216400e-01 0.000000e+00 4.389428e+04 4.000000e+00
1024 2.837500e-02 5.102900e-01 0.000000e+00 2.194714e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hmg-quadrant/data_0011_ls_4.tex <==
1024 8.420250e-01 0.000000e+00 0.000000e+00 1.401853e+06 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0003_gc_4.tex <==
1 5.000000e-04 1.200000e-01 0.000000e+00 1.936458e+02 4.000000e+00
2 5.250000e-04 6.000000e-02 0.000000e+00 9.682292e+01 4.000000e+00
4 5.250000e-04 3.000000e-02 0.000000e+00 4.841146e+01 4.000000e+00
8 5.500000e-04 1.500000e-02 0.000000e+00 2.420573e+01 4.000000e+00
16 5.250000e-04 7.500000e-03 0.000000e+00 1.210286e+01 4.000000e+00
32 5.750000e-04 3.750000e-03 0.000000e+00 6.051432e+00 4.000000e+00
64 5.500000e-04 1.875000e-03 0.000000e+00 3.025716e+00 4.000000e+00
128 5.750000e-04 9.375000e-04 0.000000e+00 1.512858e+00 4.000000e+00
256 6.000000e-04 4.687500e-04 0.000000e+00 7.564290e-01 4.000000e+00
512 6.250000e-04 2.343700e-04 0.000000e+00 3.782145e-01 4.000000e+00
1024 6.250000e-04 1.171900e-04 0.000000e+00 1.891073e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0003_ls_4.tex <==
1 6.000000e-04 1.585600e-01 0.000000e+00 1.936458e+02 4.000000e+00
2 6.000000e-04 7.928200e-02 0.000000e+00 9.682292e+01 4.000000e+00
4 6.250000e-04 3.964100e-02 0.000000e+00 4.841146e+01 4.000000e+00
8 6.250000e-04 1.982100e-02 0.000000e+00 2.420573e+01 4.000000e+00
16 6.250000e-04 9.910300e-03 0.000000e+00 1.210286e+01 4.000000e+00
32 7.000000e-04 4.955200e-03 0.000000e+00 6.051432e+00 4.000000e+00
64 6.750000e-04 2.477600e-03 0.000000e+00 3.025716e+00 4.000000e+00
128 6.750000e-04 1.238800e-03 0.000000e+00 1.512858e+00 4.000000e+00
256 7.500000e-04 6.193900e-04 0.000000e+00 7.564290e-01 4.000000e+00
512 7.500000e-04 3.097000e-04 0.000000e+00 3.782145e-01 4.000000e+00
1024 8.500000e-04 1.548500e-04 0.000000e+00 1.891073e-01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0004_gc_4.tex <==
1 1.000000e-03 3.592700e-01 0.000000e+00 1.053188e+03 4.000000e+00
2 9.750000e-04 2.146800e-01 0.000000e+00 5.265938e+02 4.000000e+00
4 9.750000e-04 1.333600e-01 0.000000e+00 2.632969e+02 4.000000e+00
8 1.075000e-03 6.472100e-02 0.000000e+00 1.316484e+02 4.000000e+00
16 1.100000e-03 3.236100e-02 0.000000e+00 6.582422e+01 4.000000e+00
32 1.150000e-03 1.667100e-02 0.000000e+00 3.291211e+01 4.000000e+00
64 1.075000e-03 8.335300e-03 0.000000e+00 1.645605e+01 4.000000e+00
128 1.100000e-03 4.167700e-03 0.000000e+00 8.228027e+00 4.000000e+00
256 1.125000e-03 2.083800e-03 0.000000e+00 4.114014e+00 4.000000e+00
512 1.150000e-03 1.041900e-03 0.000000e+00 2.057007e+00 4.000000e+00
1024 1.175000e-03 5.209600e-04 0.000000e+00 1.028503e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0004_ls_4.tex <==
1 1.250000e-03 3.337500e-01 0.000000e+00 1.053188e+03 4.000000e+00
2 1.250000e-03 2.528400e-01 0.000000e+00 5.265938e+02 4.000000e+00
4 1.250000e-03 1.896300e-01 0.000000e+00 2.632969e+02 4.000000e+00
8 1.300000e-03 1.043000e-01 0.000000e+00 1.316484e+02 4.000000e+00
16 1.325000e-03 5.489300e-02 0.000000e+00 6.582422e+01 4.000000e+00
32 1.475000e-03 2.744700e-02 0.000000e+00 3.291211e+01 4.000000e+00
64 1.375000e-03 1.372300e-02 0.000000e+00 1.645605e+01 4.000000e+00
128 1.425000e-03 6.861600e-03 0.000000e+00 8.228027e+00 4.000000e+00
256 1.500000e-03 3.430800e-03 0.000000e+00 4.114014e+00 4.000000e+00
512 1.425000e-03 1.715400e-03 0.000000e+00 2.057007e+00 4.000000e+00
1024 1.550000e-03 8.577000e-04 0.000000e+00 1.028503e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0005_gc_4.tex <==
1 1.950000e-03 6.257900e-01 0.000000e+00 6.692562e+03 4.000000e+00
2 1.700000e-03 5.122600e-01 0.000000e+00 3.346281e+03 4.000000e+00
4 1.550000e-03 3.911200e-01 0.000000e+00 1.673141e+03 4.000000e+00
8 1.475000e-03 2.894300e-01 0.000000e+00 8.365703e+02 4.000000e+00
16 1.425000e-03 1.682700e-01 0.000000e+00 4.182852e+02 4.000000e+00
32 1.400000e-03 8.413600e-02 0.000000e+00 2.091426e+02 4.000000e+00
64 1.400000e-03 4.307000e-02 0.000000e+00 1.045713e+02 4.000000e+00
128 1.425000e-03 2.206000e-02 0.000000e+00 5.228564e+01 4.000000e+00
256 1.425000e-03 1.103000e-02 0.000000e+00 2.614282e+01 4.000000e+00
512 1.450000e-03 5.515000e-03 0.000000e+00 1.307141e+01 4.000000e+00
1024 1.450000e-03 2.757500e-03 0.000000e+00 6.535706e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0005_ls_4.tex <==
1 2.225000e-03 4.655100e-01 0.000000e+00 6.692562e+03 4.000000e+00
2 2.025000e-03 4.186100e-01 0.000000e+00 3.346281e+03 4.000000e+00
4 1.950000e-03 3.505900e-01 0.000000e+00 1.673141e+03 4.000000e+00
8 1.850000e-03 2.921500e-01 0.000000e+00 8.365703e+02 4.000000e+00
16 1.750000e-03 2.417800e-01 0.000000e+00 4.182852e+02 4.000000e+00
32 1.775000e-03 1.460800e-01 0.000000e+00 2.091426e+02 4.000000e+00
64 1.775000e-03 8.347300e-02 0.000000e+00 1.045713e+02 4.000000e+00
128 1.825000e-03 4.382300e-02 0.000000e+00 5.228564e+01 4.000000e+00
256 1.950000e-03 2.191200e-02 0.000000e+00 2.614282e+01 4.000000e+00
512 1.950000e-03 1.095600e-02 0.000000e+00 1.307141e+01 4.000000e+00
1024 1.975000e-03 5.477900e-03 0.000000e+00 6.535706e+00 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0006_gc_4.tex <==
1 8.050000e-03 8.698800e-01 0.000000e+00 4.802960e+04 4.000000e+00
2 4.925000e-03 8.345700e-01 0.000000e+00 2.401480e+04 4.000000e+00
4 3.200000e-03 7.662900e-01 0.000000e+00 1.200740e+04 4.000000e+00
8 2.575000e-03 6.504000e-01 0.000000e+00 6.003701e+03 4.000000e+00
16 2.325000e-03 5.216100e-01 0.000000e+00 3.001850e+03 4.000000e+00
32 2.975000e-03 3.873700e-01 0.000000e+00 1.500925e+03 4.000000e+00
64 3.025000e-03 2.232300e-01 0.000000e+00 7.504626e+02 4.000000e+00
128 3.000000e-03 1.266400e-01 0.000000e+00 3.752313e+02 4.000000e+00
256 2.575000e-03 1.646300e-01 0.000000e+00 1.876156e+02 4.000000e+00
512 2.575000e-03 9.684200e-02 0.000000e+00 9.380782e+01 4.000000e+00
1024 2.425000e-03 5.879700e-02 0.000000e+00 4.690391e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0006_ls_4.tex <==
1 8.475000e-03 5.592300e-01 0.000000e+00 4.802960e+04 4.000000e+00
2 5.225000e-03 5.354500e-01 0.000000e+00 2.401480e+04 4.000000e+00
4 3.625000e-03 5.246300e-01 0.000000e+00 1.200740e+04 4.000000e+00
8 3.050000e-03 4.679200e-01 0.000000e+00 6.003701e+03 4.000000e+00
16 2.750000e-03 4.637400e-01 0.000000e+00 3.001850e+03 4.000000e+00
32 2.825000e-03 3.657700e-01 0.000000e+00 1.500925e+03 4.000000e+00
64 2.800000e-03 2.497100e-01 0.000000e+00 7.504626e+02 4.000000e+00
128 2.500000e-03 1.855000e-01 0.000000e+00 3.752313e+02 4.000000e+00
256 2.700000e-03 1.202300e-01 0.000000e+00 1.876156e+02 4.000000e+00
512 2.550000e-03 6.762900e-02 0.000000e+00 9.380782e+01 4.000000e+00
1024 2.600000e-03 3.864500e-02 0.000000e+00 4.690391e+01 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0007_gc_4.tex <==
1 6.695000e-02 9.432500e-01 0.000000e+00 3.656660e+05 4.000000e+00
2 3.287500e-02 9.376400e-01 0.000000e+00 1.828330e+05 4.000000e+00
4 1.572500e-02 9.255700e-01 0.000000e+00 9.141649e+04 4.000000e+00
8 1.077500e-02 9.094300e-01 0.000000e+00 4.570825e+04 4.000000e+00
16 6.550000e-03 8.674700e-01 0.000000e+00 2.285412e+04 4.000000e+00
32 5.175000e-03 7.834200e-01 0.000000e+00 1.142706e+04 4.000000e+00
64 6.025000e-03 6.562400e-01 0.000000e+00 5.713531e+03 4.000000e+00
128 4.775000e-03 5.003000e-01 0.000000e+00 2.856765e+03 4.000000e+00
256 4.700000e-03 3.081100e-01 0.000000e+00 1.428383e+03 4.000000e+00
512 5.975000e-03 1.943500e-01 0.000000e+00 7.141914e+02 4.000000e+00
1024 5.575000e-03 1.707100e-01 0.000000e+00 3.570957e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0007_ls_4.tex <==
1 6.867500e-02 6.069800e-01 0.000000e+00 3.656660e+05 4.000000e+00
2 3.415000e-02 6.021500e-01 0.000000e+00 1.828330e+05 4.000000e+00
4 1.637500e-02 5.867600e-01 0.000000e+00 9.141649e+04 4.000000e+00
8 1.125000e-02 5.658900e-01 0.000000e+00 4.570825e+04 4.000000e+00
16 6.375000e-03 5.473900e-01 0.000000e+00 2.285412e+04 4.000000e+00
32 4.750000e-03 5.534200e-01 0.000000e+00 1.142706e+04 4.000000e+00
64 4.325000e-03 5.022300e-01 0.000000e+00 5.713531e+03 4.000000e+00
128 5.475000e-03 3.692900e-01 0.000000e+00 2.856765e+03 4.000000e+00
256 6.150000e-03 3.261200e-01 0.000000e+00 1.428383e+03 4.000000e+00
512 6.700000e-03 2.025100e-01 0.000000e+00 7.141914e+02 4.000000e+00
1024 4.125000e-03 1.531200e-01 0.000000e+00 3.570957e+02 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0008_gc_4.tex <==
1 5.202750e-01 9.602100e-01 0.000000e+00 2.858333e+06 4.000000e+00
2 2.658000e-01 9.594600e-01 0.000000e+00 1.429167e+06 4.000000e+00
4 1.333750e-01 9.581200e-01 0.000000e+00 7.145833e+05 4.000000e+00
8 1.036500e-01 9.793300e-01 0.000000e+00 3.572916e+05 4.000000e+00
16 4.762500e-02 9.715400e-01 0.000000e+00 1.786458e+05 4.000000e+00
32 2.325000e-02 9.435300e-01 0.000000e+00 8.932291e+04 4.000000e+00
64 1.322500e-02 9.079000e-01 0.000000e+00 4.466145e+04 4.000000e+00
128 8.275000e-03 8.495800e-01 0.000000e+00 2.233073e+04 4.000000e+00
256 8.375000e-03 7.689000e-01 0.000000e+00 1.116536e+04 4.000000e+00
512 8.100000e-03 6.199300e-01 0.000000e+00 5.582682e+03 4.000000e+00
1024 7.825000e-03 4.678700e-01 0.000000e+00 2.791341e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0008_ls_4.tex <==
1 5.283500e-01 6.965500e-01 0.000000e+00 2.858333e+06 4.000000e+00
2 2.715500e-01 6.617800e-01 0.000000e+00 1.429167e+06 4.000000e+00
4 1.374000e-01 6.596400e-01 0.000000e+00 7.145833e+05 4.000000e+00
8 1.058250e-01 5.768500e-01 0.000000e+00 3.572916e+05 4.000000e+00
16 4.885000e-02 5.076900e-01 0.000000e+00 1.786458e+05 4.000000e+00
32 2.390000e-02 6.489300e-01 0.000000e+00 8.932291e+04 4.000000e+00
64 1.265000e-02 6.031700e-01 0.000000e+00 4.466145e+04 4.000000e+00
128 7.750000e-03 5.776400e-01 0.000000e+00 2.233073e+04 4.000000e+00
256 6.850000e-03 4.173900e-01 0.000000e+00 1.116536e+04 4.000000e+00
512 7.575000e-03 3.849100e-01 0.000000e+00 5.582682e+03 4.000000e+00
1024 9.100000e-03 3.956800e-01 0.000000e+00 2.791341e+03 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0009_gc_4.tex <==
8 8.627500e-01 9.922400e-01 0.000000e+00 2.826665e+06 4.000000e+00
16 4.284250e-01 9.978300e-01 0.000000e+00 1.413332e+06 4.000000e+00
32 2.167750e-01 9.825200e-01 0.000000e+00 7.066662e+05 4.000000e+00
64 1.062250e-01 9.708500e-01 0.000000e+00 3.533331e+05 4.000000e+00
128 5.017500e-02 9.631200e-01 0.000000e+00 1.766665e+05 4.000000e+00
256 2.522500e-02 9.443400e-01 0.000000e+00 8.833327e+04 4.000000e+00
512 1.467500e-02 9.168200e-01 0.000000e+00 4.416664e+04 4.000000e+00
1024 1.257500e-02 8.587700e-01 0.000000e+00 2.208332e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0009_ls_4.tex <==
8 8.755500e-01 5.915500e-01 0.000000e+00 2.826665e+06 4.000000e+00
16 4.353000e-01 5.272500e-01 0.000000e+00 1.413332e+06 4.000000e+00
32 2.198500e-01 6.651000e-01 0.000000e+00 7.066662e+05 4.000000e+00
64 1.066750e-01 6.497700e-01 0.000000e+00 3.533331e+05 4.000000e+00
128 5.020000e-02 5.935000e-01 0.000000e+00 1.766665e+05 4.000000e+00
256 2.432500e-02 5.852100e-01 0.000000e+00 8.833327e+04 4.000000e+00
512 1.495000e-02 5.265800e-01 0.000000e+00 4.416664e+04 4.000000e+00
1024 1.367500e-02 5.463500e-01 0.000000e+00 2.208332e+04 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0010_gc_4.tex <==
256 2.179750e-01 9.889300e-01 0.000000e+00 7.028210e+05 4.000000e+00
512 1.076250e-01 9.838100e-01 0.000000e+00 3.514105e+05 4.000000e+00
1024 5.282500e-02 9.659100e-01 0.000000e+00 1.757053e+05 4.000000e+00


==> global-coarsening-paper-data/large-scaling/hpmg-quadrant/data_0010_ls_4.tex <==
128 4.397250e-01 7.055400e-01 0.000000e+00 1.405642e+06 4.000000e+00
256 2.201500e-01 6.897700e-01 0.000000e+00 7.028210e+05 4.000000e+00
512 1.088750e-01 6.000300e-01 0.000000e+00 3.514105e+05 4.000000e+00
1024 5.325000e-02 5.956900e-01 0.000000e+00 1.757053e+05 4.000000e+00


==> global-coarsening-paper-data/small-scaling-gc-default/annulus_summary.tex <==
5  & 4.4e+1 & 21\% & 15\% & 2.8e-3 & 5.8e-3 \\
6  & 9.2e+1 & 52\% & 20\% & 3.8e-3 & 8.2e-3 \\
7  & 3.0e+2 & 83\% & 46\% & 5.4e-3 & 1.7e-2 \\
8  & 1.8e+3 & 96\% & 73\% & 9.6e-3 & 7.6e-2 \\
9  & 1.3e+4 & 99\% & 87\% & 3.1e-2 & 5.9e-1 \\
10  & 1.0e+5 & 99\% & 93\% & 1.7e-1 & - \\


==> global-coarsening-paper-data/small-scaling-gc-default/profile-0192.tex <==
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
   title={},
   bar width=14pt,
   width=0.64\textwidth,
   height=0.41\textwidth,
   ylabel={Time [s]},
   xlabel={Level [-]}, 
   xmajorgrids,xminorgrids,
   ymajorgrids,yminorgrids,
   xmin=-0.5,xmax=8.500000,
   ymin=0.0, ymax=0.111609,
   xtick distance=1,legend columns=3, legend pos={north west}
]
\addlegendimage{ybar,ybar legend,blue, fill=blue!40!white}
\addlegendentry{min};
\addlegendimage{ybar,ybar legend,red, fill=red!40!white}
\addlegendentry{max};
\addlegendimage{}
\addlegendentry{avg};
\addplot [ybar stacked, blue, fill=blue!40!white] coordinates {
(0, 0.000078)
(1, 0.000023)
(2, 0.000019)
(3, 0.000019)
(4, 0.000021)
(5, 0.000597)
(6, 0.001503)
(7, 0.010472)
(8, 0.075988)
};
\addplot [ybar stacked, red, fill=red!40!white] coordinates {
(0, 0.000586)
(1, 0.000184)
(2, 0.000296)
(3, 0.000432)
(4, 0.000649)
(5, 0.000494)
(6, 0.000898)
(7, 0.007504)
(8, 0.025475)
};
\draw (axis cs:-0.400000,0.000471) -- (axis cs:0.400000,0.000471);
\draw (axis cs:0.600000,0.000028) -- (axis cs:1.400000,0.000028);
\draw (axis cs:1.600000,0.000034) -- (axis cs:2.400000,0.000034);
\draw (axis cs:2.600000,0.000063) -- (axis cs:3.400000,0.000063);
\draw (axis cs:3.600000,0.000327) -- (axis cs:4.400000,0.000327);
\draw (axis cs:4.600000,0.000818) -- (axis cs:5.400000,0.000818);
\draw (axis cs:5.600000,0.001618) -- (axis cs:6.400000,0.001618);
\draw (axis cs:6.600000,0.011688) -- (axis cs:7.400000,0.011688);
\draw (axis cs:7.600000,0.094069) -- (axis cs:8.400000,0.094069);
\end{axis}
\end{tikzpicture}


==> global-coarsening-paper-data/small-scaling-gc-default/quadrant_summary.tex <==
3  & 2.5e+1 & 3\% & 0\% & 1.1e-3 & 2.3e-3 \\
4  & 3.4e+1 & 12\% & 1\% & 1.8e-3 & 4.0e-3 \\
5  & 6.6e+1 & 43\% & 1\% & 2.9e-3 & 7.5e-3 \\
6  & 2.5e+2 & 83\% & 3\% & 4.5e-3 & 1.1e-2 \\
7  & 1.7e+3 & 97\% & 7\% & 6.8e-3 & 5.4e-2 \\
8  & 1.3e+4 & 99\% & 16\% & 2.6e-2 & 4.5e-1 \\
9  & 1.0e+5 & 99\% & 33\% & 1.6e-1 & - \\


==> global-coarsening-paper-data/small-scaling-gc-default/workload-0192.tex <==
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
   title={},
   bar width=14pt,
   width=0.64\textwidth,
   height=0.41\textwidth,
   ylabel={Workload [-]},
   xlabel={Level [-]}, 
   xmajorgrids,xminorgrids,
   ymajorgrids,yminorgrids,
   xmin=-0.5,xmax=8.500000,
   ymin=0.0, ymax=12190.200000,
   xtick distance=1,legend columns=3, legend pos={north west}
]
\addlegendimage{ybar,ybar legend,blue, fill=blue!40!white}
\addlegendentry{min};
\addlegendimage{ybar,ybar legend,red, fill=red!40!white}
\addlegendentry{max};
\addlegendimage{}
\addlegendentry{avg};
\addplot [ybar stacked, blue, fill=blue!40!white] coordinates {
(0, 0.000000)
(1, 0.000000)
(2, 0.000000)
(3, 0.000000)
(4, 0.000000)
(5, 20.000000)
(6, 176.000000)
(7, 1400.000000)
(8, 11072.000000)
};
\addplot [ybar stacked, red, fill=red!40!white]  coordinates {
(0, 1.000000)
(1, 8.000000)
(2, 8.000000)
(3, 8.000000)
(4, 9.000000)
(5, 12.000000)
(6, 9.000000)
(7, 12.000000)
(8, 10.000000)
};
\draw (axis cs:-0.400000,0.000000) -- (axis cs:0.400000,0.000000);
\draw (axis cs:0.600000,0.000000) -- (axis cs:1.400000,0.000000);
\draw (axis cs:1.600000,0.000000) -- (axis cs:2.400000,0.000000);
\draw (axis cs:2.600000,0.000000) -- (axis cs:3.400000,0.000000);
\draw (axis cs:3.600000,3.000000) -- (axis cs:4.400000,3.000000);
\draw (axis cs:4.600000,24.000000) -- (axis cs:5.400000,24.000000);
\draw (axis cs:5.600000,181.000000) -- (axis cs:6.400000,181.000000);
\draw (axis cs:6.600000,1406.000000) -- (axis cs:7.400000,1406.000000);
\draw (axis cs:7.600000,11079.000000) -- (axis cs:8.400000,11079.000000);
\end{axis}
\end{tikzpicture}


==> global-coarsening-paper-data/small-scaling-gc-fcp/annulus_summary.tex <==
5  & 2.5e+1 & 38\% & 80\% & 4.0e-3 & 6.6e-3 \\
6  & 1.0e+2 & 48\% & 89\% & 5.1e-3 & 9.3e-3 \\
7  & 5.2e+2 & 48\% & 96\% & 7.4e-3 & 2.2e-2 \\
8  & 2.5e+3 & 69\% & 99\% & 1.2e-2 & 8.2e-2 \\
9  & 1.6e+4 & 84\% & 99\% & 3.7e-2 & 6.2e-1 \\
10  & 1.1e+5 & 92\% & 99\% & 1.9e-1 & - \\


==> global-coarsening-paper-data/small-scaling-gc-fcp/profile-0192.tex <==
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
   title={},
   bar width=14pt,
   width=0.64\textwidth,
   height=0.41\textwidth,
   ylabel={Time [s]},
   xlabel={Level [-]}, 
   xmajorgrids,xminorgrids,
   ymajorgrids,yminorgrids,
   xmin=-0.5,xmax=8.500000,
   ymin=0.0, ymax=0.087249,
   xtick distance=1,legend columns=3, legend pos={north west}
]
\addlegendimage{ybar,ybar legend,blue, fill=blue!40!white}
\addlegendentry{min};
\addlegendimage{ybar,ybar legend,red, fill=red!40!white}
\addlegendentry{max};
\addlegendimage{}
\addlegendentry{avg};
\addplot [ybar stacked, blue, fill=blue!40!white] coordinates {
(0, 0.000047)
(1, 0.000016)
(2, 0.000010)
(3, 0.000011)
(4, 0.000708)
(5, 0.001408)
(6, 0.003273)
(7, 0.010170)
(8, 0.067061)
};
\addplot [ybar stacked, red, fill=red!40!white] coordinates {
(0, 0.000532)
(1, 0.000262)
(2, 0.000384)
(3, 0.000612)
(4, 0.000497)
(5, 0.000319)
(6, 0.000441)
(7, 0.002372)
(8, 0.012256)
};
\draw (axis cs:-0.400000,0.000370) -- (axis cs:0.400000,0.000370);
\draw (axis cs:0.600000,0.000025) -- (axis cs:1.400000,0.000025);
\draw (axis cs:1.600000,0.000030) -- (axis cs:2.400000,0.000030);
\draw (axis cs:2.600000,0.000205) -- (axis cs:3.400000,0.000205);
\draw (axis cs:3.600000,0.001015) -- (axis cs:4.400000,0.001015);
\draw (axis cs:4.600000,0.001534) -- (axis cs:5.400000,0.001534);
\draw (axis cs:5.600000,0.003505) -- (axis cs:6.400000,0.003505);
\draw (axis cs:6.600000,0.011522) -- (axis cs:7.400000,0.011522);
\draw (axis cs:7.600000,0.074967) -- (axis cs:8.400000,0.074967);
\end{axis}
\end{tikzpicture}


==> global-coarsening-paper-data/small-scaling-gc-fcp/quadrant_summary.tex <==
3  & 1.1e+1 & 6\% & 89\% & 1.6e-3 & 2.9e-3 \\
4  & 1.5e+1 & 29\% & 85\% & 2.5e-3 & 4.5e-3 \\
5  & 5.6e+1 & 51\% & 88\% & 3.7e-3 & 5.5e-3 \\
6  & 3.3e+2 & 63\% & 96\% & 5.1e-3 & 1.2e-2 \\
7  & 2.1e+3 & 76\% & 99\% & 7.1e-3 & 5.0e-2 \\
8  & 1.4e+4 & 87\% & 99\% & 2.5e-2 & 4.1e-1 \\
9  & 1.1e+5 & 91\% & 99\% & 1.5e-1 & - \\


==> global-coarsening-paper-data/small-scaling-gc-fcp/workload-0192.tex <==
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
   title={},
   bar width=14pt,
   width=0.64\textwidth,
   height=0.41\textwidth,
   ylabel={Workload [-]},
   xlabel={Level [-]}, 
   xmajorgrids,xminorgrids,
   ymajorgrids,yminorgrids,
   xmin=-0.5,xmax=8.500000,
   ymin=0.0, ymax=12540.000000,
   xtick distance=1,legend columns=3, legend pos={north west}
]
\addlegendimage{ybar,ybar legend,blue, fill=blue!40!white}
\addlegendentry{min};
\addlegendimage{ybar,ybar legend,red, fill=red!40!white}
\addlegendentry{max};
\addlegendimage{}
\addlegendentry{avg};
\addplot [ybar stacked, blue, fill=blue!40!white] coordinates {
(0, 0.000000)
(1, 0.000000)
(2, 0.000000)
(3, 0.000000)
(4, 2.000000)
(5, 20.000000)
(6, 160.000000)
(7, 1266.000000)
(8, 7351.000000)
};
\addplot [ybar stacked, red, fill=red!40!white]  coordinates {
(0, 1.000000)
(1, 3.000000)
(2, 3.000000)
(3, 30.000000)
(4, 83.000000)
(5, 205.000000)
(6, 485.000000)
(7, 814.000000)
(8, 4049.000000)
};
\draw (axis cs:-0.400000,0.000000) -- (axis cs:0.400000,0.000000);
\draw (axis cs:0.600000,0.000000) -- (axis cs:1.400000,0.000000);
\draw (axis cs:1.600000,0.000000) -- (axis cs:2.400000,0.000000);
\draw (axis cs:2.600000,0.000000) -- (axis cs:3.400000,0.000000);
\draw (axis cs:3.600000,3.000000) -- (axis cs:4.400000,3.000000);
\draw (axis cs:4.600000,24.000000) -- (axis cs:5.400000,24.000000);
\draw (axis cs:5.600000,181.000000) -- (axis cs:6.400000,181.000000);
\draw (axis cs:6.600000,1406.000000) -- (axis cs:7.400000,1406.000000);
\draw (axis cs:7.600000,11079.000000) -- (axis cs:8.400000,11079.000000);
\end{axis}
\end{tikzpicture}

